One RL to See Them All: Visual Triple Unified Reinforcement Learning

Reinforcement learning (RL) is becoming an important direction for post-training vision-language models (VLMs), but public training methodologies for unified multimodal RL remain much less mature, especially for heterogeneous reasoning and perception-heavy tasks. We propose V-Triune, a Visual Triple Unified Reinforcement Learning methodology for unified multimodal RL. It organizes training around three coordinated abstractions: Sample-Level Reward Routing, Verifier-Level Outcome Verification, and Source-Level Diagnostics. Within this methodology, Dynamic IoU provides localization-specific reward shaping that avoids reward ambiguity under loose thresholds and reward sparsity under strict ones. Built on V-Triune, we develop Orsta (7B, 32B), a family of models jointly trained on eight reasoning and perception tasks. Under matched budgets, unified training matches or outperforms specialist mixtures. The final Orsta models improve over their backbones on MEGA-Bench, compare favorably with strong multi-task RL-VLM baselines, and transfer these gains to a broad set of downstream benchmarks. These results show that unified RL can improve both reasoning and perception within a single VLM RL pipeline.The V-Triune system, along with the Orsta models, is publicly available at https://github.com/MiniMax-AI/One-RL-to-See-Them-All.

==> 1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
%
The recent advancement of large language models (LLMs)~\cite{DBLP:journals/corr/abs-2412-16720,guo2025deepseek} and visual-language models (VLMs)~\cite{openai2025o3o4,google_deepmind_gemini_2025} has seen a paradigm shift from pre-training scaling to test-time scaling.
%
A key manifestation of this shift is the practice of extending context length for Chain-of-Thought (CoT) reasoning, which significantly enhances performance on complex tasks such as mathematics and coding~\cite{xia2025generative, guo2025deepseek}.

While reinforcement learning (RL) has emerged as a promising method for post-training VLMs, current research remains limited~\cite{liu2025visual,ma2025deepperception,yang2025r1,tan2025reason,liu2025othink,yu2025perception,shen2025vlm,wang2025vl,li2025minimax}.
%
Most prior work has focused on narrow task domains—typically visual reasoning tasks like math QA and Science QA~\cite{huang2025vision,yang2025r1,meng2025mm}, where the RL setup closely mirrors RL training paradigms in LLMs.
%where the RL setup aligns closely with traditional LLM paradigms.
%
Moreover, existing works~\cite{liu2025visionreasoner,liu2025x} remain an open question whether RL can be effectively scaled to visual perception tasks such as object detection and grounding, which require distinct reward design and measures to ensure training stability.


We introduce V-Triune (\textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning), the first unified RL system for post-training VLMs on both visual reasoning and perception tasks.
%
V-Triune integrates three complementary components, each operating at a distinct level for this unification:
%
\textit{Sample-Level Data Formatting} (detailed in \cref{subsec:sample_level_formatting}) handles diverse task and reward needs by allowing each sample to define its reward setup and chosen verifier.
%
\textit{Verifier-Level Reward Computation} (\cref{subsec:verifier_level_reward_computation}) offers key modularity and task-adaptability by assigning reward generation to specialized verifiers for specific task groups.
%
Lastly, \textit{Source-Level Metric Monitoring} (\cref{subsec:metric_monitoring}) provides essential tracking and diagnostics by logging metrics per data source, vital for spotting data issues and ensuring stable multi-task, multi-source learning.
%
Beyond these core components, a key innovation in V-Triune is the Dynamic IoU reward (\cref{subsec:dynamic_iou}).
%
This mechanism targets visual perception tasks like object detection and grounding, addressing issues with fixed IoU thresholds.
%
By progressively adjusting the IoU reward threshold (from relaxed to stricter criteria), it ensures useful early learning signals, guides the model towards high-precision results, and ultimately enables stable, scalable training procedure.

Leveraging the V-Triune system, we develop the Orsta model series, featuring variants with sizes ranging from 7B to 32B, built upon the Qwen2.5-VL family of baselines. These models undergo joint optimization across a diverse set of tasks, spanning visual reasoning (mathematics, science, chart, puzzle) and visual perception (object detection, grounding, OCR, counting).
%
On the comprehensive MEGA-Bench core benchmark~\cite{chen2024mega}, which covers over 400 real-world visual tasks, Orsta demonstrates substantial performance gains. These improvements range from +2.1\% up to an impressive +14.1\% across its various 7B and 32B model variants.
%
These performance benefits extend to prominent downstream benchmarks (including MMMU, MathVista, COCO, and CountBench), validating V-Triune's effectiveness and scalability.
%
Our core contributions are:
%
\begin{itemize}
\item We introduce V-Triune, the first unified, scalable, and extensible RL system designed for jointly training VLMs on both visual reasoning and perception tasks within a single paradigm.
%
\item We propose the Dynamic IoU Reward, a novel, adaptive reward mechanism that significantly enhances stability and performance for visual perception tasks like detection and grounding.
%
\item We establish and demonstrate a comprehensive training methodology, including key engineering optimizations, enabling effective and stable RL training across eight diverse VLM tasks spanning both reasoning and perception.
%
\item We present Orsta, a family of high-performance models (7B-32B) trained with V-Triune, achieving substantial gains (up to +14.1\%) on the MEGA-Bench Core and strong performance across various downstream benchmarks.
\end{itemize}
%
% \noindent \textbf{Summary of Core Contributions}:
% \begin{itemize}
%     \item \textbf{V-Triune} is the first unified, extensible, and scalable reinforcement learning system for vision-language models (VLMs) that supports both visual reasoning and perception tasks within a single training paradigm. It features a modular design with three tiers: Sample-Level Data Formatting, Verifier-Level Reward Computation, and Source-Level Metric Monitoring.
%     
%     \item \textbf{Dynamic IoU reward}, a novel reward function for visual perception tasks, significantly improves performance on detection- and grounding-related benchmarks.  
% 
%     \item \textbf{Reasoning and Perception Training}: V-Triune is evaluated on eight diverse tasks—Math, Science, Charting, Puzzle, Detection, Grounding, Counting, and OCR. To ensure stable and efficient RL training, we incorporate key engineering optimizations, resolving unintended image special tokens and out-of-memory failures.
% 
%     \item \textbf{Orsta}, trained using V-Triune, achieves compatible performance on MEGA-Bench core, with gains of \textbf{+3.2} (7B) and \textbf{+2.1} (32B), and shows consistent improvements across downstream reasoning and perception benchmarks.
% \end{itemize}


% \item V-Triune is designed to support flexible task extension, scalable data sizes, and varied model scales, making it applicable across a broad range of VLM-RL training scenarios.
% V-Triune is architected around three complementary RL components, each operating at a distinct level to achieve this unification:
%
% Sample-Level Data Formatting tackles the inherent diversity in task requirements and reward structures by enabling fine-grained, per-sample specification of reward configurations and the designated verifiers.
%
% Verifier-Level Reward Computation introduces crucial modularity and task-adaptability by delegating reward signal generation to specialized, user-defined verifiers, each responsible for a specific group of tasks and operating within an asynchronous server architecture. Finally, Source-Level Metric Monitoring provides indispensable traceability and diagnostic capabilities by facilitating per-source logging of metrics, which is vital for identifying data quality issues and ensuring stable learning dynamics in a multi-task, multi-source environment. Beyond these structural components, a pivotal innovation within V-Triune is the Dynamic IoU reward. This mechanism is tailored for visual perception tasks like object detection and grounding, addressing the shortcomings of fixed IoU thresholds. By progressively adapting the IoU threshold for rewards—starting leniently and gradually increasing stringency—it ensures informative gradients during early training phases while guiding the model towards a high-precision objective, ultimately enabling stable and scalable optimization.

%V-Triune is built upon a three-tiered RL components: \textit{Sample-Level Data Formatting}, \textit{Verifier-Level Reward Computation}, and \textit{Source-Level Metric Monitoring}. Besides, another key innovation in V-Triune is the Dynamic IoU reward, which enables stable and scalable optimization for visual perception tasks like object detection and grounding.

%V-Triune is built around three complementary components, each working at a different level to achieve this unification:
%
% \textit{Sample-Level Data Formatting} (detailed in \cref{subsec:sample_level_formatting}) handles diverse task and reward needs by allowing each sample to define its reward setup and chosen verifier.
%
% \textit{Verifier-Level Reward Computation} offers key modularity and adaptability for different tasks. It does this by assigning reward generation to specialized verifiers, each designed for specific task groups (and can operate via an asynchronous server, as detailed in the~\cref{subsec:verifier_level_reward_computation}.
%
% Finally, \textit{Source-Level Metric Monitoring} (discussed in \cref{subsec:metric_monitoring}) provides essential tracking and diagnostic scheme.
%
% By logging metrics for each data source, it is vital for spotting data quality issues and ensuring stable learning in multi-task, multi-source settings.
%
% Beyond these core components, a key innovation in V-Triune is the Dynamic IoU reward (explained in \cref{subsec:dynamic_iou}). This mechanism is specifically designed for visual perception tasks like object detection and grounding, addressing the problems with fixed IoU thresholds. By progressively adjusting the IoU reward threshold—starting with a more relaxed rule that gradually becomes stricter—it ensures useful learning signals early in training and guides the model towards high-precision results, ultimately leading to stable and scalable optimization."
%
%
%Leveraging this unified system design, we develop two high-performance models: Orsta-7B and Orsta-32B, based on Qwen2.5-VL. These models are jointly optimized across diverse visual reasoning tasks (mathematics, science, chart, puzzle) and visual perception tasks (object detection, grounding, OCR, counting). Orsta achieves consistent gains of +3.2\% (7B) and +2.1\% (32B) on the MEGA-Bench core benchmark~\cite{chen2024mega}, which spans over 400 real-world visual tasks. Furthermore, Orsta demonstrates compatible performance on prominent downstream benchmarks, including MMMU, MathVista, COCO, and CountBench, validating the scalability and effectiveness of the proposed RL framework.



% \noindent \textbf{Summary of Core Contributions}:
% \begin{itemize}
%     \item \textbf{Task scalability:} we propose a unified and task-scalable RL training protocol for VLMs that supports flexible task extension and jointly integrates 10 visual-language tasks spanning both visual perception and reasoning.
%     \item \textbf{Novel perception reward:} we propose a novel rule-based dynamic IoU reward function for visual perception tasks, leading to consistent performance gains on COCO, OVDEval, and Screenshot Pro.
%     \item \textbf{Model scalability:} we design a stable training strategy that generalizes effectively across model scales, achieving 3\% (7B) and 5\% (32B) improvements on MEGA-Bench Core under a unified framework.
%     % \item \textbf{Contribution to community:} we will release our dataset and training framework, contributing the first open-source RL pipeline tailored for scalable, multi-domain VLM training.
% \end{itemize}

% \noindent \textbf{Summary of Core Contributions}:
% \begin{itemize}
% \item We introduce \textbf{V-Triune}, the first unified reinforcement learning system for vision-language models that supports both visual reasoning and perception tasks within a single training paradigm. Notably, the proposed \textit{Dynamic IoU reward} inside V-Triune enhances the learning effectiveness on perception tasks.
% \item \textbf{Orsta}, trained using V-Triune, achieves compatible performance on real-world tasks in MEGA-Bench Core, with improvements of \textbf{+3.2} on the 7B model and \textbf{+2.1} on the 32B model.
% \item V-Triune is designed for flexibility and scalability, as it supports seamless task extension, accommodates large-scale data, and generalizes across different sizes of VLMs.
% \end{itemize}
%
%Furthermore, Orsta achieves competitive performance on prominent downstream benchmarks such as MMMU, MathVista, COCO, and CountBench. These results validate the effectiveness and scalability of our proposed unified RL framework.
%


==> 2_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

% \subsection{Reinforcement Learning from Verified Rewards}
% \label{subsec:rlvr}


The advent of Deepseek-R1~\citep{guo2025deepseek} has established Reinforcement Learning as one of the dominant paradigms for post-training LLMs.
%
Specifically, training through RL canlead to remarkably strong performance on reasoning tasks such as mathematics, code, and puzzles~\cite{xia2025generative, openai2025thinking}.
%
RL encompasses two main key components: the algorithm and (verifiable) reward function.
%
\subsection{RL Algorithm}
\label{subsec:rlvr}
We adopt Group Relative Policy Optimization (GRPO)~\cite{shao2024deepseekmath}, following standard practice, but introduce two key modifications based on recent work~\cite{yu2025dapo, hu2025open}.
%
First, we remove the reference model and its associated KL loss. This avoids restricting exploration~\cite{hu2025open} and prevents unstable KL divergence estimates~\cite{schulman2020klapprox}, while also reducing GPU memory usage and speeding up training.
Second, we apply the clip-high trick and use token-level loss, which help increase output entropy, encouraging better exploration and improving training stability.
With these changes, the GRPO objective is updated as follows:

\begin{equation}
\begin{aligned}
\mathcal{J}(\theta) &= \mathbb{E}_{q \sim \mathcal{P}(q), \{o_i\}_{i=1}^G \sim \pi_{\theta_{\text{old}}}(\cdot|q)} \\ 
&\left[ \frac{1}{\sum_{i=1}^G |o_i|} \sum_{i=1}^G \sum_{t=1}^{|o_i|} \min \left( r_{i,t}(\theta) \hat{A}_{i,t}, \text{clip}(r_{i,t}(\theta), 1 - \varepsilon_{\text{low}}, 1 + \varepsilon_{\text{high}})\hat{A}_{i,t} \right) \right] 
\end{aligned}
\end{equation}
where
\begin{equation}
\begin{aligned}
\quad \quad & r_{i,t}(\theta) = \frac{\pi_\theta(o_{i,t} \mid q, o_{i,<t})}{\pi_{\theta_{\text{old}}}(o_{i,t} \mid q, o_{i,<t})}, \quad \hat{A}_{i,t} = \frac{R_i - \text{mean}(\{R_i\}_{i=1}^G)}{\text{std}(\{R_i\}_{i=1}^G)}.
\end{aligned}
\end{equation}
In this equation, $\mathcal{P}(q)$ represents the distribution of queries.%  
The behavior model $\pi_{\theta_{\text{old}}}$ samples a group of $G$ responses $\{o_i\}_{i=1}^G$ for each query.% 
Then, the advantage of the $i$-th response $\hat{A}_{i,t}$ is calculated from the normalized group-level rewards $\{R_i\}_{i=1}^G$,
and then used to update the policy $\pi_{\theta}$.
%
The clipping range of the importance sampling ratio $r$ is bounded by $\epsilon_{\text{low}}$ and $\epsilon_{\text{high}}$.%



\subsection{Reward function} 
As discussed in~\cref{sec:intro}, visual tasks involved can be grouped into two categories: visual reasoning and visual perception.
%
To mitigate the risk of reward hacking~\cite{weng2024rewardhack}, rule-based reward functions are employed for each task.
%
For visual reasoning tasks, a binary (0-1) reward function is employed based on accuracy, as defined by the following rule:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = 
    \begin{cases} 
    1, &  \text{if}~\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a))~\text{is~True} \\
    0, & \text{else} 
    \end{cases}
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ represents the ground-truth (or golden) answer.
%
$\hat{a}$ is parsed from model output, which is instructed to be enclosed within \texttt{\textbackslash{}boxed\{\}}, and verified against the golden answer $a$ using \texttt{math\_verify}~\cite{mathverify2025}.
%

For visual perception tasks, the format of the ground-truth varies considerably.
%
The answers for counting and verifiable OCR tasks are typically numbers, words, or open-ended phrases, which can be conveniently enclosed in \texttt{\textbackslash{}boxed\{\}}.
%
Therefore, a rule-based accuracy reward, as defined in~\cref{eq:math_rule}, is utilized for these tasks.
%
In contrast, the answers for grounding and detection tasks are commonly structured in COCO-style \texttt{JSON} format, which includes both a bounding box and a label.
%
% for instance, \texttt{\{``bbox\_2d'': [484, 227, 818, 998], ``label'': ``shiba dog''\}},
%
Initial experiments revealed that the model struggled to learn enclosing such JSON format within the \texttt{\textbackslash{}boxed\{\}}, but readily learned to include it within \texttt{<answer></answer>} tags.
%
Consequently, for these two tasks, a format reward is established by referencing~\cite{openr1} setup:
%
\begin{equation}
\begin{aligned}
R_{\text{format}}(o_q) = 0.25 & \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1) \\
s_1 = \texttt{<think>}, s_2 = \texttt{</think>},&  s_3 = \texttt{<answer>}, s_4 = \texttt{</answer>}
\end{aligned}
\end{equation}
%
where $o_q$ represents the model's response to question $q$, and $s_i$ denotes a specific format tag. The indicator function $\mathbb{I}(\text{condition})$ evaluates to 1 if the condition is true, and 0 otherwise.
%
For the accuracy reward, Intersection over Union (IoU)~\cite{everingham2010pascal} with a defined threshold and mean Average Precision (mAP)~\cite{lin2014microsoft} are commonly adopted in prior works~\cite{liu2025visual,yu2025perception,shen2025vlm}. The corresponding formulations for the IoU-based reward and mAP are provided in~\cref{eq:iou_rule} and~\cref{eq:map_definition}, respectively.
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = 
    \begin{cases} 
    \text{IoU}(\hat{a}, a), &  \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
    0, & \text{else} 
    \end{cases}
    \label{eq:iou_rule}
\end{equation}
%
where
%
\begin{equation}
\begin{aligned}
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\end{aligned}
\end{equation}
%
$\hat{a}$ represents the predicted bounding box, and $a$ denotes the golden bounding box.
%
The threshold $\epsilon$ controls the strictness of the reward function, with higher values enforcing tighter matches. We adopt a dynamic $\epsilon$ finally, as detailed in~\cref{subsec:dynamic_iou}.
%
The mAP is calculated using interpolated precision curve:
\begin{equation}
  \mathrm{AP}_c \;=\;
  \int_{0}^{1} 
    \underbrace{\bigl(\max_{\tilde r \,\ge r} P_c(\tilde r)\bigr)}_{\text{interpolated precision }P_c^{\mathrm{interp}}(r)}
    \, \mathrm d r,
  \qquad
  \mathrm{mAP} \;=\;
  \frac{1}{C}\,\sum_{c=1}^{C} \mathrm{AP}_c.
  \label{eq:map_definition}
\end{equation}
%
Finally, the overall reward combines accuracy and format alignment, expressed as:
\begin{equation}
    \begin{aligned}
    \alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}
    \end{aligned}
\end{equation}
where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are the respective weighting coefficients for each reward component.


% The final reward is formulated as: $\alpha_{acc}\cdot R_{acc} + \alpha_{format} \cdot R_{format}$, where $\alpha$ represent the corresponding reward coefficients.

% Regarding the selection of $\epsilon$, we found that setting it too leniently or too stringently resulted in performance degradation during the later stages of training.
% %
% To address this issue, a dynamic IoU threshold strategy is designed.
% %
% Analogous to curriculum learning~\yan{cite}, this strategy adjusts $\epsilon$ from loose to tight during training and empirically demonstrates significant stabilization.
% %
% Empirical results demonstrate that this approach significantly stabilizes training.
% %
% More details are provided in~\cref{sec:method}.%


% \subsection{Vision Language Models}
% \label{subsec:pre-vlm}
% We adopt the Qwen2.5-VL series as the backbone model in our work. This architecture combines a large language model (LLM) with a redesigned Vision Transformer (ViT), which incorporates 2D Rotary Position Embedding (2D-RoPE) and windowed attention to enable efficient image encoding. To address the challenge of long visual feature sequences, a two-layer MLP-based merger is introduced. This module spatially compresses grouped image patches prior to alignment with the LLM’s text embeddings. Our experiments primarily utilize the 7B and 32B variants of the LLM, comprising 28 and 64 transformer layers, respectively. Both models share an identical ViT configuration with 32 layers and a patch size of 14. The models are trained on 4 trillion tokens during the multimodal pre-training stage, followed by supervised fine-tuning (SFT) on 2 million instances.

% ------------------- Move to later Section ------------------
% We adopt the Qwen2.5-VL~\cite{Qwen2.5-VL} series as the backbone model in our work. This architecture combines a LLM with a redesigned Vision Transformer (ViT), which incorporates 2D Rotary Position Embedding and windowed attention to enable efficient image encoding. To address the challenge of long visual feature sequences, a two-layer MLP-based merger is introduced. This module spatially compresses grouped image patches prior to alignment with the LLM’s text embeddings. Our experiments primarily utilize the 7B and 32B variants of the LLM, comprising 28 and 64 transformer layers, respectively. Both models share an identical ViT configuration with 32 layers and a patch size of 14. The models are trained on 4 trillion tokens during the multimodal pre-training stage, followed by supervised fine-tuning (SFT) on 2 million instances.
% -----------------------------------------------------------

% \subsection{Vision-Language Benchmarks}
% Vision-language tasks span a wide spectrum, from perception and understanding to complex reasoning and decision-making, each with distinct output formats that require tailored evaluation protocols. For tasks with discrete outputs, such as mathematical reasoning, puzzles, STEM problems, and counting, performance is directly assessed by comparing model predictions to golden references. In contrast, for structured outputs like object detection with bounding boxes and categories, the evaluation is conducted using mean Average Precision (mAP), which captures both localization and classification accuracy. The Average Precision (AP) for each category is computed as the area under its Precision-Recall Curve (PRC), and mAP is the mean of AP scores across all categories. For visual grounding tasks, accuracy is evaluated using varying IoU thresholds (e.g., Acc@0.5, Acc@0.9), reflecting the ability to spatially align language expressions with image regions. In OCR tasks with free-form textual answers, evaluation relies on sequence similarity metrics, such as BLEU, METEOR, F-measure, and edit distance, which quantify the alignment between predicted and ground-truth text.


% The evaluation of  VLMs' downstream ability heavily relies on a diverse array of benchmarks designed to probe various capabilities. Key among these is MEGA-Bench, noted as a pioneering real-world task benchmark due to its extensive collection of over 500 tasks reflecting heterogeneous daily use-cases and diverse output formats. For general knowledge, MMMU challenges models with expert-level, multi-discipline questions, while Mathvista specifically assesses mathematical problem-solving within visual contexts. Domain-specific abilities are tested by benchmarks like Screenspot-pro for UI element grounding in high-resolution professional software, CountBench for object counting accuracy, and OCRBench-v2 for advanced visual text localization, extraction, and reasoning. Foundational perception benchmarks such as COCO continue to be vital for object detection (often adapted for VLM evaluation), and OVDEval  focuses on nuanced open-vocabulary detection and grounding capabilities. To push the boundaries of current models, the highly challenging benchmarks presents tasks designed to be nearly impossible for contemporary VLMs, such as ZeroBench, Olympiadbench, thereby highlighting areas for future advancement and providing rigorous tests of model robustness and generalization.



% ------------------- Move to later Section ------------------
% The evaluation of downstream capabilities in vision-language models (VLMs) relies on a comprehensive suite of benchmarks that assess a wide range of skills. MEGA-Bench~\cite{chen2024mega} features over 500 real-world tasks encompassing diverse modalities and use cases, making it a cornerstone for general-purpose VLM evaluation. For domain-specific and knowledge-intensive reasoning, MMMU~\cite{yue2024mmmu} challenges models with expert-level, multidisciplinary questions, while MathVista~\cite{lu2023mathvista} focuses on mathematical problem-solving within visual contexts. Specialized perception and grounding abilities are assessed by benchmarks such as ScreenSpot-Pro~\cite{li2025screenspot}, which targets UI element localization in professional software interfaces; CountBench~\cite{paiss2023teaching}, which measures object counting accuracy; and OCRBench v2~\cite{fu2024ocrbench}, which evaluates text localization, extraction, and reasoning in visual scenes. Traditional benchmarks like COCO~\cite{lin2014microsoft} remain essential for object detection and are often adapted for VLM tasks, whereas OVDEval~\cite{yao2023evaluate} extends this to open-vocabulary detection and grounding, emphasizing nuanced semantic understanding. To push the limits of current models, highly challenging benchmarks such as ZeroBench~\cite{roberts2025zerobench} and OlympiadBench~\cite{he2024olympiadbench} include tasks that are nearly infeasible for today’s VLMs, offering rigorous evaluations of robustness, generalization, and areas in need of further advancement.
% -----------------------------------------------------------

% \paragraph{RL algorithm} Similar to most research, Group Relative Policy Optimization (GRPO) is adopted. 
% %
% Unlike the classic GRPO design~\cite{grpo}, our approach incorporates valuable modifications drawn from recent research~\cite{dqpo, orz}. 
% %
% First, the reference model and the corresponding KL loss are abandoned. 
% %
% This is because the reference model might constrain the policy model's exploration~\cite{orz} and introduce issues related to fluctuating KL divergence estimation~\cite{kl3}.
% %
% An additional benefit of this modification is the reduction in GPU memory usage and an increase in training speed.
% %
% Second, the clip-high trick and token-level loss are incorporated.
% %
% These techniques have been empirically shown to enhance the output entropy of the model, thereby promoting exploration and stabilizing training.
% %
% Combining these two modifications, the updated objective function is given by:

% Besides, both theoretical analysis and empirical results support that it is unreasonable for VLM to give a confident score, while the output order of bounding box is ranked from the top confidence to the bottom confidence since its auto-regressive manner. 
%
% In our initial experiments, it is observed
% In this context, $\mathbb{I}(\text{count}(o_q, s_i) = 1)$ checks if the tag $s_i$ appears exactly once in the model's response $o_q$. The reward $R_{\text{format}}(o_q)$ is then 0.25 times the sum of these indicator functions over the four specified format tags.

==> 3_method.tex <==
\begin{figure}[tb!]
    \centering    \includegraphics[width=0.98\linewidth]{images/figure2_v6.pdf}
    \caption{\textbf{V-Triune System}. It integrates three complementary components: \textit{Sample-Level Data Formatting} (to unify diverse task inputs), \textit{Verifier-Level Reward Computation} (for custom rewards via specialized verifiers), and \textit{Source-Level Metric Monitoring} (to diagnose data-source level problems). Additionally, a novel Dynamic IoU reward offers adaptive, progressive feedback for perception tasks.}
    \label{fig:framework}
\end{figure}
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}
%
This section describes V-Triune, our visual triple unified RL system. As shown in~\cref{fig:framework}, V-Triune's main goal is to jointly train VLMs on both visual reasoning and perception tasks using a single, unified training pipeline.
%
The system is built upon three core, interconnected parts designed to handle these diverse tasks together.
%
The following subsections will explain these three core components in detail and introduce our novel Dynamic IoU reward mechanism.
%
\subsection{Sample-Level Data Formatting}
\label{subsec:sample_level_formatting}
%
This section introduces how data is formatted to support unified training across perception and reasoning tasks.
%
A main challenge is that different tasks may require different types of rewards, components, and weighting strategies.
%
For example, tasks like math, puzzle, and OCR compute rewards based on the correctness of textual answers, while detection and grounding tasks rely on spatial metrics such as IoU and bounding box formatting.
%
In conventional RL setups, reward computation is typically defined at the task level.
%
While this allows modular reward functions to be implemented externally, it limits flexibility when fine-grained control is required.
%
Many multimodal tasks may contain heterogeneous samples that demand different reward strategies.
%
For instance, OCR data may include both plain-text lines and complex tables, each requiring different evaluation rules.
%
Similarly, detection samples can differ significantly in terms of object count, annotation completeness, or visual difficulty, which suggests the need for sample-wise adjustment of reward behavior.

To support such flexibility, we define reward configurations directly at the sample level.
%
Each sample specifies the types of rewards to compute, their relative weights, and the associated verifier to use.
%
This allows dynamic reward routing and fine-grained weighting during training without modifying core training logic.
%
It can also support curriculum learning or data ablation strategies simply by adjusting metadata, making the system more extensible and maintainable.

As shown in~\cref{fig:data_format}, we implement our data schema using the HuggingFace \texttt{datasets}~\cite{lhoest-etal-2021-datasets}, which serves as the unified interface for all sources described in~\cref{subsec:data}.
%
Besides common fields such as \texttt{images} and \texttt{prompt}, the format includes several task-agnostic keys to support reward control.
%
The \texttt{reward\_model} field encapsulates all reward-related metadata, including fields like \texttt{accuracy\_ratio} and \texttt{format\_ratio}, which define the weight of each reward type.
%
By adjusting these values, specific rewards can be enabled, disabled, or reweighted per sample.
%
The \texttt{verifier} field specifies which verifier should be used for evaluation and provides any required parameters.
%
More details on the verifier system are discussed in~\cref{subsec:verifier_level_reward_computation}.
%
The \texttt{data\_source} field indicates the origin of each sample and is used in source-specific evaluation in~\cref{subsec:metric_monitoring}.
%
In summary, the sample-level formatting design enables seamless integration of diverse datasets into a unified training pipeline, while allowing highly flexible and scalable reward control.
%
\begin{figure}[tb!]
    \centering

    \begin{tcolorbox}[title=Data Format, label={box:data_format}]
    \begin{lstlisting}
{
    "data_source": Value(dtype="string"),
    "images": Sequence(feature=Image(mode=None, decode=True)),
    "prompt": [
        {
            "content": Value(dtype="string"),
            "role": Value(dtype="string")
        }
    ],
    "ability": Value(dtype="string"),
    "reward_model": {
        "answer": Value(dtype="string"),
        "ground_truth": Value(dtype="string"),
        "accuracy_ratio": Value(dtype="float32"),
        "format_ratio": Value(dtype="float32"),
        "verifier": Value(dtype="string"),
        "verifier_parm": Value(dtype="dict")
    },
    "extra_info": {
        "id": Value(dtype="string"),
        "image_path": Value(dtype="string")
    }
}
    \end{lstlisting}
    \end{tcolorbox}
    
    \caption{\textbf{Sample-level Data Scheme for Unified Training}. This format, implemented using HuggingFace datasets, allows fine-grained control over reward computation by defining \texttt{reward\_model} (including reward types, weights like \texttt{accuracy/format\_ratio}) and \texttt{verifier} specifications at the individual sample level. This enables flexible and scalable handling of diverse multimodal tasks.}
    \label{fig:data_format}
\end{figure}
%
%\begin{figure}[tb!]
%    \centering 
%
%    \begin{tcolorbox}[title=Data Format, label={box:data_format}]
%        \begin{minted}[fontsize=\small, breaklines]{python}
%{
%    "data_source": Value(dtype="string"),
%    "images": Sequence(feature=Image(mode=None, decode=True)),
%    "prompt": [
%        {
%            "content": Value(dtype="string"),
%            "role": Value(dtype="string")
%        }
%    ],
%    "ability": Value(dtype="string"),
%    "reward_model": {
%        "answer": Value(dtype="string"),
%        "ground_truth": Value(dtype="string"),
%        "accuracy_ratio": Value(dtype="float32"),
%        "format_ratio": Value(dtype="float32"),
%        "verifier": Value(dtype="string"),
%        "verifier_parm": Value(dtype="dict")
%        }
%    },
%    "extra_info": {
%        "id": Value(dtype="string"),
%        "image_path": Value(dtype="string")
%    }
%}
%        \end{minted}
%    \end{tcolorbox}
%    \caption{\textbf{Sample-level Data Scheme for Unified Training}. This format, implemented using HuggingFace datasets, allows fine-grained control over reward computation by defining \texttt{reward\_model} (including reward types, weights like \texttt{accuracy/format\_ratio}) and \texttt{verifier} specifications at the individual sample level. This enables flexible and scalable handling of diverse multimodal tasks.}
%    \label{fig:data_format}
%
%\end{figure}
%
\subsection{Verifier-Level Reward Computation}
\label{subsec:verifier_level_reward_computation}
%
Unlike approaches using fixed reward functions, we implement a standalone, asynchronous reward server to generate RL signals.
%
Decoupling reward computation from the main training loop offers key advantages: it enhances modularity and extensibility for diverse tasks, supports flexible deployment and independent scaling (crucial for GPU-based evaluations), improves maintainability, and boosts throughput via distributed, asynchronous processing.
%
The term \textit{verifier-level} defines our reward computation granularity: instead of monolithic functions, rewards are delegated to specialized verifiers, each handling specific task groups.

We use an asynchronous client-server architecture (\cref{fig:reward_server}) using FastAPI~\cite{ramirez_fastapi}.
%
The client collects batches of samples from the dataloader and processes them in thread level parallel.
%
Each sample is transformed into a structured payload containing task-specific key-value pairs.
%
The client consists of multiple proxy workers that asynchronously send requests to the server with a dynamic balance strategy.
%
The proxy server routes each request to the appropriate verifier based on the ``\texttt{verifier}'' key in data format.

Each verifier is user-defined, containing custom functions to compute task-specific rewards based on model outputs and ground truth.
%
In our implementation, we primarily use two types:
%
\textit{MathVerifyVerifier}: Handles reasoning, OCR, and counting tasks by evaluating answer correctness.
%
\textit{DetectionVerifier}: Manages detection and grounding tasks, notably employing our novel Dynamic IoU reward (\cref{subsec:dynamic_iou}) alongside format-based rewards.
%
This verifier-level approach grants significant flexibility and modularity.
%
It greatly simplifies adding new tasks or updating reward logic independently, without altering the core training pipeline.
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/reward_server.png}
    \caption{\textbf{Architecture of the Asynchronous Reward Server.} The RL trainer interacts with a remote server via client-server proxies, where specialized verifiers (e.g., MathVerify, Detection) compute rewards using task-specific logic and dynamic thresholds (e.g., dynamic IoU threshold).}
    \label{fig:reward_server}
\end{figure}
%
\subsection{Source-Level Metric Monitoring}
\label{subsec:metric_monitoring}
%
Monitoring training metrics is essential for understanding model dynamics and real-time issue diagnosis.
%
However, for multi-task, multi-source training, aggregated or single-task metrics are often insufficient due to lack of traceability and per-source data variations.
%
Therefore, we adopt source-level metric monitoring.
%
This involves logging metrics per \texttt{data\_source} for each batch.
%
This approach helps identify faulty data sources, enables targeted debugging, and reveals cross-source learning interactions.
%
Such granular monitoring is particularly vital in RL, where training can be unstable, to verify stability and model behavior. We note that while many RL infrastructures support metric logging~\cite{sheng2024hybridflow,hu2024openrlhf}, our source-level detail provides deeper insights.
%
Empirical signs of training stability are further discussed in \cref{sec:training_recipe}.
%
Specifically, we log per-source reward values to trace dataset-specific stability. For perception tasks like grounding and detection, we also log detailed per-source IoU values (at thresholds {50, 75, 95, 99}) and mAP scores for fine-grained convergence insights.

Inspired by~\citet{maye}, we also track model behavior by monitoring response length and reflection ratio per source. For response length, we log various metrics including overall average, lengths of correct/incorrect responses, and truncation rates. Truncation rates (outputs hitting maximum length) can indicate overly verbose or collapsed generation. For reflection ratio, we track 15 pre-defined reflection-related words (e.g., \textit{"re-check", "re-think", "verify"}).
%
We then compute \texttt{reflection ratio}: the proportion of responses containing these reflection words and \texttt{correct ratio in reflection responses}: the accuracy of responses that include these words.
%
This helps diagnose model tendencies like overthinking versus superficial responses by linking reflection to correctness. All mentioned metrics are consistently logged per data source.
%
\subsection{Dynamic IoU Reward}
\label{subsec:dynamic_iou}
%
\begin{figure}[t]
    % \hfill
    \centering
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure5/various_iou_map_compare.pdf}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure5/iou_50_99.pdf}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_coco.pdf}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_ovd.pdf}
        \end{subfigure}
    % \hfill        
    \caption{\textbf{COCO Test Set Performance with Various Reward Designs.} (a) Comparison between IoU-based and mAP-based rewards on a selected COCO multi-object subset; (b) Comparison between vanilla IoU reward and rule-based IoU reward on a selected COCO single-object subset; (c, d) Comparison between rule-based IoU reward and dynamic IoU reward on the COCO multi-object subset and the OVDEval negation subset.}
    \centering
    \label{fig:dyn_iou}
\end{figure}
%
In object detection and visual grounding, Intersection over Union (IoU) and mean Average Precision (mAP) are standard metrics for evaluating the overlap between predicted and ground-truth boxes. While mAP summarizes performance across multiple IoU thresholds, our preliminary detection experiments show that using a thresholded IoU reward achieves comparable overall performance while providing more interpretable and controllable feedback (\cref{fig:dyn_iou}a). Therefore, we adopt an IoU-based reward strategy for its robustness and stronger alignment with localization accuracy (\cref{eq:iou_rule}).

However, relaxed thresholds like $\epsilon = 0.5$ (common option~\cite{liu2025visual,yu2025perception}) can be too lenient for RL in VLMs, especially when compared to the strict exact-match rewards used in reasoning tasks (\cref{eq:math_rule}).
%
%
Moreover, these loose thresholds result in reward ambiguity: even if predicted bounding boxes merely shift or are oriented differently around the ground-truth, they can still receive the same high reward. Such ambiguity
%
can ultimately lead to a decline in performance during later training stages for detection task (\cref{fig:dyn_iou}b).


\begin{wrapfigure}[16]{tr}{0.33\textwidth} 
  \centering
  \includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_ovd_acc.pdf}
  \caption{\textbf{Training accuracy rewards under Dynamic IoU versus a fixed Rule-based IoU (IoU@99).}}
  \label{fig:traning_acc_track}
\end{wrapfigure}

To address these issues, we initially use a rule-based IoU reward scheme that enforces a stringent threshold of $\epsilon=0.99$, requiring near-exact spatial alignment between predicted and ground-truth boxes (\cref{fig:dyn_iou}b).
%
This strict criterion enhances consistency between perception and reasoning signals and, by providing an unambiguous target, aims to improve training stability. However, its very stringency introduces a cold-start problem in early rollouts, where most predictions receive 0 reward.

To mitigate this cold-start problem, we adopt a dynamic IoU reward strategy, inspired by curriculum learning~\cite{bengio2009curriculum}. The IoU threshold $\epsilon$ is adjusted in stages based on training progress: starting at 0.85 for the initial 10\% of training steps, increasing to 0.95 for the subsequent 15\% of steps (i.e., from 10\% to 25\% of total steps), and finally settling at 0.99 for the remainder of training (as illustrated in~\cref{fig:traning_acc_track}).

% This curriculum-based approach, characterized by initially lenient criteria that become progressively stricter, enhances training efficiency. It ensures the model receives informative gradients during early exploration and learning phases (\cref{fig:dyn_iou}c,d), while consistently guiding it towards a high-precision objective."
% To mitigate this, we adopt a \textbf{dynamic IoU reward} inspired by curriculum learning~\cite{bengio2009curriculum}. The IoU threshold $\epsilon$ is gradually increased from 0.85 to 0.99 over training and then fixed at 0.99 (Figure~\ref{fig:traning_acc_track}). This progressive schedule enables informative gradients during early training (Figure~\cref{fig:dyn_iou}c,d), while guiding the Orsta toward a high-precision objective.

% To address these issues, we propose a \textbf{rule-based IoU reward} mechanism that employs a stringent threshold of $\epsilon \geq 0.99$, effectively enforcing exact spatial alignment between predicted and ground-truth boxes as shown in Figure~\cref{fig:dyn_iou}b. While this strict criterion improves the alignment between perception and reasoning signals and enhances training stability, it introduces a cold-start challenge in early rollout stages, where most predictions yield zero reward—particularly when the model backbone is a pre-trained base model without instruction fine-tuning.

% To mitigate this issue, and inspired by curriculum learning strategies~\cite{bengio2009curriculum}, we introduce a \textbf{dynamic IoU thresholding} mechanism. Specifically, the IoU threshold $\epsilon$ is gradually increased from $0.8$ to $0.99$ throughout training, eventually stabilizing at $0.99$, as shown in Figure~\ref{fig:traning_acc_track}. This progressive tightening allows the agent to receive meaningful gradient signals during early training as shown in Figure~\cref{fig:dyn_iou}c and d, while still converging to a high-precision objective in later stages.

% \cref{fig:framework} illustrates the pipeline, where the left part covers the data curation process, and the right part details how the data format is formulated, how the reward server is initiated, and how the model is engaged in interactive training and inference.


% ------------------- Move to later Section ------------------
% \subsection{Data Curation}
% \label{subsec:data}

% This section outlines the data curation process used to prepare high-quality datasets for unified training across various visual tasks.
% %
% Four reasoning tasks are selected: Math, Puzzle, Science, and Chart. These tasks are chosen for their diversity and relevance to different reasoning capabilities.
% %
% Four perception tasks are selected: detection, grounding, counting, and OCR. These tasks are chosen for their comprehensive coverage of key perception challenges.
% %
% The data sources for each task are as follows:


% \begin{itemize}
%     \item For the Math task, \texttt{mm\_math}~\cite{sun2024mm}, \texttt{geometry3k}~\cite{lu2021inter}, and \texttt{mmk12}~\cite{meng2025mm} are chosen.%
%     \item For the Puzzle task, \texttt{PuzzleVQA}\cite{chia2024puzzlevqa} and \texttt{AlgoPuzzleVQA}\cite{ghosal2024algopuzzlevqa} are merged due to their shared origin, and \texttt{VisualPuzzles}~\cite{song2025visualpuzzles} is additionally included.%
% \item For the Science task, \texttt{ScienceQA}~\cite{lu2022learn}, \texttt{SciVQA}~\cite{borisova2025scivqa}, and the ``Broader STEM Topics'' and ``(GradeSchool) Science'' categories from \texttt{ViRL39K}~\cite{wang2025vl} are used.%
%     \item For the Chart task, \texttt{ChartQAPro}~\cite{masry2025chartqapro}, \texttt{ChartX}~\cite{xia2024chartx}, \texttt{Table-VQA}~\cite{kim2024tablevqa}, and the Tables/Diagrams/Charts categories from \texttt{ViRL39K}~\cite{wang2025vl} are used.%
%     \item For the Detection task, \texttt{V3Det}~\cite{xie2023described} and \texttt{Object365}~\cite{shao2019objects365} are chosen.%
%     \item For the Grounding task, \texttt{$D^3$}~\cite{xie2023described} is used.%
%     \item For the Counting task, \texttt{CLEVR}~\cite{johnson2017clevr,tan2025reason} is used.%
%     \item For the OCR task, English OCR questions are extracted from \texttt{LLaVA-OV Data}~\cite{li2024llava} and \texttt{EST-VQA}~\cite{wang2020general}.%
% \end{itemize}

% We express our gratitude to the creators of these outstanding datasets for their invaluable contributions.
% %
% To address potential noisy data, further cleaning is performed.
% %
% As shown in~\cref{fig:data_curation}, data filtering is conducted in two stages: 1) Rule-based Filter, and 2) Difficulty-based Filter.
% %
% \begin{figure}
%     \centering
%     \includegraphics[width=0.98\linewidth]{images/data_curation.pdf}
%     \caption{Data Curation Process. First, visual reasoning and visual perception data pass through a rule-based filter, which removes samples that do not meet preset criteria. Subsequently, the data enters a difficulty filter, which removes samples that are too easy or too hard based on model performance, ultimately producing the Curated Dataset.}
%     \label{fig:data_curation}
% \end{figure}
% %
% \subsubsection{First Stage: Rule-based Filter} 
% %
% For the four visual reasoning tasks, the following filters are applied:
% \begin{itemize}
%     \item Multiple-choice and true/false questions that are prone to hacking are discarded.~\cite{kimiteam2025kimivltechnicalreport}
%     \item Answers containing symbols such as ``='', ``['', ``]'', ``('', ``)'', and ``;'' are removed, as the absence of these symbols may cause answer mismatches even if the numeric values are correct.
%     \item Answers longer than 20 characters are discarded to avoid overly complex answers.
% \end{itemize}

% % For the visual perception tasks, the filtering process is slightly more complex:
% The filtering process for visual perception tasks involves additional complexity:
% %
% \begin{itemize}
%     \item \textbf{Detection:} Following the \texttt{Qwen2.5-VL}~\cite{Qwen2.5-VL}, data is processed into relative coordinates. Single-box and multi-box samples are treated separately: single-box data includes only one bounding box per category, while multi-box data preserves its original structure. Data with more than 10 bounding boxes per category is filtered out. Any data with a box size greater than 50\% of the image is also discarded. A 1:2 ratio of single-box to multi-box data is maintained, and category-level long tails are avoided.%
%     \item \textbf{Grounding:} Data is processed into relative coordinates, and data with a box size greater than 50\% of the image is discarded. Complex phrase labels are filtered out.%
%     \item \textbf{Counting:} Data is balanced per category and only English data is retained.%
%     \item \textbf{OCR:} Only English OCR data is retained, and final labels must be verifiable by \texttt{math\_verify}~\cite{math_verify_2025}. Since no verifiable reward model (RM) is designed, the OCR task data must pass this validation.
% \end{itemize}



% \subsubsection{Second Stage: Difficulty-based Filter}

% \begin{wrapfigure}[18]{tr}{0.5\textwidth} 
%   \centering
%   \includegraphics[width=\linewidth]{images/data_distribution.png}
%   \caption{\textbf{Training Data Distribution of 8 Tasks}} 
%   \label{fig:data_dist}
% \end{wrapfigure}


% %
% Some easy questions may be covered by the base model's capabilities, offering little potential for learning. These should be filtered out.
% %
% For the four reasoning tasks, pass@8 accuracy is computed using \texttt{Qwen2.5-VL-32B-0321}, and only samples with $0 \leq \text{pass@8} < 100\%$ are retained.
% %
% For the perception tasks, \texttt{Qwen2.5-VL-7B} is used to compute pass@16 with an IoU reward threshold of 50.
% %
% Only samples with accumulated IoU rewards between 2 and 10 are retained.

% The curated data is finally packaged into Parquet format~\cite{parquet} and mixed together for training.
% %
% No online filtering process or specific curriculum learning order is implemented, and all data is mixed for training.
% %
% The overall data distribution is visualized in Figure~\ref{fig:data_dist}, and the post-processed statistics for each data source are summarized in Table~\ref{tab:training_data}.


% -----------------------------------------------------------



% \subsection{Data Curation}
% \label{subsec:data}
% This section outlines the data curation process used to prepare high-quality datasets for unified training across various visual tasks.%
% %
% The dataset is divided into two major categories: visual reasoning and visual perception, with distinct data sources for each task.%
% %
% Each task is paired with a specific data source, and preprocessing steps are applied accordingly to ensure data consistency and quality.%
% %
% The curation process follows these key steps:
% 
% \begin{itemize}
%     \item \textbf{Visual Reasoning Tasks:} A rule-based filter is applied to remove problematic queries.%
%     \begin{itemize}
%         \item All multiple-choice questions are discarded.%
%         \item Queries with complex or noisy answers are excluded, including those with ambiguous or irrelevant content.%
%         \item The remaining queries are evaluated using Qwen2.5-VL-32B with pass@8 accuracy.%
%         \item Only samples with $0 \leq \text{acc} < 100\%$ are retained for further training.%
%     \end{itemize}
%     
%     \item \textbf{Visual Perception Tasks:} Task-specific preprocessing steps are applied, including the normalization of relative and absolute coordinates when necessary.%
% \end{itemize}
% 
% Once the data is curated, it is organized into two subsets: one for visual reasoning tasks and one for visual perception tasks.%
% %
% The curated data is then packaged into a Parquet format, ensuring efficient storage and easy access during training.%
% 
% We express our gratitude to the original data sources and contributors for providing the high-quality datasets that enable the success of these tasks.%

% \subsection{Data Curation}
% \label{subsec:data}
% This section describes the methodology for curating high-quality data to support unified training across multiple visual tasks.%
% 
% For visual reasoning tasks, a filtering strategy is applied to enhance data quality.%
% First, all multiple-choice questions are discarded.
% %
% Then, queries with complex or noisy answers, such as [examples needed], are excluded.%
% Finally, Qwen2.5-VL-32B is used to evaluate pass@8 accuracy, and only samples with $0 \leq \text{acc} < 100\%$ are retained for further training.%
% 
% For visual perception tasks, specific preprocessing steps are applied depending on the task requirements.
% %
% This includes the normalization of relative and absolute coordinates when applicable.%
% 
% Each task is paired with a distinct data source, and task-specific preprocessing is conducted accordingly.
% %
% After curation, the final dataset is divided into two major subsets: visual reasoning and visual perception.
% %
% The total number of samples in each subset, along with detailed statistics, is summarized in Table~[refer to the supplementary table].%
% 来一段简介，介绍下这一段干啥。

% Filter用了什么逻辑。对于视觉推理数据：首先去掉多选。然后筛除掉带有复杂的答案的样本和噪声答案的query，例如xxxx。最后，用Qwen2.5-VL-32B打pass@8, 保留0≤ acc <100%的数据。

% % 对于视觉感知数据，我们是如何处理的xxx。相对坐标，绝对坐标。
% \yan{@yema, add a figure to illustrate the partition of each part data}

% 分任务大讲解每个任务都用了什么data source。数据处理好后，两块各自总共多少数据，具体的数据细节可以看土土的表。

% \subsection{V-Triune: Visual Triple Unified Reinforcement Learning}
% \label{sec:main_method}


% --------- 挪到前面了 -----------
% This section introduces the core methodology of the paper.
% %
% The training of perception and reasoning tasks is unified under a single framework to enable efficient learning and generalization across modalities.
% %
% To achieve this, specific designs are proposed to align the objectives of different tasks and optimize learning through reinforcement-based supervision.
% %
% The proposed training paradigm ensures mutual enhancement between perception and reasoning tasks by sharing representations and gradients within a common training loop.

% -------------------------------------------------------

%

%
%
% Overall, our dynamic IoU reward strategy bridges the gap between perception accuracy and reasoning supervision, improves training robustness, and enhances performance on both in-distribution and OOD detection benchmarks.

% The \texttt{verifier\_parm} configuration includes two key components: \texttt{det\_verifier\_normalized} and \texttt{det\_reward\_ratio}.
% %
% \begin{itemize}
%     \item \texttt{det\_verifier\_normalized} (\texttt{bool}): Controls whether the predicted bounding boxes are normalized to account for the actual image size and grid dimensions. When set to \texttt{True}, the bounding boxes are scaled accordingly to maintain consistent measurements across different image sizes.
%     
%     \item \texttt{det\_reward\_ratio} (\texttt{dict}): Defines the weighting of various detection metrics in the reward calculation. This dictionary contains:
%     \begin{itemize}
%         \item \texttt{iou\_max\_label\_first} (\texttt{float32}): Weight for the maximum IoU score when prioritizing label matching.
%         \item \texttt{iou\_max\_iou\_first} (\texttt{float32}): Weight for the maximum IoU score when prioritizing IoU value matching.
%         \item \texttt{iou\_completeness} (\texttt{float32}): Weight for completeness, penalizing missed detections.
%         \item \texttt{map} (\texttt{float32}): Weight for the mean Average Precision (mAP) score across all categories.
%         \item \texttt{map50} (\texttt{float32}): Weight for the mAP score at IoU threshold 0.5.
%         \item \texttt{map75} (\texttt{float32}): Weight for the mAP score at IoU threshold 0.75.
%     \end{itemize}
% \end{itemize}
% \Cref{fig:framework} illustrates the core methodology of \textbf{v}isual \textbf{t}riple \textbf{u}nified \textbf{r}einforcement \textbf{l}earning system: \textit{Sample-Level Data Formatting}, \textit{Verifier-Level Reward Computation}, and \textit{Source-Level Metric Monitoring}.
% This unified framework enables joint training of visual reasoning and perception tasks through task-aligned design and reinforcement-based supervision. By sharing representations and gradients across tasks, the system promotes efficient learning and mutual enhancement between modalities.
%
% In contrast to research endeavors that define the reward computation as a fixed function, this work constructs a standalone reward server that interacts asynchronously with the RL training loop to generate reward signals for RL.
%
% There are several motivations for adopting a separate reward server rather than invoking reward functions inline within the training code.
%
%First, the reward design varies significantly across tasks; decoupling reward computation from the training code enhances modularity and extensibility, reducing the need to frequently modify core training logic.
%
% Second, this design supports flexible deployment—especially important when reward evaluation depends on GPU resources—so the server can be scaled independently from the training infrastructure.
%
% Third, this architecture improves maintainability and allows centralized management of reward computation as the number of supported tasks increases.
%
% Lastly, the server-based architecture enables distributed and asynchronous processing of rewards, which improves throughput and efficiency in multi-task RL settings.%
% The term \textit{verifier-level} refers to the granularity at which the rewards are computed.
%
% Rather than defining a monolithic reward function per task, reward computation is delegated to specialized verifiers, each responsible for handling a specific group of tasks.

% As illustrated in~\cref{fig:reward_server}, the reward server is implemented as a client-server architecture using FastAPI~\cite{ramirez_fastapi}.
%

% Each verifier is user-defined, containing custom functions to compute task-specific rewards. For instance, we implemented \textit{MathVerifyVerifier} for reasoning, OCR, and counting tasks and \textit{DetectionVerifier} for detection and grounding tasks.
%
% The former evaluates the correctness of answers enclosed in \verb|\boxed{}| as the accuracy reward.
%
% The latter computes both the IoU-based accuracy reward and the format reward for visual detection tasks, as introduced in ~\cref{subsec:rlvr}.
%
% This verifier-level design offers high flexibility and modularity. It simplifies adding new tasks and updating reward logic without modifying the core training pipeline.
%he verifier-level design offers high flexibility, enabling users to define diverse rule-based or model-based evaluators independently.
%
% This modularity allows the reward server to support new tasks and to flexibly accommodate changes in how model outputs are evaluated.
%
% It enables developers to update or replace reward logic without modifying the core training pipeline.

%
% Source-level metric monitoring is crucial because global metrics lack traceability in multi-task, multi-source training. By logging metrics per data source, we can identify data issues, enable targeted debugging, and analyze cross-source effects. This granular monitoring is vital in RL, known for potential instability (\cref{sec:training_recipe}).
%
% Monitoring metrics during training is essential for understanding model dynamics and diagnosing issues in real time.
%
% However, due to the presence of multiple tasks and data sources, aggregated metrics alone are insufficient.
%
% If a problem arises, global metrics provide no traceability.
%
% Monitoring only one task also fails, as data quality may vary across sources within the same task.

% To address this, we adopt source-level metric monitoring.
% %
% Each batch is grouped by the \texttt{data\_source} key defined in the data format, allowing per-source logging during training.
% %
% This design helps identify faulty or low-quality data sources early.
% %
% It also enables targeted debugging when performance anomalies are observed.
% %
% Further, it supports the comparison of learning progress across sources, revealing task-source interactions that may not be obvious from global metrics.%
% 
% Monitoring is especially important in RL, where training can be unstable and opaque.
% %
% A well-designed evaluation scheme is necessary to verify whether training is stable and whether the model behaves as expected.
% %
% Many off-the-shelf RL infrastructure offer comprehensive support for metric logging~\cite{sheng2024hybridflow,hu2024openrlhf}.
%  %
% We highlight several empirical signs of training stability in~\cref{sec:training_recipe}.
% 
% Additionally, we group and log reward values by data source to trace stability per input dataset.
% %
% For grounding and detection tasks, we also log source-specific IoU values at thresholds \{50, 75, 95, 99\} and mAP scores, offering fine-grained insight into convergence behavior.
% 
% To track model behavior during training, we draw inspiration from MAYE~\cite{maye} and monitor two categories: response length and reflection ratio.
% %
% For response length, we log 6 metrics:  the overall average, the average length of correct and incorrect responses, and truncation ratios for each.
% %
% Truncation rate measures how often model outputs hit the maximum length limit.
% %
% A high truncation rate can mean two things.%
% The model might be producing longer, thoughtful answers—for example, showing some cognition behaviors as  test-time scaling~\yan{cite ACT II} —or mode collapse where the model repeats uninformative content.
% %
% The actual cause should be judged by checking model output examples.%
% 
% For reflection rate, we follow~\yan{cita maye} and track the presence of 15 handpicked reflection-related words: \textit{[``re-check'', ``re-evaluate'', ``re-examine'', ``re-think'', ``recheck'', ``reevaluate'', ``reexamine'', ``reevaluation'', ``rethink'', ``check again'', ``think again'', ``try again'', ``verify'', ``wait'', ``yet'']}.
% %
% For each batch, we compute the ratio of responses containing these reflection words, the accuracy among those, and the accuracy of responses without them.
% %
% This logging reveals how reflective behavior correlates with correctness and helps identify overthinking or superficial answering patterns.
% %
% All these metrics are logged per data source to maintain consistency and enable cross-source comparison.


% In object detection and visual grounding, Intersection over Union (IoU) and mean Average Precision (mAP) are widely adopted evaluation metrics to quantify the overlap between predicted and ground-truth bounding boxes. While mAP integrates performance across multiple IoU thresholds, our experimental comparisons demonstrate that thresholded IoU provides a more direct and interpretable measure of prediction accuracy as shown in Figure\ref{fig:dyn_iou}a, with improved training stability. As a result, we adopt an IoU-based reward strategy for its robustness and clearer alignment with localization performance. As formalized in~\cref{eq:iou_rule}, we define a reward function based on thresholded IoU, where a prediction is considered successful only if its IoU exceeds a predefined threshold $\epsilon$. Conventionally, $\epsilon$ is set to 0.5, or averaged over a range of thresholds $[0.5, 0.95]$, as seen in classical computer vision papers and perception RL-VLM methods~\cite{liu2025visual,yu2025perception}.

% However, such loose thresholds can be suboptimal for VLM reinforcement learning, especially when compared to reasoning tasks that are evaluated by exact match criteria, as defined in~\cref{eq:math_rule}. Under relaxed thresholds, predictions with substantial localization errors may still yield high rewards, creating an inconsistency between perception rewards and strict verification criteria. Moreover, the presence of multiple predictions receiving identical rewards leads to reward ambiguity and unstable policy updates, characterized by elevated gradient clipping ratios and erratic gradient norms. This instability also negatively impacts out-of-distribution (OOD) generalization performance, as shown in~\cref{fig:dyn_iou}b.
% Loose thresholds may grant high rewards to poor predictions, introducing inconsistencies between tasks. Additionally, identical rewards for diverse predictions lead to ambiguity, unstable updates (e.g., high gradient clipping), and poor generalization to out-of-distribution data (\cref{fig:dyn_iou}b).
%
% This strict criterion enhances consistency between perception and reasoning signals and improves training stability. However, it introduces a cold-start problem in early rollouts, where most predictions receive zero reward—especially when using a pre-trained backbone without instruction tuning

==> 4_infra.tex <==
\section{Training Recipe}
\label{sec:training_recipe}
% %
% As discussed in the previous section, the three-level design enables the unification of perception and reasoning training.
% %
% It also provides flexibility for scaling across data, tasks, and verifiers.
% %
% In our early experiments, it is found that mixing these tasks for joint training led to instability.

% Several empirical signs are shared that help indicate whether training remains stable.
% %
% Common symptoms of instability include: 1) a decline in evaluation performance on online test data, 2) a sharp increase in gradient norm, often following a slow rise, 3) large fluctuations in entropy, and 4) a sudden surge in response length, particularly for incorrect samples.
% %
% When such patterns are observed, it usually suggests that the training process has encountered instability.%
% %
% The following section presents the challenges encountered and the efforts made to stabilize the training process.


V-Triune enables a scalable system of data, tasks, verifiers, and metrics as the foundation of training. However, early experiments revealed that joint training can lead to instability: (1) degraded evaluation performance, (2) sudden spikes in gradient norms, (3) large entropy fluctuations, and (4) abrupt increases in response length, particularly in incorrect outputs. We address training instability and scalability through targeted adjustments, including freezing ViT to prevent gradient explosion, filtering spurious image tokens, randomizing CoT prompts, and decoupling evaluation to manage memory during large-scale training.



\subsection{Disable ViT Training}

\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.98\linewidth]{images/disable_vit.pdf}
    \caption{\textbf{Analysis of ViT Training Instability.} (a) COCO testset (OOD) performance comparison. (b) Sum of gradient norms under different training schemes. (c) Layer-wise gradient norms of ViT and LLM during full parameter training. Notably, incorporating ViT training leads to a performance decline and highly unstable gradients; remarkably, ViT's gradients amplify during back-propagation, contrasting with the stable layer-wise gradients of the LLM.}
    \label{fig:disable_vit}
\end{figure}

% %
% During the initial experiments, full parameter training is employed, i.e., training ViT and LLM simultaneously.
% %
% However, no matter how the hyperparameters are adjusted, the performance of the detection task always collapses after several dozen steps.
% %
% By observing the experiment logs, it is found that the gradient norm during training is particularly large (> 1) and there are frequent spikes.
% %
% It is suspected that the cause of this phenomenon lies in the ViT.

% To verify this hypothesis, three experimental setups are designed: 1) Only LLM training; 2) Only ViT training; 3) Full parameter training.
% %
% Data from all tasks is mixed, and Qwen2.5-VL-7B is trained via RL with the exact same setup.
% %
% Three types of metrics are monitored: 1) Performance on the COCO test set (OOM); 2) Sum of gradient norms; 3) The trend of gradient changes in each layer during full parameter training (ViT+LLM).
% %
% As shown in,
% %
% First, from the COCO performance plot (\cref{fig:disable_vit}-a), it is observed that during full parameter training, performance starts to decline, while performance remains stable when only LLM is trained.
% %
% The performance of the ViT-only training remains largely unchanged, indicating that most of the performance improvement comes from RL incentivizing the LLM capabilities.
% %
% Additionally, from~\cref{fig:disable_vit}-b, it can be seen that even when only training ViT, the gradient norm is large (much higher than training with only the LLM, more than 10 times greater.).

% Upon careful examination of the gradients in each layer (\cref{fig:disable_vit}-c) during full parameters training, it is found that for LLM, the gradient norms of all layers remain stable during backpropagation, with the gradients of the last and first layers being nearly the same.
% %
% In contrast, the gradients of ViT increase during the backward pass.
% %
% The gradient of the 0th layer is 5-10 times larger than that of the last layer.
% %
% Such large gradients lead to instability, which worsens the vision capabilities of the VLM and, consequently, degrades the performance of the detection task.
% %
% At this point, it is confirmed that the source of the problem is ViT, so in subsequent experiments, ViT's parameters are frozen.


% As for the root cause of this phenomenon, it is believed to be an open problem that remains valuable for future research.
% %
% The following insights are shared here: 1) RL, as a post-training method, activates the VLM's capabilities while also aligning modalities, i.e., the model's responses are expected to be grounded in visual content.
% %
% When ViT and LLM parameters are trained together, the basic perception of visual content constantly changes, meaning the target to be aligned is continuously shifting.
% %
% This resembles the classic problem of Target Drift in machine learning~\yan{cite}, which leads to model collapse.
% %
% Future work may consider alternating training, as seen in GANs~\yan{gan}, where one model is frozen while the other is trained, and then the process is cycled.
% %
% 2) ViT's contrastive learning pretraining may make it difficult to utilize RL for post-training.
% %
% The contrastive learning pretraining of ViT results in a feature space that emphasizes static details, which does not fully align with the dynamic and causal understanding required for RL tasks, leading to poor post-training performance.
% %
% To address this issue, auxiliary self-supervised tasks can be introduced during the RL process to guide ViT in learning representations that better match the current RL task requirements.


In initial experiments, we performed full-parameter training by jointly optimizing the ViT and LLM. However, detection performance consistently collapsed after several dozen steps, regardless of hyperparameter settings. Log analysis revealed unusually large and spiking gradient norms (often >1), suggesting instability originating from the ViT. To verify this, we conducted three training configurations: (1) LLM-only, (2) ViT-only, and (3) full-parameter training, all using identical RL settings on Orsta-7B with mixed task data. We monitored: (a) COCO test set performance, (b) total gradient norm, and (c) layer-wise gradient trends during full-parameter training.

As shown in~\cref{fig:disable_vit}a, joint training leads to a performance drop, whereas LLM-only training maintains stable gains. ViT-only training yields minimal improvement, indicating that RL benefits primarily stem from updating the LLM. Figure~\cref{fig:disable_vit}b shows that ViT training produces significantly higher gradient norms—over 10× larger than LLM-only training.

Layer-wise analysis (\cref{fig:disable_vit}c) confirms this: LLM gradients remain stable across layers, while ViT gradients amplify during backpropagation, with the first layer exhibiting 5–10× larger norms than the last. This gradient explosion destabilizes training and undermines visual performance. Consequently, we freeze ViT parameters in subsequent experiments.

The root cause of this instability remains an open research question, but we offer two key insights. First, RL not only activates VLM capabilities but also enforces modality alignment by grounding responses in visual content. When ViT and LLM are trained jointly, the visual representation—i.e., the alignment target—shifts constantly, leading to instability analogous to the concept drift problem in machine learning~\cite{gama2014survey}. This dynamic target undermines stable optimization and may cause model collapse. Alternating training, similar to GANs~\cite{goodfellow2020generative}, where one component is frozen while the other is updated, could offer a solution. Second, ViT’s contrastive pretraining may limit its suitability for RL, as it encourages static, instance-level features rather than the dynamic and causal representations needed for RL tasks. To mitigate this mismatch, auxiliary self-supervised objectives could be introduced during RL to help ViT adapt to the evolving task demands.



% \subsubsection{Stability of VLM-RL training}

% Stability reflected by clip fraction of policy gradient and gradinet normalization. 


% \subsection{Recomputing Log-Probabilities with Conflicting Image Tokens and Features}
\subsection{Mitigating Spurious Image Special Tokens}
%

%  Red box: "vision\_end" token (end of image in query); orange box: generated thinking process; blue box: unexpected image token in generated sequence.

\begin{wrapfigure}[12]{tr}{0.55\textwidth} 
  \centering
  \vspace{-9pt}
  \begin{tcolorbox}[title=Sample,label={box:sample}]
  \includegraphics[width=\linewidth]{images/image_pad.png}
  \end{tcolorbox}
  \caption{\textbf{An Example of Spurious Image Tokens.}}
  \label{fig:image_token}
\end{wrapfigure}

To enable accurate advantage estimation, logits for both the query and the generated response are recomputed, as those returned by the inference engine may be imprecise. During the forward pass, image placeholders (highlighted in the red box in~\cref{fig:image_token}, appearing before the ``vision\_end`` token)
%
%
are replaced with visual features extracted by the ViT and adapter modules.
%
However, the model may mistakenly generate special tokens (highlighted in the blue box in Figure~\ref{fig:image_token}), such as image or video placeholders, that lack corresponding features—particularly under RL-zero settings. To ensure input–feature alignment and maintain training stability, a filtering step is applied to remove all such special tokens from the rollout sequence prior to recomputation.

% The recomputation of logits is performed to obtain more accurate logits for the query and generated response in order to estimate the advantages, as the logits returned by the inference engine may be imprecise. During the forward pass, the estimated number of image placeholders among the input tokens is replaced with actual image features extracted via the ViT and adapter modules. These placeholders are represented by special tokens in the tokenizer vocabulary. However, during generation, the model may generate image placeholder tokens, causing a mismatch between image tokens and the expected image features. To address this issue and maintain training stability, we add a filtering step that replaces generated image/video placeholder tokens with empty tokens, thereby preserving alignment between the input sequence and the corresponding image features.



\subsection{CoT Prompt Pool}
% %
% In the early stages of training for visual mathematics tasks, it is observed that the CoT prompt appended to the instructions (e.g., "Let's think step by step, place the answer in \verb|\boxed{}|") matter.
% %
% Even when the meanings are identical, variations in phrasing can impact the model's training dynamics, such as accuracy and response length.
% %
% To minimize the variance introduced by CoT prompt words, a CoT prompt pool is designed.
% %
% This pool contains 10 sentences with the same meaning as "Let's think step by step" and 10 sentences with the same meaning as "Place the answer in \verb|\boxed{}|."
% %
% During training, for each data sample, a random sentence from both the first and second groups in the pool is concatenated as the CoT prompt.
% %
% The benefit of this approach is that it helps reduce the impact of different prompt styles on training dynamics.
% %
% This Prompt Pool is applied to data where \texttt{MathVerifyVerifier} is used as the verifier.

In the early stages of training for visual mathematics tasks, variations in CoT prompts, despite conveying identical meanings, which can influence model performance, affecting metrics such as accuracy and response length. To reduce this variability, we construct a CoT prompt pool comprising 10 alternatives for “Let’s think step by step” and 10 for “Place the answer in \verb|\boxed{}|.” During training, one sentence from each group is randomly selected and appended to the instruction. This strategy mitigates prompt-induced variance and is applied specifically to samples verified with \texttt{MathVerifyVerifier}.





\subsection{System Memory Management}
V-Trinue is implemented atop Verl, a single-controller training framework that can approach system memory limits on the master node, particularly with large-scale vision datasets. To enable effective OOD performance monitoring, we introduce online test-set benchmarking at regular intervals. To mitigate the resulting system overhead, we decouple the testing phase from the main training loop and batch-process benchmarks, bypassing the default vLLM data handling. 
% These modifications enhance system stability at scale.


% \subsection{Lowering Learning Rate of Detection Task}
% During early training for detection tasks, performance is found to be highly sensitive to the learning rate. Learning rates above 1e-6 lead to declines in both training rewards and test accuracy. This issue is mitigated by lowering the learning rate; thus, all subsequent experiments adopt a learning rate of 1e-6 or lower.

% In the early stages of training for detection tasks, it is observed that the task is sensitive to the learning rate.
% %
% When the learning rate exceeds 1e-6, both the training reward and the test set accuracy decrease during training.
% %
% This issue is alleviated by reducing the learning rate.
% %
% Therefore, all subsequent experiments use a learning rate of 1e-6 or lower.




==> 5_experiment.tex <==
\section{Experiment}

% We conduct comprehensive experiments across multiple multimodal tasks to validate the effectiveness of our approach. \S~\ref{evaluation benchmarks} introduces the evaluation benchmarks, outlining the datasets used to rigorously assess our model's capabilities. \S~\ref{implementation details} details the implementation of Orsta, covering the selection of training data and experimental settings. In \S~\ref{main results}, we compare our method with the base model, demonstrating its enhanced performance in perception and reasoning. Finally, \S~\ref{ablation study} presents in-depth analyses and ablation studies to investigate the design choices and components of our approach.


% We adopt the Qwen2.5-VL~\cite{Qwen2.5-VL} series as the backbone model in our work. This architecture combines a LLM with a redesigned Vision Transformer (ViT), which incorporates 2D Rotary Position Embedding and windowed attention to enable efficient image encoding. To address the challenge of long visual feature sequences, a two-layer MLP-based merger is introduced. This module spatially compresses grouped image patches prior to alignment with the LLM’s text embeddings. Our experiments primarily utilize the 7B and 32B variants of the LLM, comprising 28 and 64 transformer layers, respectively. Both models share an identical ViT configuration with 32 layers and a patch size of 14. The models are trained on 4 trillion tokens during the multimodal pre-training stage, followed by supervised fine-tuning (SFT) on 2 million instances.




\subsection{Implementation Details}
\label{implementation details}


\noindent\textbf{Model:} We adopt Qwen2.5-VL-7B-Instruct and Qwen2.5-VL-32B-Instruct (0321 and 0326 versions, denoting their release dates) as our base models, which are trained on 4 trillion tokens during the multimodal pre-training stage, followed by supervised fine-tuning (SFT) on 2 million instances. They are chosen for their strong performance in vision-language reasoning and perception tasks.


\noindent\textbf{Framework and Hardware:} V-Triune is implemented on verl~\cite{sheng2024hybridflow}. We enable native FSDP for training and use vLLM for generation. All experiments are conducted on 64 NVIDIA H20 GPUs to meet the memory-intensive requirements of RL training.


% \subsection{Framework}
% We adopt the Verl (version 0.2.0.dev) framework\cite{} as our unified infrastructure for reinforcement learning (RL), which features a single controller and a hybrid execution paradigm. To orchestrate the distributed components, it employs Ray and actor management, integrated with a custom-designed unified data flow (as described in Sec.\ref{sec:main_method}) that spans the entire RL training pipeline. Specifically, we enable native Fully Sharded Data Parallel (FSDP) during training for efficient memory and compute utilization. For inference, we leverage vLLM to support high-throughput rolling out. A unified reward mechanism is adopted for reward computation, as described in Sec.\ref{sec:main_method}.


% \noindent\subsection{Hardware}
% Our experiments are conducted on a GPU cluster comprising 64 NVIDIA H20 GPUs, each equipped with 96GB of memory. Given the memory-intensive nature of inference workloads during the RL rollout phase, the H20 delivers strong performance, exhibiting only around a 10\% slowdown compared to an equivalent setup using H800 GPUs.

 % informative and appropriately challenging samples, we adopt a filtering strategy based on a \textit{pass@k} criterion, which discards instances that the base model can already solve reliably or finds overwhelmingly difficult. This enables more effective learning by concentrating on examples that offer meaningful reward reflection for both perception and reasoning. 







\subsubsection{Data Curation}
\label{subsec:data}
 
We select four reasoning tasks—Math, Puzzle, Science, and Chart—for their varied reasoning demands, and four perception tasks—Detection, Grounding, Counting, and OCR—for their broad coverage of visual understanding. Data sources for each task are listed below:

\begin{itemize}
    \item For the Math task, \texttt{mm\_math}~\cite{sun2024mm}, \texttt{geometry3k}~\cite{lu2021inter}, and \texttt{mmk12}~\cite{meng2025mm} are chosen.%
    \item For the Puzzle task, \texttt{PuzzleVQA}\cite{chia2024puzzlevqa} and \texttt{AlgoPuzzleVQA}\cite{ghosal2024algopuzzlevqa} are merged due to their shared origin, and \texttt{VisualPuzzles}~\cite{song2025visualpuzzles} is additionally included.%
\item For the Science task, \texttt{ScienceQA}~\cite{lu2022learn}, \texttt{SciVQA}~\cite{borisova2025scivqa}, and the ``Broader STEM Topics'' and ``(GradeSchool) Science'' categories from \texttt{ViRL39K}~\cite{wang2025vl} are used.%
    \item For the Chart task, \texttt{ChartQAPro}~\cite{masry2025chartqapro}, \texttt{ChartX}~\cite{xia2024chartx}, \texttt{Table-VQA}~\cite{kim2024tablevqa}, and the Tables/Diagrams/Charts categories from \texttt{ViRL39K}~\cite{wang2025vl} are used.%
    \item For the Detection task, \texttt{V3Det}~\cite{xie2023described} and \texttt{Object365}~\cite{shao2019objects365} are chosen.%
    \item For the Grounding task, \texttt{$D^3$}~\cite{xie2023described} is used.%
    \item For the Counting task, \texttt{CLEVR}~\cite{johnson2017clevr,tan2025reason} is used.%
    \item For the OCR task, English OCR questions are extracted from \texttt{LLaVA-OV Data}~\cite{li2024llava} and \texttt{EST-VQA}~\cite{wang2020general}.%
\end{itemize}

% We express our gratitude to the creators of these outstanding datasets for their invaluable contributions.
% %
To reduce noise, we apply a two-stage data filtering process (Figure~\cref{fig:data_curation}): (1) rule-based filtering and (2) difficulty-based filtering. This yields 47.7K high-quality samples across 18 datasets and 8 tasks. To mitigate dataset bias, puzzle data is duplicated to ensure sufficient coverage. The final corpus includes approximately \textbf{20.6K perception} and \textbf{27.1K reasoning} samples, primarily consisting of single-image, single-turn conversations.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{images/data_curation_v3.pdf}
    \caption{\textbf{Data Curation Process}. First, visual reasoning and visual perception data pass through a rule-based filter, which removes samples that do not meet preset criteria. Subsequently, the data enters a difficulty filter, which removes samples that are too easy or too hard based on model performance, ultimately producing the Curated Dataset.}
    \label{fig:data_curation}
\end{figure}

%
\paragraph{First Stage: Rule-based Filter} 
%
For the four visual reasoning tasks, the following filters are applied:
\begin{itemize}
    \item Multiple-choice and true/false questions that are prone to hacking are discarded.~\cite{kimiteam2025kimivltechnicalreport}
    \item Answers containing symbols such as ``='', ``['', ``]'', ``('', ``)'', and ``;'' are removed, as the absence of these symbols may cause answer mismatches even if the numeric values are correct.
    \item Answers longer than 20 characters are discarded to avoid overly complex answers.
\end{itemize}

% For the visual perception tasks, the filtering process is slightly more complex:
The filtering process for visual perception tasks involves additional complexity:
%
\begin{itemize}
    \item \textbf{Detection:} Following \texttt{Qwen2.5-VL}~\cite{Qwen2.5-VL}, data is converted to relative coordinates. Single-box samples contain one box per category, while multi-box samples retain original annotations. Samples with over 10 boxes per category or boxes exceeding 50\% of the image are removed. A 1:2 single-to-multi-box ratio is enforced, and category-level long tails are avoided.
    \item \textbf{Grounding:} Data is processed into relative coordinates, and data with a box size greater than 50\% of the image is discarded. Complex phrase labels are filtered out.%
    \item \textbf{Counting:} Data is balanced per category and only English data is retained.%
    \item \textbf{OCR:} Only English OCR data is retained, and final labels must be verifiable by \texttt{math\_verify}~\cite{mathverify2025}. Since no verifiable reward model (RM) is designed, the OCR task data must pass this validation.
\end{itemize}



\paragraph{Second Stage: Difficulty-based Filter}

% \begin{wrapfigure}[18]{tr}{0.5\textwidth} 
%   \centering
%   \includegraphics[width=\linewidth]{images/data_distribution.png}
%   \caption{\textbf{Training Data Distribution of 8 Tasks}} 
%   \label{fig:data_dist}
% \end{wrapfigure}

To remove low-value samples, easy questions already solvable by the base model are filtered out.

For reasoning tasks, we use \texttt{Qwen2.5-VL-32B-0321} to compute pass@8, retaining only samples with $0 \leq \text{pass@8} < 100\%$. For perception tasks, specifically detection and grounding, pass@16 is computed using \texttt{Qwen2.5-VL-7B} with a 0.5 IoU threshold, and samples with cumulative IoU rewards between 2 and 10 are selected.

All curated data is stored in Parquet format~\cite{parquet} and uniformly mixed for training without online filtering or curriculum scheduling. 
% Data distribution and post-filter statistics are shown in Figure~\ref{fig:data_dist} and Table~\ref{tab:training_data}, respectively.

% %
% Some easy questions may be covered by the base model's capabilities, offering little potential for learning. These should be filtered out.
% %
% For the four reasoning tasks, pass@8 accuracy is computed using \texttt{Qwen2.5-VL-32B-0321}, and only samples with $0 \leq \text{pass@8} < 100\%$ are retained.
% %
% For the perception tasks, \texttt{Qwen2.5-VL-7B} is used to compute pass@16 with an IoU reward threshold of 50.
% %
% Only samples with accumulated IoU rewards between 2 and 10 are retained.

% The curated data is finally packaged into Parquet format~\cite{parquet} and mixed together for training.
% %
% No online filtering process or specific curriculum learning order is implemented, and all data is mixed for training.
% %
% The overall data distribution is visualized in Figure~\ref{fig:data_dist}, and the post-processed statistics for each data source are summarized in Table~\ref{tab:training_data}.





% \begin{table}[htbp]
% \small
% \centering
% \caption{\textbf{Training Data Composition.}}
% % It comprises 18 publicly available datasets spanning 8 tasks. Puzzle-related data is duplicated to maintain the task balance, resulting in a total of 47.7K training samples.}
% \label{tab:training_data}
% \renewcommand{\arraystretch}{1.2}
% \begin{tabular}{c|c|cc}
% \toprule
% \textbf{Domain} & \textbf{Task} & \textbf{Dataset} & \textbf{Curated Training Samples} \\
% \midrule

% \multirow{13}{*}{Reasoning}
%   & \multirow{3}{*}{Math}    
%     & Geometry3K \cite{lu2021inter} & 2,539 \\
%   & 
%     & MMK12 \cite{meng2025mm} & 5,732 \\
%   & 
%     & MM\_Math \cite{sun2024mm} & 3,539 \\
%   \cline{2-4}
%   & \multirow{3}{*}{Science}  
%     & ScienceQA \cite{lu2022learn} & 536 \\
%   & 
%     & SciVQA \cite{borisova2025scivqa} & 1,264 \\
%   & 
%     & ViRL39K (stem) \cite{wang2025vl} & 2,539 \\
%   \cline{2-4}
%   & \multirow{4}{*}{Chart}    
%     & ChartQAPro \cite{masry2025chartqapro} & 498 \\
%   & 
%     & ChartX \cite{xia2024chartx} & 2,353 \\
%   & 
%     & TableVQA-Bench \cite{kim2024tablevqa}& 496 \\
%   & 
%     & ViRL39K (chart) \cite{wang2025vl} & 1,657 \\
%   \cline{2-4}
%   & \multirow{2}{*}{Puzzle}   
%     & PuzzleVQA \cite{chia2024puzzlevqa} & 2,648 \\
%   & 
%     & VisualPuzzles \cite{song2025visualpuzzles} & 342 \\
% \midrule

% \multirow{7}{*}{Perception}
%   & \multirow{2}{*}{Detection}  
%     & V3Det \cite{wang2023v3det} & 4,000 \\
%   & 
%     & Object365 \cite{shao2019objects365} & 4,000 \\
%   \cline{2-4}
%   & Grounding 
%     & $D^3$ \cite{xie2023described} & 4,870 \\
%   \cline{2-4}
%   & Counting  
%     & CLEVR \cite{johnson2017clevr,tan2025reason} & 1,725 \\
%   \cline{2-4}
%   & \multirow{2}{*}{OCR}    
%     & LLaVA-OV (OCR-en) \cite{li2024llava} & 3,092 \\
%   & 
%     & EST-VQA (en) \cite{wang2020general} & 2,946 \\

% \bottomrule
% \end{tabular}
% \end{table}



\subsubsection{Training Details} 

Two distinct RL training paradigms are explored: on-policy and off-policy. For both settings, the rollout batch size is fixed at 1024 across all experiments. The backward batch size is set to 1024 for on-policy and 128 for off-policy. All experiments use the GRPO algorithm, generating 8 candidate sequences per prompt.

To promote exploration while maintaining stability, we apply the clip-high strategy from DAPO~\cite{yu2025dapo} with clipping thresholds $\varepsilon_{\text{high}} = 0.28$ and $\varepsilon_{\text{low}} = 0.2$. This encourages low-probability token sampling without destabilizing training. No reference model is used; the final loss is computed solely via token-level mean PPO-clip loss.

To further stabilize learning, the ViT and connector modules remain frozen throughout. Learning rates are set to $1 \times 10^{-6}$ (on-policy) and $5 \times 10^{-7}$ (off-policy), with a 5\% warmup before being held constant. During rollout, we use the vLLM engine with a temperature of 1.0, top-$p$ of 1.0, and a maximum sequence length of 2048. Greedy decoding is applied during testing.

% \begin{table}[h!]
% \small
% \renewcommand{\arraystretch}{1.5}
% \centering
% \caption{\textbf{Hyper-parameter Settings for Training Variants.}}
% \setlength{\tabcolsep}{6mm}
% \label{tab:rl_settings}
%     \begin{tabular}{cccccc}
%     \toprule
%     \textbf{Setting} & \textbf{Rollout Batch Size} & \textbf{Rollout N} & \textbf{PPO Batch Size} & \textbf{Learning Rate}\\ 
%     \midrule
%     On-Policy   &  1024  &  8  &  1024  &  1e-6    \\
%     Off-Policy  &  1024  &  8  &  128    &  5e-7    \\
%     \bottomrule
%     \end{tabular}
% % \vspace{0.5em}
% \end{table}


\subsubsection{Evaluation Benchmarks}
\label{evaluation benchmarks}

% The evaluation of downstream capabilities in vision-language models (VLMs) relies on a comprehensive suite of benchmarks that assess a wide range of skills. MEGA-Bench~\cite{chen2024mega} features over 500 real-world tasks encompassing diverse modalities and use cases, making it a cornerstone for general-purpose VLM evaluation. For domain-specific and knowledge-intensive reasoning, MMMU~\cite{yue2024mmmu} challenges models with expert-level, multidisciplinary questions, while MathVista~\cite{lu2023mathvista} focuses on mathematical problem-solving within visual contexts. Specialized perception and grounding abilities are assessed by benchmarks such as ScreenSpot-Pro~\cite{li2025screenspot}, which targets UI element localization in professional software interfaces; CountBench~\cite{paiss2023teaching}, which measures object counting accuracy; and OCRBench v2~\cite{fu2024ocrbench}, which evaluates text localization, extraction, and reasoning in visual scenes. Traditional benchmarks like COCO~\cite{lin2014microsoft} remain essential for object detection and are often adapted for VLM tasks, whereas OVDEval~\cite{yao2023evaluate} extends this to open-vocabulary detection and grounding, emphasizing nuanced semantic understanding. To push the limits of current models, highly challenging benchmarks such as ZeroBench~\cite{roberts2025zerobench} and OlympiadBench~\cite{he2024olympiadbench} include tasks that are nearly infeasible for today’s VLMs, offering rigorous evaluations of robustness, generalization, and areas in need of further advancement.

To comprehensively assess the model’s capabilities, we evaluate performance across three domains: real-world tasks, visual reasoning, and visual perception.

For real-world task evaluation, we employ the core subset of \textbf{MEGA-Bench}~\cite{chen2024mega}, which consists of 440 diverse, long-tailed tasks encompassing over 6,000 expert-curated samples. All results are reported using the official MEGA-Bench evaluation implementation to ensure consistency.

To evaluate reasoning and knowledge capabilities, we adopt \textbf{MMMU}\cite{yue2024mmmu} and \textbf{MathVista}\cite{lu2023mathvista}. Both benchmarks are assessed using VLMEvalKit with default prompts (i.e., without Chain-of-Thought) and inference settings. Since GPT-4o is used for both answer extraction and scoring—which may introduce variability—we report both rule-based and GPT-4o-based scores for MMMU.

%
For visual perception evaluation, we include \textbf{COCO} (val-2017)\cite{lin2014microsoft}, \textbf{OVDEval}\cite{yao2023evaluate}, \textbf{CountBench}\cite{paiss2023teaching}, \textbf{OCRBench} (v2)\cite{fu2024ocrbench}, and \textbf{ScreenSpot-Pro}~\cite{li2025screenspot}. We report both IoU and mAP for COCO and OVDEval. Notably, mAP and NMS-mAP are computed as the mean of sample-level metrics, rather than over the entire dataset, due to the absence of confidence scores in model outputs. These benchmarks are evaluated using simple task-specific queries, with examples provided below. OCRBench is evaluated using LMMs-Eval\cite{zhang2024lmmsevalrealitycheckevaluation} on the entire dataset, encompassing both English and Chinese samples. ScreenSpot-Pro is assessed with its official evaluation code, using instruction-style English prompts, positive ground truth, and all task types. All bounding boxes and keypoints are represented using coordinate values relative to the original input image dimensions.
%
\begin{figure}[tb!]
  \centering
  \begin{tcolorbox}[title=Query Example of Detection and Grounding]
  \begin{lstlisting}[basicstyle=\ttfamily\small, breaklines=true, numbers=none]
Please detect all instances of the following category within the image:
{LABEL}. 

Let's think step by step and output the final answer in <answer> and </answer> tags.
For example:
Your detailed reasoning process here.
<answer>
[{'bbox_2d': [x1,y1,x2,y2],'label': label_name}]
</answer>
  \end{lstlisting}
  \end{tcolorbox}
  \caption{\textbf{Example query format for detection and grounding tasks.} The query instructs VLMs to identify instances of a given object and format the output in a specific reasoning-answer format.}
  \label{fig:det_sample}
\end{figure}
%
% \begin{figure}[tb!]
%   \centering
%   \begin{tcolorbox}[title=Query Example of Detection and Grounding]
%   \begin{minted}[fontsize=\small, breaklines]{text}
% Please detect all instances of the following category within the image:
% {LABEL}. 
% 
% Let's think step by step and output the final answer in <answer> and </answer> tags.
% For example:
% Your detailed reasoning process here.
% <answer>
% [{'bbox_2d': [x1,y1,x2,y2],'label': label_name}]
% </answer>
%   \end{minted}
%   \end{tcolorbox}
%   \caption{\textbf{Example query format for detection and grounding tasks.} The query instructs VLMs to identify instances of a given object and format the output in a specific reasoning-answer format.}
%   \label{fig:det_sample}
% \end{figure}



% \subsubsection{Visual Reasoning}We utilize MMMU and MathVista for evaluation. MathVista is utilized to evaluate model's capabilities in mathematical reasoning within visual contexts. MMMU provides a comprehensive evaluation across 30 college-level disciplines, emphasizing both subject-specific knowledge and deliberate multimodal reasoning. 

% \subsubsection{Visual Perception}We evaluate the model’s perceptual capabilities using several benchmarks. For open-vocabulary object detection, we use COCO (val2017 subset) and OVDEval to test its ability to localize and classify both seen and unseen objects in natural scenes. For visual grounding, RefCOCO is used for natural images, and ScreenSpot-Pro for structured user interfaces, evaluating both free-form and layout-constrained referring expressions. For OCR, we employ OCRBenchv2 that spans 31 diverse scenarios to comprehensively evaluate the model’s capacity for fine-grained multimodal text comprehension. For visual counting, we use CountBench and Super-CLEVR, which focus on object counting in diverse visual scenes.


    % \caption{\textbf{Performance Comparison on Real-World Tasks - MEGA-Bench}. We present a comparative analysis of general-purpose and reasoning-oriented VLMs with approximately 7B and 32B parameters. Models with enhanced reasoning capabilities are denoted by \faLightbulb[regular]. The final column reports the overall MEGA-Bench Core score, calculated as a weighted average of the preceding task categories. Notably, the QwenVL-2.5-32B-0321 model contains known issues that are resolved in the subsequent 0326 version. All scores are reproduced using the official MEGA-Bench evaluation code, except for Gemma3-27B (marked with $\dagger$).}
  \begin{table}[ht!]
    \small
    \renewcommand{\arraystretch}{1.5}
    \centering
    \caption{\textbf{Performance of Orsta on MEGA-Bench core}. Comparison of general-purpose and reasoning-enhanced VLMs (7B+ \& 32B+). Models with improved reasoning are marked by \faLightbulb[regular]; final scores are reported as weighted averages. QwenVL-2.5-32B-0321 has known issues, which are resolved in the 0326 version. All results are obtained using the official MEGA-Bench evaluation code, except for Gemma3-27B ($\dagger$).}
    \setlength{\tabcolsep}{0.8mm}
    \scalebox{0.88}{
        \begin{tabular}{l|cccccccc|c}
            \toprule 
            Model                                                & Knowledge    & Mathematics    & Perception    & Coding         & Info. Ex.     & Planning      & Science       & Metrics       &  \makecell{MEGA-Bench \\ Core} \\
            \midrule
            \multicolumn{10}{c}{7B+ Model}  \\ \midrule
            
            QwenVL-2-7B                                           & 39.96         & 25.95         & 39.99         & 31.49         & 40.29         & 16.64         & 28.59         & 43.61         & 34.47 \\
            QwenVL-2.5-7B                                         & 38.84         & 27.67         & 41.24         & 28.93         & 50.23         & 16.32         & 36.75         & 41.64         & 35.07 \\ 
            InternVL-3-8B                                         & 36.64         &\textbf{32.75} & 42.17         &\textbf{35.11} & 48.92         & 14.35         & 36.51         &\textbf{53.94} & 36.48 \\
            Gemma3-12B                                            & 41.11         & 29.10         & 37.38         & 30.27         & 46.56         & 16.10         & 36.83         & 50.40         & 35.04 \\
            Kimi-VL-A3B                                           & 37.63         & 27.07         & 39.50         & 22.30         & 40.99         &\textbf{22.17} & 33.94         & 46.65         & 34.40 \\
            MM-Eureka-7B \faLightbulb[regular]                    & 40.12         & 31.59         & 39.71         & 28.75         & 49.32         & 16.64         & 37.25         & 46.39         & 35.96 \\
            VL-Rethinker-7B \faLightbulb[regular]                 & 40.65         & 30.08         & 42.02         & 29.87         & 52.03         & 17.83         & 36.82         & 46.90         & 37.25 \\ 
            Kimi-VL-A3B-Thinking  \faLightbulb[regular]           & 33.45         & 17.76         & 28.11         & 14.69         & 41.14         & 12.64         & 28.60         & 43.97         & 27.08 \\
            \hline
            \textbf{Orsta-7B (Ours) \faLightbulb[regular]}        &\textbf{41.65} & 31.48         &\textbf{43.84} & 32.82         &\textbf{54.07} & 17.83         &\textbf{36.91} & 41.66         &\textbf{38.31} \\  
            
            \rowcolor{blue_light_1}
            $\triangle$ (Ours - Backbone)                         & +2.8          & +3.8         & +2.6          & +3.9           & +3.8          & +1.5          & +0.2          & +0.0          & +3.2   \\
            \midrule \midrule
            
            \multicolumn{10}{c}{32B+ Model}  \\ \midrule
            QwenVL-2.5-32B-0321                                   & 8.48          & 12.62         & 11.99         & 13.59         & 15.44         & 8.61          & 16.78         & 14.91         & 11.87 \\ 
            MM-Eureka-32B     \faLightbulb[regular]               & 12.20         & 20.19         & 21.88         & 15.86         & 21.23         & 15.47         & 19.95         & 22.77         & 18.57 \\
            VL-Rethinker-32B   \faLightbulb[regular]              & 12.16         & 28.09         & 22.99         & 11.89         & 21.50         & 15.09         & 28.10         & 15.73         & 19.41 \\
            \hline
            \textbf{Orsta-32B-0321 (Ours) \faLightbulb[regular]}  &\textbf{21.33} &\textbf{28.55} &\textbf{32.23} &\textbf{19.44} &\textbf{26.38} &\textbf{17.78} &\textbf{33.20} &\textbf{24.18} &\textbf{25.94} \\
            \rowcolor{blue_light_1}
            $\triangle$ (Ours - Backbone)                         & +12.9         & +15.9         & +20.2         & +5.9          & +10.9         & +9.2         & +16.4         & +9.3           & +14.1 \\
            \midrule
            
            Gemma3-27B $\dagger$                                  & 49.43         & 42.20         & 45.46         & 40.18         & 49.30         & 24.96         & 47.08         & 58.99         & 41.82 $\dagger$  \\
            QwenVL-2.5-32B-0326                                   & 46.09         & 32.04         & 47.55         & 38.36         & 61.65         & 28.43         & 37.55         & 50.38         & 43.67 \\  
            InternVL-3-38B                                        & 46.32         &\textbf{40.29} &\textbf{55.05} &\textbf{45.29} & 56.63         & 22.88         &\textbf{52.04} &\textbf{58.04} &\textbf{46.69} \\
            Skywork-R1V-38B \faLightbulb[regular]                 & 25.59         & 28.45         & 22.95         & 19.88         & 19.53         & 9.74          & 22.64         & 37.55         & 21.54 \\
            Skywork-R1V2-38B \faLightbulb[regular]                & 17.08         & 12.38         & 15.65         & 7.14          & 9.90          & 17.60         & 14.29         & 0.0           & 15.39 \\
            \hline
            \textbf{Orsta-32B-0326 (Ours) \faLightbulb[regular]}  &\textbf{46.78} & 37.43         & 50.86         & 38.92         &\textbf{63.14} & 28.05         & 42.68         & 53.01         & 45.78 \\ 
            \rowcolor{blue_light_1}
            $\triangle$ (Ours - Backbone)                         & +0.7           & +5.4          & +3.3          & +0.6           & +1.5          & -0.4         & +5.1         & +2.6           & +2.1  \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:main_results}
\end{table}
%
\subsection{Performance}
%
\subsubsection{MEGA-Bench}
%
A comprehensive comparison of Orsta against its backbone and leading general-purpose/reasoning-enhanced VLMs is available in~\cref{tab:main_results}.
%
Orsta shows consistent gains at both 7B and 32B scales: Orsta-7B achieves 38.31 (+3.2) on MEGA-Bench Core, and Orsta-32B reaches 45.78 (+2.1).
%
Our method V-Triune notably boosts performance in domains with enriched training data—mathematics (+3.8 at 7B, +5.4 at 32B), perception, planning, and science—indicating strong generalization in both reasoning and perception tasks. In contrast, coding and metric-related tasks show limited improvement due to sparse supervision, underscoring the targeted scalability of our unified RL training approach.


\cref{fig:mega_performance_track} shows the MEGA-Bench performance trajectories of three Orsta variants (7B, 32B-0321, 32B-0326) under on-policy and off-policy RL. All variants exhibit stable improvement, with on-policy training generally outperforming off-policy. The 7B model shows smoother and more pronounced gains, while the 32B models experience slower or more variable progress, indicating increased optimization challenges at larger scales.


Qwen2.5-VL-0321, a publicly released checkpoint, exhibits known issues in perception and output formatting but performs reliably in reasoning tasks, as confirmed by our evaluations and VL-Rethinker~\cite{vl_rethinker}. These issues are addressed in the subsequent 0326 release. We regard the 0321 version as a clean baseline with core knowledge capabilities. As shown in~\cref{fig:32b_details}, Orsta-32B-0321 demonstrates that reinforcement learning primarily enhances existing model strengths, serving as an alignment mechanism rather than introducing new capabilities. Performance gains are most notable in in-domain tasks—mathematics, perception, science, and planning, while out-of-domain tasks like coding see limited improvement, underscoring RL’s alignment-focused impact.

In summary, our results demonstrate that reinforcement learning effectively enhances both visual reasoning and perception within a unified framework. RL consistently improves performance across MEGA-Bench core’s 440 diverse tasks, supporting its role as a general-purpose alignment strategy that unlocks latent capabilities in pretrained vision-language models.

% Qwen2.5-VL-0321 is a publicly released checkpoint known to exhibit irregularities in perception-related tasks and output formatting, while maintaining reliable performance in reasoning domains—as verified by both our and the VL-Rethinker benchmarks~\cite{vl_rethinker}. These issues are resolved in the later Qwen2.5-VL-0326 release. Therefore, we consider Qwen2.5-VL-0321 to reflect a pure baseline with basic knowledge ability. Figure~\ref{fig:32b_details} illustrates the task-level training dynamics of Orsta-32B-0321 across MEGA-Bench Core. Reinforcement learning (RL) appears to amplify capabilities already present in the base model, acting more as an alignment tools rather than constructing new competencies from scratch. Notably, in-domain tasks such as mathematics, perception, science, and planning demonstrate more pronounced performance gains compared to out-of-domain tasks like coding, highlighting the alignment-driven nature of RL fine-tuning.

% In summary, our experimental findings show that reinforcement learning in VLMs can effectively benefit both visual reasoning and visual perception tasks in a unified framework. RL consistently boosts performance across the MEGA-Bench Core’s 440 diverse real-world tasks, suggesting its broad applicability for enhancing vision-language models. This supports the hypothesis that RL serves as a general-purpose alignment strategy that can unlock latent capabilities in pretrained vision-language models across heterogeneous task domains.


\begin{figure}[t]
    \centering
        \begin{subfigure}{0.32\textwidth}
            \includegraphics[width=\linewidth]{images/figure3/7b.pdf}
        % \caption{Model 7B}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.32\textwidth}
            \includegraphics[width=\linewidth]{images/figure3/32b_0321.pdf}
        % \caption{Model 32B}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\linewidth]{images/figure3/32b_0326.pdf}
        % \caption{Orsta}
        \end{subfigure}
    \caption{\textbf{Training Trends of On-Policy vs Off-Policy Across Three Model Variants on MEGA-Bench core (7B, 32B-0321, 32B-0326)}.
Models are evaluated every 5 steps from step 0 to 135. Starting points and peak performances are annotated on the curves.}
    \centering
    \label{fig:mega_performance_track}
\end{figure}

\subsubsection{Common Downstream Tasks}
%
\begin{wrapfigure}[22]{tr}{0.350\textwidth} 
  \centering
  \vspace{-5pt}
  % \hspace{-10mm}
  \includegraphics[width=\linewidth]{images/figure3/32b_0321_details.pdf}
  \vspace{0pt}
  \caption{\textbf{Training Trends of Orsta-32B-0321 on MEGA-Bench core.} The dark line denotes the overall MEGA-Bench Core, linking to the performance shown in~\cref{fig:mega_performance_track}.} 
  \label{fig:32b_details}
\end{wrapfigure}
%
As shown in~\cref{tab: downstream_result}, on the general knowledge benchmark MMMU, Orsta outperforms its backbone by ~4\% at 7B and ~1\% at 32B-0326. On the math-focused MathVista benchmark, it achieves over 5\% gains across all model sizes. These results align with improvements seen on math tasks in MEGA-Bench, reinforcing Orsta’s strength in enhancing reasoning capabilities. 

Orsta consistently improves visual perception across benchmarks. On COCO detection, Orsta-7B achieves notable gains (+7.81 mAP and +12.17 mAP@50 for single-object; +3.77 mAP and +5.48 mAP@50 for multi-object), with stronger gains in simpler scenarios. Orsta-32B-0321 shows marked improvements, addressing prior perception issues, while Orsta-32B-0326 yields ~+3\% mAP gains across both subsets. On OVDEval, Orsta-7B and 32B improve by +5.3 and +3.5 mAP, validating the dynamic IoU reward. GUI and OCR tasks (ScreenSpot-Pro, OCRBench) show consistent 1–2\% gains. CountBench sees the most significant boost, with Orsta-7B outperforming 32B SFT models and Orsta-32B setting a new state of the art. Overall, V-Triune delivers greater perception improvements for less-aligned base models (0321) than for already-instructed ones (0326).



\begin{table}[t]
    \small
    \renewcommand{\arraystretch}{1.5}
    \centering
    \caption{\textbf{Benchmarking Orsta Against Baselines on Common Visual Reasoning and Perception Tasks}. For COCO, we report both mAP and mAP@50 as evaluation metrics (mAP|mAP@50), while OVDEval is evaluated using NMS-AP (task-wide mAP). Accuracy serves as the evaluation metric for all remaining tasks.}
    \setlength{\tabcolsep}{1.0mm}
    \scalebox{0.9}{
       \begin{tabular}{lcccccc}
            \toprule 
            % \multirow{2}{*}{Tasks} & \multicolumn{2}{c}{7B}           & \multicolumn{4}{c}{32B}     \\
            Tasks       & QwenVL-2.5-7B          & \textbf{Orsta-7B }       & \makecell{QwenVL-2.5-32B\\0321}      & \makecell{\textbf{Orsta-32B}\\0321}       & \makecell{QwenVL-2.5-32B\\0326}     & \makecell{\textbf{Orsta-32B}\\0326} \\
            \midrule
            \multicolumn{7}{c}{Visual Reasoning}  \\ 
            \midrule
            MMMU$_{val, rule}$      & 45.56          & 49.70          & 37.11          & 34.67          & 39.22         & 38.00 \\ 
            MMMU$_{val, model}$     & 54.40          & 57.10          & 60.80          & 64.11          & 64.20         & 64.78 \\
            MathVista$_{testmini}$  & 67.50          & 72.50          & 70.80          & 76.30          & 73.40         & 76.40 \\
            \midrule
            \multicolumn{7}{c}{Visual Perception} \\ 
            \midrule
            COCO$_{single}$         & 35.02 | 62.26  & 42.83 | 74.43  &  12.19  |  21.43      &    31.64   |   53.44     &   40.26   |  68.07     &    42.12   |    71.55   \\  
            COCO$_{multiple}$       & 59.59 | 74.74  & 63.36 | 80.22  &    1.61   |    2.00    &   50.32    |    63.33    &   62.80    |   78.75    &   64.28    |     81.19     \\
            OVDEval                 & 52.23          &  57.52              & 3.84               &  35.65              &  56.80             &  60.36              \\
            ScreenSpot-Pro          & 22.71          & 23.91          & 49.46          & 50.98          & 51.23         & 52.69  \\
            CountBench              & 71.69          & 82.28          & 83.71          & 88.59          & 83.91         & 88.19  \\     
            OCRBenchv2                & 55.11          & 56.05          & 44.85          & 43.78          & 58.14         & 59.09  \\
            \bottomrule
        \end{tabular}
    }
    \label{tab: downstream_result}
\end{table}



\subsection{Training  Metric Analysis}
%   1. Training reward. soure
%   2. Length (x6）
%   3. Reflection ratio 有些任务没有反思
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.90\linewidth]{images/train_analysis.pdf}
    \caption{Training dynamics of response length (top row), reflection ratio (middle row), and correct ratio in reflection responses (bottom row) during training steps for Math (MMK12), Puzzle (PuzzleVQA), Detection (V3Det), and OCR (estvqa) tasks using the Orsta-32B-0321 off-policy setting. Each column corresponds to a different task, and each row represents a distinct metric.}
    \label{fig:train_analysis}
\end{figure}
% %
% V-Truine's Source-level Metric Monitoring enables a detailed analysis of training metrics.
% %
% Of particular interest are the cognitive behaviors learned by the model during the training process, such as reflection patterns.
% %
% Specifically, it is investigated whether visual perception tasks, such as detection, can achieve test-time scaling through a long Chain-of-Thought (CoT) format, similar to reasoning tasks.
% %
% Consequently, the experimental logs from the Orsta-32B-0321 off-policy setting are selected for analysis, as this experiment exhibits a notable increase in response length, which aids in observing changes in reflective behaviors.

% For this analysis, visual reasoning tasks, specifically Math (MMK12) and Puzzle (PuzzleVQA), and visual perception tasks, namely Detection (V3Det) and OCR (estvqa), are selected, with one data source chosen for each respective task.
% %
% Three metrics are reported: response length, reflection ratio, and correct ratio in reflection responses, as previously introduced in~\cref{subsec:metric_monitoring}.


V-Triune’s source-level metric monitoring enables detailed analysis of cognitive behaviors learned during training, such as reflection patterns. To explore whether perception tasks can benefit from test-time scaling via extended CoT, we analyze Orsta-32B-0321 off-policy logs, which show a marked increase in response length. The analysis focuses on four tasks—Math (MMK12), Puzzle (PuzzleVQA), Detection (V3Det), and OCR (estvqa)—each represented by a single dataset. We report three key metrics: response length, reflection ratio, and accuracy of reflection responses, as defined in~\cref{subsec:metric_monitoring}.


\cref{fig:train_analysis} shows the evolution of key metrics across training steps for the selected tasks. Reasoning tasks (Math and Puzzle) consistently exhibit higher response lengths and reflection ratios than perception tasks (Detection and OCR). For reasoning tasks, response length generally increases over time, with Puzzle showing a steady rise and Math displaying more fluctuation. Among perception tasks, OCR also shows a clear upward trend in response length, while Detection initially decreases before stabilizing around a mean of ~325 tokens, without a clear upward trajectory.


The middle row of \cref{fig:train_analysis} shows a clear increase in reflection ratios for Math and Puzzle, indicating a growing use of reflective steps during training. OCR also exhibits an upward trend, though with greater variability. In contrast, Detection maintains a consistently low reflection ratio, near zero, suggesting little engagement in reflective reasoning. In the bottom row, the correctness of reflection responses improves steadily for Puzzle and gradually for OCR, rising from ~0.4 to ~0.7–0.8. Math shows fluctuating correctness between ~0.3 and ~0.7, without a clear trend but indicating partial effectiveness. Detection, however, remains at zero throughout, reflecting the absence or failure of reflective responses.

Overall, reasoning tasks and OCR demonstrate increasing reflection usage and, to varying degrees, improved reflection quality. Detection diverges from this pattern, showing minimal reflective behavior and no apparent benefit from longer, reasoning-style responses.


% \cref{fig:train_analysis} presents the dynamics of these metrics throughout the training process, measured in steps, for the selected tasks.
% %
% It should first be noted that the response lengths and reflection ratios for reasoning tasks (Math and Puzzle) are considerably higher than those for perception tasks (Detection and OCR) throughout the training period.
% %
% Observing the top row, the response length for the reasoning tasks, Math (MMK12) and Puzzle (PuzzleVQA), generally shows an increasing trend as training progresses, although Math (MMK12) exhibits more fluctuations.
% %
% Similarly, the OCR (estvqa) task, a visual perception task, also demonstrates a noticeable increase in response length over the training steps.
% %
% In contrast, the Detection (V3Det) task displays a different pattern for response length; after an initial decrease, it stabilizes and fluctuates around a mean value of approximately 325, without a clear overall increasing trend.

% Turning to the middle row, the reflection ratio for both Math (MMK12) and Puzzle (PuzzleVQA) displays a clear upward trajectory, indicating an increased tendency for reflective steps as training advances.
% %
% The OCR (estvqa) task also shows an increasing trend in its reflection ratio, though it is more volatile compared to the Puzzle (PuzzleVQA) task.
% %
% However, for the Detection (V3Det) task, the reflection ratio remains consistently low, fluctuating close to zero throughout the training steps, suggesting minimal engagement in reflective processing.
% %
% Finally, the bottom row illustrates the correct ratio in reflection responses.
% %
% For the Puzzle (PuzzleVQA) task, this ratio shows a discernible improvement over training, suggesting that the model becomes more effective when it employs reflection.
% %
% The OCR (estvqa) task also exhibits a general, albeit fluctuating, upward trend in the correctness of its reflection responses, starting from around 0.4 and reaching towards 0.7-0.8.
% %
% In the Math (MMK12) task, the correct ratio in reflection responses fluctuates significantly between approximately 0.3 and 0.7, without a clear monotonic improvement, but indicates that a substantial portion of reflections can be correct.
% %
% Most notably, the correct ratio in reflection responses for the Detection (V3Det) task is consistently zero.
% %
% This, combined with its very low reflection ratio, strongly suggests that the model either does not generate reflection responses for detection, or any such attempts are entirely incorrect.

% %
% In summary, building on this baseline observation, the reasoning tasks (Math and Puzzle) and the OCR perception task demonstrate an increasing propensity for longer responses and higher reflection ratios with training, with varying degrees of improvement in the correctness of these reflections.
% %
% The Detection task, however, does not exhibit these characteristics, indicating a different learning behavior that does not seem to involve or benefit from an extended reflective process in the same manner.
%
\subsection{Ablation Study}
\label{ablation study}

\begin{figure}[t]
    \centering
        \begin{subfigure}{0.32\textwidth}
            \includegraphics[width=\linewidth]{images/figure6/7b_strategy.pdf}
        % \caption{Model 7B}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.32\textwidth}
            \includegraphics[width=\linewidth]{images/figure6/7b_task.pdf}
        % \caption{Model 32B}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.32\textwidth}
                \includegraphics[width=\linewidth]{images/figure6/32b_lr.pdf}
        % \caption{Orsta}
        \end{subfigure}
    \caption{\textbf{Ablation Study on Training Strategies (a), Task Composition (b), and Learning Rates (c).}(a) Various training strategies evaluated on the 7B model (LLM-only, ViT-only, joint training); (b) Different task compositions evaluated on the 7B model (reasoning, perception, or both); (c) Effects of learning rates (1e-6, 1.5e-6, 2e-6, 3e-6) on the performance of the 32B model. Each subfigure shows the score progression over training steps.}
    \centering
    \label{fig:abaltaion_study}
\end{figure}
%
% \subsubsection{1. training llm, training vit, training full: MEGABench track.}
% \subsubsection{2. reasoing only + perception only: MEGABench track}
% \subsubsection{3. 32B learning rate: MEGABench track}

\noindent\textbf{Training-strategy ablation}
As shown in~\cref{fig:abaltaion_study}a, updating only the LLM stack raises the score from approximately 35 to 38 by step 120, indicating that reasoning weights are the primary driver of performance improvement. In contrast, tuning only the vision backbone results in negligible gains, with scores plateauing around 35.5. When both branches are optimized jointly, performance initially mirrors the LLM-only trajectory but slightly surpasses it in later stages (peaking at approximately 38.5).

\noindent\textbf{Task-composition ablation}
Training on both reasoning and perception data yields the strongest performance, reaching approximately 37.5. A reasoning-only curriculum closely trails (within 0.3 points) and briefly surpasses it mid-training, suggesting that the benchmark prioritizes logical competence over pure perception. Perception-only training consistently lags by 0.7–1.0 points but still shows steady improvement, indicating that visual supervision provides transferable alignment signals. The consistent performance hierarchy (Reasoning+Perception > Reasoning > Perception) underscores the value of mixed-task corpora: combining complementary signals leads to additive gains rather than diluted optimization.

\noindent\textbf{Learning-rate ablation}
For the Orsta-32B model, conservative step sizes are essential. A learning rate of 1e-6 yields the highest and most stable plateau (45.5), while 1.5e-6 performs similarly until a mild degradation after 80 steps. Increasing the rate to 2e-6 causes a late-stage collapse to ~38, and 3e-6 diverges catastrophically after 50 steps, dropping below 36. This pattern suggests that larger models sit closer to the edge of the loss landscape, benefiting from small, stable updates, with 1e-6 offering the best trade-off between convergence speed and final performance on MEGABench.


% We present a comprehensive comparison of Orsta against both its backbone and a range of general-purpose and reasoning-enhanced vision-language models (VLMs) in~\cref{tab:main_results}. Orsta consistently outperforms prior models across both the 7B and 32B parameter regimes. Specifically, Orsta-7B achieves a MEGA-Bench Core score of 38.31, representing a +3.2 improvement over its backbone, while Orsta-32B reaches 45.77, marking a +2.6 gain. These results highlight Orsta’s effectiveness in boosting performance across diverse visual-language tasks. Notably, our reinforcement learning (RL) training brings significant gains in domains where our training data is most enriched—mathematics (+3.8 at 7B, +5.4 at 32B), perception, planning, and science—demonstrating strong generalization in both reasoning and perception categories. In contrast, modest or negligible changes are observed in coding and metrics, where less task-specific supervision was provided.These findings underline the targeted scalability of our unified RL training strategy across both model sizes and task domains.

% Figure~\ref{fig:mega_performance_track} illustrates the performance trajectories of three Orsta variants (7B, 32B-0321, and 32B-0326) on MEGA-Bench under both on-policy and off-policy RL paradigms. Across all settings, Orsta demonstrates a consistent upward trend, indicating stable training and effective performance enhancement. Notably, the performance gap between on-policy and off-policy training varies across model sizes, with on-policy generally yielding better results. Interestingly, the smaller 7B model exhibits smoother and more substantial performance gains, while the larger 32B models show slower or more fluctuating improvements, suggesting that scaling up model size may introduce greater optimization challenges. 

% On the general knowledge benchmark MMMU, Orsta consistently outperforms its backbone models, achieving approximately a 4\% improvement for the 7B variant and around 1\% for the 32B-0326 variants. In the mathematics-specific benchmark MathVista, Orsta delivers more substantial gains—exceeding 5\% across all model sizes. These improvements are consistent with the performance trends observed on mathematics-related tasks in MEGA-Bench, further highlighting Orsta’s effectiveness in enhancing reasoning capabilities. 

% For visual perception tasks, Orsta demonstrates consistent and notable improvements over baseline models. On COCO detection, Orsta-7B outperforms the baseline by +7.81 mAP and +12.17 mAP@50 on the single-object subset, and by +3.77 mAP and +5.48 mAP@50 on the multi-object subset, indicating stronger gains in simpler detection scenarios. Orsta-32B-0321 also shows substantial enhancements, effectively mitigating its prior perception issues. Orsta-32B-0326 achieves an average improvement of approximately +3\% mAP for both single-object and multi-object detection. On OVDEval, both Orsta-7B and Orsta-32B exhibit improvements of roughly +5.3 and +3.5 mAP, respectively, over their corresponding backbones, further validating the effectiveness and generalizability of the dynamic IoU reward function. For GUI-focused perception tasks such as ScreenSpot-Pro, Orsta delivers consistent gains of around 1–2\%, with similar trends observed in the OCR-specific benchmark OCRBench. The most significant gains appear in CountBench, where Orsta-7B surpasses even the 32B SFT models, and Orsta-32B achieves state-of-the-art performance, highlighting the effectiveness of our method in enhancing object counting capabilities across diverse perception tasks. Moreover, through comparing 0321 and 0326, our benchmarking on perception-related tasks indicates that RL offers more substantial improvements for base models lacking prior alignment, compared to already instructed models

==> 6_related_work.tex <==
\section{Related Work}
%
\begin{table}[tb!]
\small
\renewcommand{\arraystretch}{1.5}
\centering
\setlength{\tabcolsep}{0.8mm}
\scalebox{0.88}{
    \begin{tabular}{l|cc|cccccccc|c}
    \toprule 
    Model                                         & Size    & Backbone          & Math      & Science        & Chart      & Puzzle    & OCR        & DET  & GND  & CNT   & Others \\
    \midrule
    Visual-RFT~\cite{liu2025visual}               & 2B      & Qwen2-VL              & -          & -          & -          & -         & -          & \checkmark & \checkmark & -          & CLS    \\
    DeepPerception~\cite{ma2025deepperception}    & 2B      & Qwen2-VL Base$^{*}$   & -          & -          & -          & -         & -          & -          & -          & -          & S.QA \\
    Vision-R1~\cite{huang2025vision}              & 7B,72B  & Qwen2.5-VL            & \checkmark & \checkmark & -          & -         & -          & -          & -          & -          & - \\
    R1-Onevision~\cite{yang2025r1}                & 7B      & Qwen2.5-VL            & \checkmark & \checkmark & \checkmark & -         & -          & -          & -          & -          & V.QA \\
    Reason-RFT~\cite{tan2025reason}	             & 2B,7B   & Qwen2-VL              & \checkmark & -          & -          & -         & -          & -          & -          & \checkmark & S.QA \\
    OThink-MR1~\cite{liu2025othink}	             & 2B,7B   & Qwen2.5-VL            & \checkmark & -          & -          & -         & -          & -          & -          & \checkmark & -  \\
    Perception-R1~\cite{yu2025perception}	     & 2B,3B   & Qwen2$\And$2.5-VL & -          & -          & -          & -         & \checkmark & \checkmark & \checkmark & -          & - \\
    VLM-R1~\cite{shen2025vlm}	                 & 3B      & Qwen2.5-VL            & -          & -          & -          & -         & -          & \checkmark & \checkmark & -          & - \\
    MM-EUREKA~\cite{meng2025mm}	                 & 7B,32B  & Qwen2.5-VL            & \checkmark & -          & -          & -         & -          & -          & -          & -          & S.QA \\
    VL-Rethinker~\cite{vl_rethinker}	             & 7B,32B,72B  & Qwen2.5-VL            & \checkmark & \checkmark          & \checkmark          & -         & -          & -          & -          & -          & S.QA \\
    \midrule
    \textbf{Orsta (ours)}                        & 7B,32B  & Qwen2.5-VL            & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - \\
    \bottomrule
    \end{tabular}
}
\caption{\textbf{Task-wise Comparison of Public VLM-RL Models with Varying Model Configurations}.
The evaluated tasks include Math, Science, Chart, Puzzle, OCR, Detection, Grounding, Counting, Classification, Spatial question answering, and Visual question answering. Backbones marked with a star$^{*}$ indicate models trained from pre-trained backbone (i.e. zero-RL setting), while others are trained from instructed models.}
\label{tab:vlm-rl-comparble}
\end{table}
%
Adopted from DeepSeek R1~\cite{guo2025deepseek}, recent advancements in visual reinforcement learning (summarized in Table~\ref{tab:vlm-rl-comparble}) have explored diverse strategies to enhance multimodal reasoning and perception. Models such as Vision-R1~\cite{huang2025vision}, LMM-R1~\cite{peng2025lmm}, R1-OneVision~\cite{yang2025r1}, VisualThinker-R1-Zero~\cite{zhou2025r1}, and MM-Eureka~\cite{meng2025mm} primarily focus on strengthening reasoning capabilities through instruction tuning or reinforcement learning, leveraging CoT datasets, image-to-text conversion, or rule-based signals to elicit problem-solving behavior. In parallel, models like Visual-RFT~\cite{liu2025visual}, R1-V~\cite{chen2025r1v}, Reason-RFT~\cite{tan2025reason}, and DeepPerception~\cite{ma2025deepperception} apply task-specific, verifiable reward signals (e.g., IoU, mAP, math\_verify) to improve perception tasks such as detection, grounding, and counting. Seg-Zero~\cite{liu2025seg}, Perception-R1~\cite{yu2025perception}, and VLM-R1~\cite{shen2025vlm} further propose tailored reward functions for segmentation and OCR, though they largely remain within task-specific generalization boundaries. To address broader cross-task generalization, OThink-MR1~\cite{liu2025othink} incorporates GRPO with Dynamic KL, while VL-Rethinker~\cite{wang2025vl} introduces selective sample replay and forced rethinking to enhance reasoning capabilities.
\citet{su2025openthinkimg} explores visual RL for tools.
Additionally, several general-purpose VLMs have demonstrated the promise of visual reinforcement learning~\cite{team2025kimi,seed2025seed1_5vl}. In contrast to prior efforts that treat reasoning and perception in isolation, our proposed V-Triune unifies both domains under a single reinforcement learning system.


% Reinforcement learning (RL) has significantly advanced the reasoning capabilities of LLMs, prompting its extension to Vision-Language Models (VLMs). , models such as Vision-R1~\cite{huang2025vision}, R1-OneVision~\cite{yang2025r1}, and VL-Rethinker~\cite{vl_rethinker} focus on visual reasoning tasks—like math and science—via curated datasets and multimodal CoT strategies. RL-based approaches like VisualThinker-R1-Zero~\cite{zhou2025r1} and MM-EUREKA~\cite{meng2025mm} elicit emergent reasoning abilities through rule-based optimization. Concurrently, models like Visual-RFT~\cite{liu2025visual}, Reason-RFT~\cite{tan2025reason}, and DeepPerception~\cite{ma2025deepperception} extend RL to visual perception tasks such as detection and counting, using verifiable rewards (e.g., IoU, mAP). Perception-R1~\cite{yu2025perception} and VLM-R1~\cite{shen2025vlm} target detection and OCR, while OThink-MR1~\cite{liu2025othink} evaluates cross-task generalization using Dynamic KL. VL-Rethinker further introduces Forced Rethinking and Selective Sample Replay to improve slow reasoning. , achieving comprehensive task coverage.
% —spanning Math, Science, Charting, Puzzle, Detection, Grounding, Counting, and OCR—and demonstrates consistent performance gains across all evaluated benchmarks.
% %
% Reinforcement learning has effectively enhanced reasoning capabilities in Large Language Models (LLMs), and the success of DeepSeek R1\cite{guo2025deepseek} and Kimi K1.5\cite{team2025kimi} has driven the extension of the R1 training paradigm to Vision-Language Models (VLMs)\cite{zhou2025reinforced}. Certain studies focus on extending the performance limits of models in visual reasoning tasks\cite{xia2025generative}. 

% Vision-R1\cite{huang2025vision} constructs a multimodal CoT dataset using MLLM and DeepSeek R1 to cold-start the base model, and further enhances its reasoning ability through RL on mixed math datasets. Similarly targeting complex problem-solving, LMM-R1\cite{peng2025lmm} adopts a two-stage RL strategy on pure text and image-text data, whereas R1-OneVision\cite{yang2025r1} converts images into formal textual representations and builds a more diverse dataset with step-by-step reasoning annotations to apply SFT followed by RL. VisualThinker-R1-Zero\cite{zhou2025r1} and MM-Eureka\cite{meng2025mm} directly employ rule-based RL on base models, successfully eliciting the “Aha Moment” phenomenon in spatial reasoning and mathematical tasks.

% In parallel, Visual-RFT\cite{liu2025visual} and R1-V\cite{chen2025r1v} extend RL with verifiable rewards to visual perception, leveraging task-specific reward signals to update the model via GRPO, such as IoU-based reward for object detection and visual grounding, and math\_verify-based reward for visual counting. Reason-RFT\cite{tan2025reason} and DeepPerception\cite{ma2025deepperception} apply two-stage training strategy across multiple perception tasks. Similar to Visual-RFT, Seg-Zero\cite{liu2025seg} further designs bounding box and keypoint L1 distance, thinking format, and segmentation format rewards tailored for segmentation tasks to enhance performance. Perception-R1\cite{yu2025perception} and VLM-R1\cite{shen2025vlm} explore various reward designs for detection tasks, incorporating signals such as IoU, mean Average Precision (mAP), F1 score, and recall to optimize model training. While VLM-R1 primarily focuses on detection and visual grounding, Perception-R1 covers a broader range of tasks, including detection, grounding, counting, and optical character recognition (OCR). However, prior works mainly evaluate OOD performance within the same tasks, limiting validation to shifts in data distribution rather than across distinct task domains. OThink-MR1\cite{liu2025othink} adopts GRPO with a Dynamic KL divergence strategy and assesses cross-task generalization in counting and geometric reasoning. VL-Rethinker\cite{wang2025vl} integrates Selective Sample Replay (SSR) into GRPO and introduces Forced Rethinking to encourage slow-thinking, enhancing mathematical reasoning, multidisciplinary understanding, and performance on complex real-world tasks. 

% Our Orsta further broadens RL training to encompass a more extensive spectrum of perception and reasoning tasks, demonstrating consistently superior and robust performance across comprehensive benchmark suites and a wide range of downstream tasks.



==> 7_conclusion.tex <==
\section{Discussion \& Future Work}

In this paper, we propose V-Triune, the first visual triple-unified reinforcement learning system for vision-language models (VLMs) that effectively scales across both reasoning and perception tasks. Unlike previous approaches that are often limited to single-domain or lightweight tasks, V-Triune achieves substantial performance improvements across a broad spectrum of real-world vision-language challenges through its three-tier component design and dynamic IoU-based reward.

Notably, V-Triune yields Orsta-7B and Orsta-32B, with improvements of 3.2\% and 2.1\% over strong backbones, respectively. Our experiments indicate that reinforcement learning in VLMs primarily serves as an alignment strategy, refining the model’s decision-making and response behavior rather than enabling new knowledge acquisition. This supports the notion that RL fine-tuning enhances the utility and robustness of pre-trained VLMs without altering their foundational capabilities.


We also acknowledge several limitations that merit further investigation:
\begin{itemize}
    \item \textbf{Limited performance scaling in perception tasks:} For visual reasoning tasks, we observe clear trends of increasing response length and reflection ratio as training progresses, akin to test-time scaling laws observed in LLMs. However, such trends are not evident in visual perception tasks. The underlying factors driving performance improvements in perception remain unclear. Exploring multi-step RL for perception tasks, similar to approaches in OpenAI’s o3, may offer new insights and avenues for progress.
    
    \item \textbf{Underexplored potential of RL-zero in VLMs:} There is currently limited research on RL-zero for vision-language models. Nonetheless, we see early indications that RL-zero has the potential to surpass the current limitations imposed by supervised fine-tuning (SFT). Given that multi-modal alignment remains a fundamental challenge in VLMs, and that supervised fine-tuning (SFT) may be inherently limited in addressing this issue, we believe that RL-zero has the potential to redefine the optimization paradigm and unlock new capabilities for vision-language models.

\end{itemize}

The V-Triune system and Orsta models will be publicly available at \href{https://github.com/MiniMax-AI}{https://github.com/MiniMax-AI}. We hope this work inspires further research into reinforcement learning as a general-purpose training paradigm for vision-language understanding, and encourages exploration of richer reward schemes, advanced reasoning strategies, and task-specific adaptations.

==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

While reinforcement learning (RL) has emerged as a powerful paradigm for post-training Vision Language Models (VLMs), the current research landscape remains fragmented~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl}.
%
Prior works have largely specialized in one of two distinct domains: visual reasoning tasks like math and science QA~\citep{huang2025vision,yang2025r1,meng2025mm, vl_rethinker}, where RL training mirrors established LLM paradigms, or a narrow subset of perception tasks like object detection~\citep{yu2025perception, ma2025deepperception, liu2025visionreasoner}. This specialization has left a critical challenge largely unexplored: the creation of a unified RL framework that can jointly optimize a single VLM for both high-level reasoning and fine-grained perception.

This divide stems from a cascade of interlocking challenges that render existing RL frameworks ill-suited for unified VLM training. First, the heterogeneity of data requires managing diverse reward compositions even within a single task (e.g., some reasoning samples require only an accuracy reward, while others demand a joint accuracy-format reward with sample-specific weightings), demanding a level of fine-grained, sample-specific control that conventional systems lack. Second, this complexity is magnified by the fundamental incompatibility between reward paradigms: the exact-match verification required for reasoning tasks and the continuous spatial metrics (e.g., IoU) used in perception tasks like detection. Bridging these disparate paradigms in turn presents a major architectural hurdle, as a monolithic design would be brittle and unscalable. Finally, the joint training process itself is plagued by an opacity of dynamics, where aggregated metrics obscure source-specific failures, making it nearly impossible to diagnose instability or reward collapse.
%

To address these challenges,
we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a RL system to unify VLM training across reasoning and perception through a holistic co-design of data formatting, reward computation, and training diagnostics. V-Triune systematically resolves the aforementioned conflicts through a tightly integrated, three-tier architecture:
%
Sample-Level Data Formatting (\S\ref{subsec:sample_level_formatting}) tackles the challenge of task diversity by allowing each data sample to self-define its own reward configuration and verifier, enabling unparalleled flexibility.
%
Verifier-Level Reward Computation (\S\ref{subsec:verifier_level_reward_computation}) resolves the conflict between reward paradigms by delegating computation to specialized, modular verifiers.
A key innovation within this framework is the Dynamic IoU Reward mechanism (\S\ref{subsec:dynamic_iou}), which gradually raises the localization precision bar as training progresses, guiding the model toward high-precision localization. 
%
Lastly, Source-Level Metric Monitoring (\S\ref{subsec:metric_monitoring}) ensures training stability and provides granular diagnostics in this complex multi-task setting by logging metrics on a per-source basis.
%
Crucially, these components are not independent: sample-level declarations route data to the correct verifier, while source-level metrics inform adjustments to reward configurations, forming a closed-loop system for unified RL.

Leveraging the V-Triune system, we develop Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model series (7B-32B). These models undergo joint optimization across a diverse set of eight tasks, spanning visual reasoning (mathematics, science, chart, puzzle) and visual perception (object detection, grounding, OCR, counting). 
%
On the comprehensive MEGA-Bench core~\citep{chen2024mega} benchmark, which encompasses over 440 diverse, human-annotated tasks spanning reasoning, perception, and multimodal understanding, Orsta demonstrates substantial performance gains ranging from +2.1\% to +14.1\% across its variants compared to the base models. These benefits extend to prominent downstream benchmarks, including MMMU, MathVista, COCO, and CountBench, validating V-Triune's effectiveness and scalability.
%
Our core contributions are: 1) We introduce V-Triune, an unified, scalable, and extensible RL system for jointly training VLMs on both visual reasoning and perception tasks.
%
2) We propose the Dynamic IoU reward, a novel, adaptive reward mechanism that significantly enhances stability and performance for visual perception tasks like detection and grounding.
%
3) We establish a comprehensive training recipe, with key engineering optimizations, for stable and effective RL training across eight diverse tasks.
%
4) We present Orsta, a family of high-performance models trained with V-Triune, achieving strong performance across various benchmarks.


%
% The recent advancement of large language models (LLMs)~\citep{DBLP:journals/corr/abs-2412-16720,guo2025deepseek} and visual-language models (VLMs)~\citep{openai2025o3o4,google_deepmind_gemini_2025} has seen a paradigm shift from pre-training scaling to test-time scaling.
%
% A key manifestation of this shift is the practice of extending context length for Chain-of-Thought (CoT) reasoning, which significantly enhances performance on complex tasks such as mathematics and coding~\citep{xia2025generative, guo2025deepseek}.
% Moreover, existing works~\citep{liu2025visionreasoner,liu2025x} remain an open question whether RL can be effectively scaled to visual perception tasks such as object detection and grounding, which require distinct reward design and measures to ensure training stability.
% Beyond these core components, a key innovation in V-Triune is the Dynamic IoU reward (\cref{subsec:dynamic_iou}).
%
% This mechanism targets visual perception tasks like object detection and grounding, addressing issues with fixed IoU thresholds.
%
% By progressively adjusting the IoU reward threshold (from relaxed to stricter criteria), it ensures useful early learning signals, guides the model towards high-precision results, and ultimately enables stable, scalable training procedure.
% To visually situate our work within the current research landscape, \cref{tab:vlm-rl-comparble} provides a direct comparison, showcasing V-Triune's unification of a broad spectrum of reasoning and perception tasks where prior works have remained specialized.

==> sections/2_preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}
%
\noindent\paragraph{RL Algorithm}
\label{subsec:rlvr}
We adopt Group Relative Policy Optimization (GRPO)~\citep{shao2024deepseekmath}, following standard practice, but introduce two key modifications based on recent work~\citep{yu2025dapo, hu2025open}.
%
First, we remove the reference model and its associated KL loss. This avoids restricting exploration~\citep{hu2025open} and prevents unstable KL divergence estimates~\citep{schulman2020klapprox}, while also reducing GPU memory usage and speeding up training.
Second, we apply the clip-high trick and use token-level loss~\citep{yu2025dapo}, which help increase output entropy, encouraging better exploration and improving training stability.



\noindent\paragraph{Reward Function}
As discussed in~\cref{sec:intro}, the visual tasks are grouped into two categories: visual reasoning and visual perception.
%
To mitigate reward hacking, we employ rule-based reward functions for all tasks.
%
Visual reasoning tasks use a binary (0-1) accuracy-based reward function:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
The predicted answer $\hat{a}$ is parsed from model output, (instructed to be enclosed in  \texttt{\textbackslash{}boxed\{\}},  and verified against the ground-truth $a$ using \texttt{math\_verify}~\citep{mathverify2025}.
%

For visual perception tasks, the format of the ground-truth varies considerably.
%
Answers for counting and verifiable OCR are typically textual (e.g., numbers, words), making them compatible with the \texttt{\textbackslash{}boxed{}} format
%
Therefore, these tasks utilize the same accuracy reward defined in~\cref{eq:math_rule}.
%
In contrast, the answers for grounding and detection tasks are commonly structured in COCO-style \texttt{JSON} format, which includes both a bounding box and a label (see~\cref{fig:det_sample}).
%
Initial experiments revealed the model struggled to enclose this JSON format within \texttt{\textbackslash{}boxed{}} but readily learned to use \texttt{<answer></answer>} tags.
%
Consequently, we introduce a format reward for these two tasks:
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ represents the model's response to question $q$, and $s_i$ denotes a specific format tag ($\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$). The indicator function $\mathbb{I}(\text{condition})$ evaluates to 1 if the condition is true, and 0 otherwise.
%
For the accuracy component, we adapt the standard Intersection over Union (IoU)~\citep{everingham2010pascal} metric, a common practice in object detection and adopted in prior works~\citep{liu2025visual,yu2025perception,shen2025vlm}, with formulations provided in~\cref{eq:iou_rule}.
%
\begin{equation}
R_\text{acc}(\hat{a}, a) = 
\begin{cases} 
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else} 
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
$\hat{a}$ represents the predicted bounding box, and $a$ denotes the golden bounding box.
%
The threshold $\epsilon$ controls the strictness of the reward function, with higher values enforcing tighter matches. We ultimately adopt a dynamic $\epsilon$ finally, as detailed in~\cref{subsec:dynamic_iou}.
%
Finally, the overall reward, combining accuracy and format alignment, is defined as: $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are the respective weighting coefficients for each reward component.
%
% \begin{equation}
%     \begin{aligned}
%     \alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}
%     \end{aligned}
% \end{equation}

% \begin{equation}
%     R_\text{acc}(\hat{a}, a) = 
%     \begin{cases} 
%     \text{IoU}(\hat{a}, a), &  \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
%     0, & \text{else} 
%     \end{cases}
%     \label{eq:iou_rule}
% \end{equation}
% %
% where
% %
% \begin{equation}
% \begin{aligned}
% \text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
% \end{aligned}
% \end{equation}
%

% The advent of Deepseek-R1~\citep{guo2025deepseek} has established Reinforcement Learning as one of the dominant paradigms for post-training LLMs.
%
% Specifically, training through RL canlead to remarkably strong performance on reasoning tasks such as mathematics, code, and puzzles~\citep{xia2025generative, openai2025thinking}.
%
% RL encompasses two main key components: the algorithm and (verifiable) reward function.


% With these changes, the GRPO objective is updated as follows:
% 
% \begin{equation}
% \begin{aligned}
% \mathcal{J}(\theta) &= \mathbb{E}_{q \sim \mathcal{P}(q), \{o_i\}_{i=1}^G \sim \pi_{\theta_{\text{old}}}(\cdot|q)} \\ 
% &\left[ \frac{1}{\sum_{i=1}^G |o_i|} \sum_{i=1}^G \sum_{t=1}^{|o_i|} \min \left( r_{i,t}(\theta) \hat{A}_{i,t}, \text{clip}(r_{i,t}(\theta), 1 - \varepsilon_{\text{low}}, 1 + \varepsilon_{\text{high}})\hat{A}_{i,t} \right) \right] 
% \end{aligned}
% \end{equation}
% where
% \begin{equation}
% \begin{aligned}
% \quad \quad & r_{i,t}(\theta) = \frac{\pi_\theta(o_{i,t} \mid q, o_{i,<t})}{\pi_{\theta_{\text{old}}}(o_{i,t} \mid q, o_{i,<t})}, \quad \hat{A}_{i,t} = \frac{R_i - \text{mean}(\{R_i\}_{i=1}^G)}{\text{std}(\{R_i\}_{i=1}^G)}.
% \end{aligned}
% \end{equation}
% In this equation, $\mathcal{P}(q)$ represents the distribution of queries.%  
% The behavior model $\pi_{\theta_{\text{old}}}$ samples a group of $G$ responses $\{o_i\}_{i=1}^G$ for each query.% 
% Then, the advantage of the $i$-th response $\hat{A}_{i,t}$ is calculated from the normalized group-level rewards $\{R_i\}_{i=1}^G$,
% and then used to update the policy $\pi_{\theta}$.
% %
% The clipping range of the importance sampling ratio $r$ is bounded by $\epsilon_{\text{low}}$ and $\epsilon_{\text{high}}$.%

==> sections/3_method.tex <==
%
\begin{figure}[tb!]
    \centering    \includegraphics[width=0.99\linewidth]{images/figure2_v13.pdf}
    \caption{\textbf{The V-Triune System}. It integrates three core components operating at distinct levels: 1) Sample-Level Data Formatting to unify diverse task inputs; 2) Verifier-Level Reward Computation for custom rewards, which incorporates our novel Dynamic IoU reward for perception tasks like detection; and 3) Source-Level Metric Monitoring to diagnose problems at the data-source level.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}
%
This section describes V-Triune, our visual triple unified RL system. As shown in~\cref{fig:framework}, V-Triune jointly trains VLMs on diverse tasks spanning visual reasoning and perception within a unified pipeline.
%
The system comprises three core, interconnected components designed to collectively handle these diverse tasks.
%
The following subsections detail these three components, highlighting our novel Dynamic IoU reward mechanism.
%
\subsection{Sample-Level Data Formatting}
\label{subsec:sample_level_formatting}
%
This section introduces how data is formatted to support unified training across perception and reasoning tasks.
%
A key challenge is accommodating the diverse reward computations, components, and weighting strategies required by different tasks.
%
For example, tasks like math, puzzle, and OCR compute rewards based on the correctness of textual answers, while detection and grounding tasks rely on spatial metrics such as IoU and bounding box formatting.
%
In conventional RL setups, reward computation is typically defined at the task level.
%
While this allows modular reward functions to be implemented externally, it limits flexibility when fine-grained control is required.
%
Many tasks may contain heterogeneous samples that demand different reward strategies.
%
For instance, some samples require only an accuracy-based reward, while others demand a joint reward that accounts for accuracy and format, with sample-specific weightings, necessitating per-sample reward configurations.

%
To achieve this flexibility, we define reward configurations at sample level. Each sample specifies its reward types, relative weights, and associated verifier, enabling automatic reward routing and fine-grained weighting without modifying the core training logic.

Our data schema (the left of~\cref{fig:framework}), implemented with HuggingFace Datasets, extends common fields like \texttt{images} and \texttt{prompt} with several task-agnostic keys for reward control.
%
Specifically, we include: 1) \texttt{accuracy\_ratio} and \texttt{format\_ratio} to enable, disable or reweight different types of rewards on a per-sample basis by adjusting these ratios; 2) a \texttt{verifier} field to specify which verifier should be used for reward computation. (detailed in~\cref{subsec:verifier_level_reward_computation}); and 3) \texttt{data\_source} field to indicate sample origin and enable source-level metric monitoring (\cref{subsec:metric_monitoring}). \cref{fig:data_format} illustrates the complete data format, a design that reinforces the aforementioned sample-level flexibility.
%
In summary, this sample-level design is the key to integrating diverse datasets into a unified pipeline while maintaining flexible, scalable reward control.
%
\subsection{Verifier-Level Reward Computation}
\label{subsec:verifier_level_reward_computation}
%
A core design principle of V-Triune is to handle diverse tasks through a modular and scalable reward computation mechanism. To achieve this, we introduce the \textit{verifier-level}, a computation granularity where monolithic reward functions are replaced by specialized verifiers for specific task groups.
%
To implement this principle, we designed a standalone, asynchronous client-server architecture, illustrated in the middle of \cref{fig:framework}. Decoupling reward computation from the main training loop enhances modularity and scalability. In this architecture, requests are routed to the appropriate verifier based on the \texttt{verifier} field in each sample’s metadata, ensuring flexibility and extensibility.
%
To support the diverse visual reasoning and perception tasks involved in this work, we implement two primary verifiers, each encapsulating distinct, rule-based reward logic:
%
\noindent\paragraph{MathVerifyVerifier: For Reasoning, Counting, and OCR}
This verifier handles tasks with short-form textual answers that can be parsed and unambiguously verified by deterministic rules, such as reasoning, counting, and OCR. To mitigate reward hacking~\citep{weng2024rewardhack}, it employs a simple yet robust binary (0-1) accuracy-based reward function:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where the predicted answer $\hat{a}$ is parsed from model output, (instructed to be enclosed in  \texttt{\textbackslash{}boxed\{\}},  and verified against the ground-truth $a$ using \texttt{math\_verify}~\citep{mathverify2025}.

\noindent\paragraph{DetectionVerifier: For Detection and Grounding}
%
This verifier manages tasks that require spatial understanding and produce structured outputs, such as COCO-style \texttt{JSON}. Initial experiments revealed that the model struggled with the \texttt{\textbackslash boxed{}} format in JSON but readily learned to use \texttt{<answer>} tags. Consequently, this verifier computes a composite reward based on both format and accuracy.
%
First, to enforce the correct output structure, a format reward is defined as:
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ represents the model's response to question $q$, and $s_i$ denotes a specific format tag ($\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$). The indicator function $\mathbb{I}(\text{condition})$ evaluates to 1 if the condition is true, and 0 otherwise.

For the accuracy component, we adapt the standard Intersection over Union (IoU)~\citep{everingham2010pascal} metric, a common practice in object detection and adopted in prior works~\citep{liu2025visual,yu2025perception,shen2025vlm}, with formulations provided as:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) = 
\begin{cases} 
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else} 
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ represents the predicted bounding box, and $a$ denotes the golden bounding box.
%
The threshold $\epsilon$ controls the strictness of the reward function, with higher values enforcing tighter matches. We ultimately adopt a dynamic $\epsilon$ finally, as detailed in~\cref{subsec:dynamic_iou}.
%
Finally, the overall reward, combining accuracy and format, is defined as: $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are sample-specific weighting coefficients specified in the data format.

%
This verifier-level approach grants significant flexibility, modularity, and
extensibility. For instance, supporting a new task group merely requires implementing a new verifier, leaving the core training pipeline untouched. Finally, the computed rewards are returned and
integrated into their corresponding data samples for subsequent training and metric logging.

\subsubsection{Dynamic IoU Reward in DetectionVerifier}
%
\label{subsec:dynamic_iou}
%
For detection and grounding tasks, a robust reward signal is crucial for guiding the model toward fine-grained localization accuracy. We adopt a reward strategy based on IoU, as it provides a direct, interpretable, and controllable signal that is strongly aligned with task objective. While an IoU-based reward is a direct and robust choice, selecting a fixed threshold presents a fundamental dilemma.

On one hand, relaxed thresholds like IoU@50 (a common choice in~\citet{liu2025visual,yu2025perception}) can be too lenient as an RL reward signal. This leniency, especially when contrasted with the strict exact-match rewards in reasoning tasks, creates reward ambiguity. It allows multiple, distinct predicted bounding boxes to receive the same reward, and this ambiguous signal fails to provide a clear gradient for the model to refine its localization precision.
%
On the other hand, a potential solution to this ambiguity is to enforce a highly stringent threshold, such as $\epsilon=0.99$. This approach enhances consistency between perception and reasoning signals and provides an unambiguous target. However, its extreme stringency leads to a severe reward sparsity problem, as most initial predictions receive zero reward, hindering learning.

To resolve this dilemma, we adopt a dynamic IoU reward strategy. The IoU threshold is progressively tightened: starting at 0.85 for the initial 10\% of training, increasing to 0.95 until the 25\% mark, and finally settling at 0.99 for the remainder. This staged approach results in a distinctive step-like reward pattern, where the training reward drops with each increase in difficulty and subsequently recovers as the model adapts, as demonstrated in the lower right of~\cref{fig:framework}. This curriculum-based approach thus resolves the trade-off between reward ambiguity and sparsity.
%
\subsection{Source-Level Metric Monitoring}
\label{subsec:metric_monitoring}
%
Monitoring training metrics is essential for understanding model dynamics and real-time issue diagnosis. However, for multi-task, multi-source training, aggregated or single-task metrics are often insufficient due to lack of traceability and per-source data variations. Therefore, we adopt source-level metric monitoring, which involves logging metrics per \texttt{data\_source} for each batch.
%
This approach helps identify faulty data sources, enables targeted debugging, and reveals cross-source learning interactions.
%
This granular monitoring is particularly vital in RL, where training instability requires the more granular diagnostic capabilities that our source-level detail provides over standard built-in logging.
%
This design has been instrumental in diagnosing and resolving numerous training issues, which are detailed in~\cref{sec:training_recipe} as a contribution to the community.
%

As shown in the upper right of~\cref{fig:framework}, data batches are grouped by data source for metric logging after rewards are computed.
%
We designed a comprehensive set of metrics, organized into four categories, all of which are logged on a per-source basis.
%
We log a detailed breakdown of \textit{Training Reward}, including rule-based accuracy, output format, and IoU-based signals, to directly assess how well the model is learning specific data source. In parallel, we track \textit{Response Length} metrics, such as average lengths and truncation rates, to analyze the model’s generative patterns and diagnose critical issues like undesirable verbosity or potential model collapse.

For deeper insights and overall stability, we monitor two additional metric suites.
%
To understand the model’s reasoning process, we monitor \textit{Reflection} metrics inspired by \citet{ma2025rethinking}, computing the reflection ratio by tracking a curated list of 15 reflective words from their work, alongside the correctness rate within these reflection responses~(see \cref{appx:reflection_metrics} for details). This lightweight analysis helps distinguish productive self-correction from inefficient ``overthinking''. Finally, a suite of \textit{Auxiliary Metrics} provides a comprehensive overview of secondary objectives and training stability. These include standard perception evaluations, such as mAP and IoU at fixed thresholds (@50, 75, 95, 99), complemented by logging of sample responses for qualitative assessment of model behavior.
%

% To address these issues, we initially use a rule-based IoU reward scheme that enforces a stringent threshold of $\epsilon=0.99$, requiring near-exact spatial alignment between predicted and ground-truth boxes (\cref{fig:dyn_iou}b).
%
% This strict criterion enhances consistency between perception and reasoning signals and, by providing an unambiguous target, aims to improve training stability. However, its very stringency introduces a cold-start problem in early rollouts, where most predictions receive 0 reward.

% To mitigate this cold-start problem, we adopt a dynamic IoU reward strategy, inspired by curriculum learning~\citep{bengio2009curriculum}. The IoU threshold $\epsilon$ is adjusted in stages based on training progress: starting at 0.85 for the initial 10\% of training steps, increasing to 0.95 for the subsequent 15\% of steps (i.e., from 10\% to 25\% of total steps), and finally settling at 0.99 for the remainder of training (as illustrated in the lower right of~\cref{fig:framework}).



% To support such flexibility, we define reward configurations directly at the sample level.
% %
% Each sample specifies the types of rewards to compute, their relative weights, and the associated verifier to use.
% %
% This allows dynamic reward routing and fine-grained weighting during training without modifying core training logic.
% %
% It can also support curriculum learning or data ablation strategies simply by adjusting metadata, making the system more extensible and maintainable.

% As shown in the left~\cref{fig:framework}, we implement our data schema using the HuggingFace datasets~\citep{lhoest-etal-2021-datasets}, which serves as the unified interface for all data sources described in~\cref{subsec:data}.
% %
% Besides common fields such as \texttt{images} and \texttt{prompt}, the format includes several task-agnostic keys to support reward control.
% %
% Fields like \texttt{accuracy\_ratio} and \texttt{format\_ratio}, which define the weight of each reward type.
% %
% By adjusting these values, specific rewards can be enabled, disabled, or reweighted per sample.
% %
% The \texttt{verifier} field specifies which verifier should be used for reward computation.
% %
% More details on the verifier system are discussed in~\cref{subsec:verifier_level_reward_computation}.
% %
% The \texttt{data\_source} field indicates the origin of each sample and is used in source-specific metric monitoring in~\cref{subsec:metric_monitoring}.

% We use an asynchronous client-server architecture (the middle of \cref{fig:framework}) using FastAPI~\citep{ramirez_fastapi}.
% %
% The client collects batches of samples from the dataloader and processes each sample to a structured payload (~\yan{To express the payload is to retain only the key value required to calculate the reward in the data}) containing task-specific key-value pairs.
% %
% The client asynchronously send http requests and transport these structured payloads to multiple remote servers with a random balance strategy.
% %
% Each remote server routes each request to the appropriate verifier based on the ``\texttt{verifier}'' key in data format.

% For training reward, we log per-source reward values to trace dataset-specific stability. For perception tasks like grounding and detection, we also log detailed per-source IoU values (at thresholds {50, 75, 95, 99}) and mAP scores for fine-grained convergence insights.
%
% Inspired by~\citet{maye}, we also track model behavior by monitoring response length and reflection ratio per source. For response length, we log various metrics including overall average, lengths of correct/incorrect responses, and truncation rates. Truncation rates (outputs hitting maximum length) can indicate overly verbose or collapsed generation. For reflection ratio, we track 15 pre-defined reflection-related words (e.g., \textit{"re-check", "re-think", "verify"}).
%
% We then compute \texttt{reflection ratio}: the proportion of responses containing these reflection words and \texttt{correct ratio in reflection responses}: the accuracy of responses that include these words.
%
% This helps diagnose model tendencies like overthinking versus superficial responses by linking reflection to correctness. All mentioned metrics are consistently logged per data source.
% In object detection and visual grounding, Intersection over Union (IoU)~\citep{everingham2010pascal} and mean Average Precision (mAP)~\citep{lin2014microsoft} are standard metrics for evaluating the overlap between predicted and ground-truth bounding boxes. While mAP summarizes performance across multiple IoU thresholds, our preliminary detection experiments show that using a thresholded IoU reward achieves comparable overall performance while providing more interpretable and controllable feedback (\cref{fig:dyn_iou}a). Therefore, we adopt an IoU-based reward strategy for its robustness and stronger alignment with localization accuracy (\cref{eq:iou_rule}).
%
% \begin{wrapfigure}[16]{tr}{0.30\textwidth} 
%   \centering
%   \includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_ovd_acc.pdf}
%   \caption{Training accuracy rewards under Dynamic IoU versus a fixed Rule-based IoU (IoU@99).}
%   \label{fig:traning_acc_track}
% \end{wrapfigure}
% However, relaxed thresholds like IoU@50 (common option in~\citet{liu2025visual,yu2025perception}) can be too lenient for RL in VLMs, especially when compared to the strict exact-match rewards used in reasoning tasks (\cref{eq:math_rule}).
%
% Moreover, these loose thresholds result in reward ambiguity: even if predicted bounding boxes merely shift or are oriented differently around the ground-truth, they can still receive the same high reward. Such ambiguity can ultimately lead to a decline in performance during later training stages for detection task (\cref{fig:dyn_iou}b).
% Our pilot results (\cref{fig:dyn_iou}c and d) empirically confirm that this strategy significantly improves learning efficiency and overall test set performance.
% As our pilot study confirms (\cref{fig:dyn_iou}b), this ambiguity ultimately hinders the learning process, leading to performance degradation.
% However, we found relaxed thresholds like IoU@50 (a common choice in~\citet{liu2025visual,yu2025perception}) can be too lenient as an RL reward signal. This leniency, especially when contrasted with the strict exact-match rewards in reasoning tasks (\cref{eq:math_rule}), creates reward ambiguity. It allows multiple, distinct predicted bounding boxes to receive the same reward. This ambiguous signal fails to provide a clear gradient for the model to refine its localization precision. 
% One potential solution to the reward ambiguity is to enforce a highly stringent threshold, such as $\epsilon=0.99$, to approximate an exact-match criterion. This approach enhances consistency between perception and reasoning signals and provides an unambiguous target. However, its extreme stringency leads to a severe reward sparsity problem, as most initial predictions receive zero reward, hindering learning.
%
% While many RL infrastructures support built-in metric logging, our source-level detail provides more granular diagnostic capabilities.
%
% This design has been instrumental in diagnosing and resolving numerous training issues, which are detailed in~\cref{sec:training_recipe} as a contribution to the community.
%This metadata-driven approach also naturally supports strategies like curriculum learning or data ablation, enhancing system's extensibility.
% \begin{equation}
%     R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
%     \label{eq:math_rule}
% \end{equation}
%

%
% To overcome the limitations of fixed reward functions, our system utilizes a standalone, asynchronous reward server to generate RL signals.
%
% Decoupling reward computation from the main training loop offers several key advantages. This design enhances modularity for diverse tasks and supports independent scaling, which is crucial for GPU-based evaluations. Furthermore, it improves maintainability and boosts training throughput via distributed, asynchronous processing.
%
% The term \textit{verifier-level} defines our computation granularity, where specialized verifiers for specific task groups replace monolithic reward functions.

% We use an asynchronous client-server architecture (the middle of \cref{fig:framework}) using FastAPI~\citep{ramirez_fastapi}. The client collects data batches and processes each sample into a lightweight payload, containing only the key-value pairs essential for reward computation (e.g., model predictions and ground-truth labels). These payloads are then sent asynchronously via HTTP requests to multiple remote server replicas using a random load-balancing strategy. Each remote server routes the request to the appropriate verifier based on the \texttt{verifier} key in the data format.
%
% Each user-defined verifier encapsulates custom functions to compute task-specific rewards based on model outputs and ground truth.
%
% In our implementation, we primarily use two types:
%
% \textit{MathVerifyVerifier}: Handles reasoning, OCR, and counting tasks by evaluating answer correctness.
%
% \textit{DetectionVerifier}: Manages detection and grounding tasks, notably employing our novel Dynamic IoU reward (\cref{subsec:dynamic_iou}) alongside format-based rewards.
% $R_\text{acc}(\hat{a}, a) = \mathbb{I}(\text{verify}(\text{parse}(\hat{a}), \text{parse}(a)))$.
%
% The predicted answer $\hat{a}$ is parsed from the model output (enclosed in \texttt{\textbackslash{}boxed\{\}}) and verified against the ground-truth $a$ using \texttt{math\_verify}~\citep{mathverify2025}.
% For instance, OCR data may include both plain-text lines and complex tables, each requiring different evaluation rules.
%
% Similarly, detection samples can differ significantly in terms of object count, annotation completeness, or visual difficulty, which necessitates sample-wise adjustment of reward behavior.


==> sections/5_experiment.tex <==
\section{Experiment}
%
\begin{figure}[tb!]
    \centering
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure3/7b.pdf}
        % \caption{Model 7B}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure3/32b_0321.pdf}
        % \caption{Model 32B}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.24\textwidth}
                \includegraphics[width=\linewidth]{images/figure3/32b_0326.pdf}
        \end{subfigure}
    % \hfill
        \begin{subfigure}{0.24\textwidth}
            \includegraphics[width=\linewidth]{images/figure3/32b_0321_details_v2.pdf}
        \end{subfigure}
    \caption{Training trends of on-policy vs off-policy across three model variants on MEGA-Bench core: 7B-(a), 32B-0321-(b) 32B-0326-(c) and task level performance of Orsta-32B-0321-(d).
Models are evaluated every 5 generation steps from 0 to 135. The dark line in (d) denotes the task-level MEGA-Bench Core, linking to the performance shown in the blue line of (b).}
    \centering
\label{fig:mega_performance_track}
\vspace{-10px}
\end{figure}
%
\subsection{Implementation Details}
\label{subsec:implementation details}

\noindent\textbf{Models and Data:} We adopt Qwen2.5-VL-7B-Instruct and Qwen2.5-VL-32B-Instruct (0321 and 0326 versions, denoting their release dates) as our base models, chosen for their strong performance across both vision-language reasoning and perception.
%
We curated a multi-task dataset of 47.7K high-quality samples from 18 sources, covering four reasoning and four perception tasks. Detailed information on data sources, filtering, and hyperparameters is provided in~\cref{subsec:data}.

\noindent\textbf{Training Recipe:}
%
V-Triune is implemented upon verl~\citep{sheng2024hybridflow}.
%
All experiments are conducted on 64 NVIDIA H20 GPUs.
%
Informed by our source-level monitoring, we implemented several key strategies to ensure stable and scalable training: freeze the ViT to prevent gradient explosion, filter leaked image tokens in responses, utilize a prompt pool to mitigate variance, and optimize system memory management. A detailed analysis of these strategies is provided in~\cref{sec:training_recipe}.

\noindent\textbf{Experimental Settings:}
%
We employ a modified version of Group Relative Policy Optimization (GRPO)~\citep{shao2024deepseekmath} for all experiments.
%
Inspired by recent work~\citep{yu2025dapo, hu2025open}, we remove the reference model and its associated KL loss to improve exploration and training efficiency~\citep{hu2025open, schulman2020klapprox}, and apply the clip-high trick with token-level loss to further enhance stability~\citep{yu2025dapo}.
%
We compare two configurations: a standard on-policy setup and an off-policy setup with 8 optimization steps per rollout.
%
Both are trained for 3 epochs with a rollout batch size of 1024, generating 8 candidate sequences per prompt.
%
We freeze the ViT and connector modules for stability. Learning rates are $1 \times 10^{-6}$ (on-policy) and $5 \times 10^{-7}$ (off-policy) with a 5\% warmup. Rollouts use the vLLM engine with sampling (temperature=1.0, top-p=1.0, max length=2048), while testing uses greedy decoding.
\vspace{-7px}
\noindent\paragraph{Evaluation Benchmarks:}
% \label{evaluation benchmarks}
%
To comprehensively assess our model's capabilities, we evaluate its performance across three key domains: real-world tasks, visual reasoning, and visual perception. 
%
For a holistic evaluation on real-world tasks, we employ the core subset of MEGA-Bench~\citep{chen2024mega}
which consists of 440 diverse, long-tailed tasks encompassing over 6,000 expert-curated samples. For visual reasoning, we adopt MMMU~\citep{yue2024mmmu} and MathVista~\citep{lu2023mathvista}. For visual perception, our evaluation suite includes COCO~\citep{lin2014microsoft}, OVDEval~\citep{yao2023evaluate}, CountBench~\citep{paiss2023teaching}, OCRBench~\citep{fu2024ocrbench}, and ScreenSpot-Pro~\citep{li2025screenspot}.
%
Detailed evaluation protocols for each benchmark, including specific metrics, scoring methods, and implementation details, are provided in~\cref{sec:eval_details}.
%
\begin{table}[tb!]
\small
\renewcommand{\arraystretch}{1.5}
\centering
\caption{Performance comparison on MEGA-Bench core. Models with improved reasoning are marked by \faLightbulb[regular]; final scores are reported as weighted averages. QwenVL-2.5-32B-0321 is a version with incomplete post training, which are resolved in the 0326 version. All results are obtained using the official MEGA-Bench evaluation code, except for Gemma3-27B ($\dagger$).}
\setlength{\tabcolsep}{0.8mm}
\scalebox{0.75}{
    \begin{tabular}{l|cccccccc|c}
        \toprule 
        Model                                                & Knowledge    & Mathematics    & Perception    & Coding         & Info. Ex.     & Planning      & Science       & Metrics       &  \makecell{MEGA-Bench \\ Core} \\ \midrule \multicolumn{10}{c}{7B+ Model}   \\ \midrule
        
        QwenVL-2-7B~\citep{wang2024qwen2}                                           & 39.96         & 25.95         & 39.99         & 31.49         & 40.29         & 16.64         & 28.59         & 43.61         & 34.47 \\
        QwenVL-2.5-7B~\citep{Qwen2.5-VL}                                         & 38.84         & 27.67         & 41.24         & 28.93         & 50.23         & 16.32         & 36.75         & 41.64         & 35.07 \\ 
        InternVL-3-8B~\citep{zhu2025internvl3}                                         & 36.64         &\textbf{32.75} & 42.17         &\textbf{35.11} & 48.92         & 14.35         & 36.51         &\textbf{53.94} & 36.48 \\
        Gemma3-12B~\citep{team2025gemma}                                            & 41.11         & 29.10         & 37.38         & 30.27         & 46.56         & 16.10         & 36.83         & 50.40         & 35.04 \\
        Kimi-VL-A3B~\citep{kimiteam2025kimivltechnicalreport}                                           & 37.63         & 27.07         & 39.50         & 22.30         & 40.99         &\textbf{22.17} & 33.94         & 46.65         & 34.40 \\
        MM-Eureka-7B \faLightbulb[regular]~\citep{meng2025mm}                    & 40.12         & 31.59         & 39.71         & 28.75         & 49.32         & 16.64         & 37.25         & 46.39         & 35.96 \\
        VL-Rethinker-7B \faLightbulb[regular]~\citep{vl_rethinker}                 & 40.65         & 30.08         & 42.02         & 29.87         & 52.03         & 17.83         & 36.82         & 46.90         & 37.25 \\ 
        Kimi-VL-A3B-Thinking  \faLightbulb[regular]           & 33.45         & 17.76         & 28.11         & 14.69         & 41.14         & 12.64         & 28.60         & 43.97         & 27.08 \\
        \hline
        \textbf{Orsta-7B (Ours) \faLightbulb[regular]}        &\textbf{41.65} & 31.48         &\textbf{43.84} & 32.82         &\textbf{54.07} & 17.83         &\textbf{36.91} & 41.66         &\textbf{38.31} \\  
        
        \rowcolor{blue_light_1}
        $\triangle$ (Ours - Backbone)                         & +2.8          & +3.8         & +2.6          & +3.9           & +3.8          & +1.5          & +0.2          & +0.0          & +3.2   \\
        \midrule \midrule
        
        \multicolumn{10}{c}{32B+ Model}  \\ \midrule
        QwenVL-2.5-32B-0321~\citep{Qwen2.5-VL}                                   & 8.48          & 12.62         & 11.99         & 13.59         & 15.44         & 8.61          & 16.78         & 14.91         & 11.87 \\ 
        MM-Eureka-32B     \faLightbulb[regular]~\citep{meng2025mm}               & 12.20         & 20.19         & 21.88         & 15.86         & 21.23         & 15.47         & 19.95         & 22.77         & 18.57 \\
        VL-Rethinker-32B   \faLightbulb[regular]~\citep{vl_rethinker}              & 12.16         & 28.09         & 22.99         & 11.89         & 21.50         & 15.09         & 28.10         & 15.73         & 19.41 \\
        \hline
        \textbf{Orsta-32B-0321 (Ours) \faLightbulb[regular]}  &\textbf{21.33} &\textbf{28.55} &\textbf{32.23} &\textbf{19.44} &\textbf{26.38} &\textbf{17.78} &\textbf{33.20} &\textbf{24.18} &\textbf{25.94} \\
        \rowcolor{blue_light_1}
        $\triangle$ (Ours - Backbone)                         & +12.9         & +15.9         & +20.2         & +5.9          & +10.9         & +9.2         & +16.4         & +9.3           & +14.1 \\
        \midrule
        
        Gemma3-27B $\dagger$~\citep{team2025gemma}                                  & 49.43         & 42.20         & 45.46         & 40.18         & 49.30         & 24.96         & 47.08         & 58.99         & 41.82 $\dagger$  \\
        QwenVL-2.5-32B-0326~\citep{Qwen2.5-VL}                                   & 46.09         & 32.04         & 47.55         & 38.36         & 61.65         & 28.43         & 37.55         & 50.38         & 43.67 \\  
        InternVL-3-38B~\citep{zhu2025internvl3}                                       & 46.32         &\textbf{40.29} &\textbf{55.05} &\textbf{45.29} & 56.63         & 22.88         &\textbf{52.04} &\textbf{58.04} &\textbf{46.69} \\
        Skywork-R1V-38B \faLightbulb[regular]~\citep{peng2025skywork}                 & 25.59         & 28.45         & 22.95         & 19.88         & 19.53         & 9.74          & 22.64         & 37.55         & 21.54 \\
        Skywork-R1V2-38B \faLightbulb[regular]~\citep{peng2025skywork}                & 17.08         & 12.38         & 15.65         & 7.14          & 9.90          & 17.60         & 14.29         & 0.0           & 15.39 \\
        \hline
        \textbf{Orsta-32B-0326 (Ours) \faLightbulb[regular]}  &\textbf{46.78} & 37.43         & 50.86         & 38.92         &\textbf{63.14} & 28.05         & 42.68         & 53.01         & 45.77 \\ 
        \rowcolor{blue_light_1}
        $\triangle$ (Ours - Backbone)                         & +0.7           & +5.4          & +3.3          & +0.6           & +1.5          & -0.4         & +5.1         & +2.6           & +2.1  \\
        \bottomrule
    \end{tabular}
}
\label{tab:main_results}
\end{table}
%
\subsection{Performance and Analysis}
%
\subsubsection{MEGA-Bench}
%
\cref{tab:main_results} compares Orsta against its backbone and other leading general-purpose/reasoning-enhanced VLMs.
%
Orsta shows consistent gains at both 7B and 32B scales: Orsta-7B achieves 38.31 (+3.2) on MEGA-Bench Core, and Orsta-32B-0326 reaches 45.78 (+2.1).
%
V-Triune notably boosts performance in domains with enriched training data—mathematics (+3.8 at 7B, +5.4 at 32B), perception, planning, and science—indicating strong generalization in both reasoning and perception tasks. More impressively, our method’s benefits generalize to out-of-domain tasks, with coding and metrics showing performance gains despite the absence of corresponding training data.

Beyond these top-line numbers, a deeper analysis of the two 32B variants reveals the core impact of our V-Triune system.
%
The Orsta-32B-0321 variant serves as an ideal case study for the alignment power of our approach. Its underlying checkpoint, Qwen2.5-VL-0321, is a publicly released version with known deficiencies in perception and output formatting, a finding confirmed by both our evaluations and prior work like~\citet{vl_rethinker}. These issues are addressed in the subsequent 0326 release. We therefore consider 0321 version a strong baseline with significant untapped potential that our RL framework aims to unlock.
%
V-Triune successfully unlocks this potential: as shown in~\cref{tab:main_results} and \cref{fig:mega_performance_track}(d), in-domain tasks covered by our training data see substantial gains exceeding 10\%. More significantly, out-of-domain tasks like coding and metrics also achieve a 5-10\% performance boost. This demonstrates that our unified RL training acts as a powerful, general-purpose alignment mechanism, enhancing the model's overall capabilities through strong generalization.
%
Furthermore, the results from the already well-aligned 32B-0326 variant confirm that V-Triune is also a potent fine-tuning tool. Despite this model's strong initial performance, our framework still elicits considerable gains, pushing its capabilities even further.

In addition to the final scores, the training dynamics themselves offer valuable insights into the optimization behavior of different RL strategies. As shown in \cref{fig:mega_performance_track}, the MEGA-Bench learning curves reveal that the relative effectiveness of on-policy versus off-policy RL varies across model sizes. For the 7B variant, off-policy training leads to faster convergence and higher final performance, whereas for the larger 32B models (32B-0321 and 32B-0326), on-policy training, despite its slower initial progress, achieves more sustained improvement and higher peak performance. These results indicate that neither strategy consistently outperforms the other; instead, their relative merits appear to differ depending on the specific model. In practice, it is advisable to evaluate both approaches empirically and select the one that yields better performance for the given model and task.

%In addition to the final scores, the training dynamics themselves provide further insights into the optimization process.
%\cref{fig:mega_performance_track} shows the MEGA-Bench learning curves of three Orsta variants (7B, 32B-0321, 32B-0326) under on-policy and off-policy RL. Off-policy training typically yields faster initial improvements but tends to plateau earlier, suggesting a trend to settle into local optima. In contrast, on-policy training, while starting slower, demonstrates more sustained growth and ultimately achieves higher peak performance across most model variants, indicating it is more effective for long-term optimization.
%
In summary, our results show that V-Triune is a versatile system: it can both unlock the latent potential of less-aligned models and further polish state-of-the-art ones, solidifying the role of unified RL as a powerful and general-purpose alignment strategy for VLMs.



% As shown in~\cref{fig:mega_performance_track}~d, Orsta-32B-0321 demonstrates that reinforcement learning primarily enhances existing model strengths, serving as an alignment mechanism rather than introducing new capabilities. Performance gains are most notable in in-domain tasks—mathematics, perception, science, and planning, while out-of-domain tasks like coding see limited improvement, underscoring RL’s alignment-focused impact.
%
% In summary, our results demonstrate that reinforcement learning effectively enhances both visual reasoning and perception within a unified framework. RL consistently improves performance across MEGA-Bench core’s 440 diverse tasks, supporting its role as a general-purpose alignment strategy that unlocks latent capabilities in pretrained vision-language models.
%
\begin{table}[tb!]
    \small
    \renewcommand{\arraystretch}{1.5}
    \centering
    \caption{Performance on common downstream tasks. We report the mAP\textbar{}mAP@50 for COCO, NMS-mAP for OVDEval and accuracy for others. We compute mAP score on COCO using the standard cocoapi, with full evaluation details in~\cref{sec:vlm_centric_map_final_definitive}.}
    \setlength{\tabcolsep}{1.0mm}
    \scalebox{0.77}{
       \begin{tabular}{lcccccc}
            \toprule 
            % \multirow{2}{*}{Tasks} & \multicolumn{2}{c}{7B}           & \multicolumn{4}{c}{32B}     \\
            Tasks       & QwenVL-2.5-7B          & \textbf{Orsta-7B }       & \makecell{QwenVL-2.5-32B\\0321}      & \makecell{\textbf{Orsta-32B}\\0321}       & \makecell{QwenVL-2.5-32B\\0326}     & \makecell{\textbf{Orsta-32B}\\0326} \\
            \midrule
            \multicolumn{7}{c}{Visual Reasoning}  \\ 
            \midrule
            MMMU$_{\text{val, rule-score}}$~\citep{yue2024mmmu}      & 45.56          & 49.70          & 37.11          & 34.67          & 39.22         & 38.00 \\ 
            MMMU$_{\text{val, gpt-score}}$~\citep{yue2024mmmu}     & 54.40          & 57.10          & 60.80          & 64.11          & 64.20         & 64.78 \\
            MathVista$_{\text{testmini}}$~\citep{lu2023mathvista}  & 67.50          & 72.50          & 70.80          & 76.30          & 73.40         & 76.40 \\
            \midrule
            \multicolumn{7}{c}{Visual Perception} \\ 
            \midrule
            COCO$_{\text{val, single-object}}$~\citep{lin2014microsoft}         & 79.20 \textbar{} 89.79  & 80.73 \textbar{} 91.45  &  2.09  \textbar{}  2.33      &    52.99   \textbar{}   62.93     &   79.30   \textbar{}  94.19     &    79.10   \textbar{}    93.76   \\  
            COCO$_{\text{val, multiple-object}}$~\citep{lin2014microsoft}       & 32.12 \textbar{} 42.65  & 41.41 \textbar{} 56.06  &    0.88   \textbar{}    1.01    &   28.65    \textbar{}    38.35    &   42.16    \textbar{}   56.39    &   45.43    \textbar{}     60.98     \\
            COCO$_{\text{val, full}}$~\citep{lin2014microsoft}       & 33.63 \textbar{} 44.16  & 42.45 \textbar{} 56.92  &    0.88   \textbar{}    1.00    &   29.29    \textbar{}    38.89    &   43.28    \textbar{}   57.43    &   46.39    \textbar{}     61.81     \\
            OVDEval~\citep{yao2023evaluate}                 & 52.23          &  57.52              & 3.84               &  35.65              &  56.80             &  60.36              \\
            ScreenSpot-Pro~\citep{li2025screenspot}          & 22.71          & 23.91          & 49.46          & 50.98          & 51.23         & 52.69  \\
            CountBench~\citep{paiss2023teaching}              & 71.69          & 82.28          & 83.71          & 88.59          & 83.91         & 88.19  \\     
            OCRBenchv2~\citep{fu2024ocrbench}                & 55.11          & 56.05          & 44.85          & 43.78          & 58.14         & 59.09  \\
            \bottomrule
        \end{tabular}
    }
    \label{tab: downstream_result}
    \vspace{-10px}
\end{table}
%
\subsubsection{Common Downstream Tasks}
%
As shown in~\cref{tab: downstream_result}, MMMU shows consistent gains on the more reliable gpt-score evaluation, with improvements of +2.7\% (7B), +3.3\% (32B-0321), and +0.6\% (32B-0326). On MathVista, it achieves around 5\% gains. These results align with improvements seen on math tasks in MEGA-Bench, reinforcing Orsta’s strength in enhancing reasoning capabilities. 

Orsta models demonstrate consistent improvements in visual perception on the COCO benchmarks. Specifically, Orsta-7B delivers notable gains, particularly in the more challenging multi-object detection task with a +9.29 mAP increase. 
%
Orsta-32B-0321 dramatically rectifies the perception shortcomings of its baseline, achieving massive boosts of over 50 mAP for single-object and nearly 28 mAP for multi-object detection. Building on a strong foundation, Orsta-32B-0326 further advances multi-object performance by +3.27 mAP, while maintaining a similar level of performance on single-object detection. On OVDEval, Orsta-7B and 32B-0326 improve by +5.3 and +3.5 mAP. The trend of broad improvements continues on other benchmarks: while GUI and OCR tasks see modest but consistent gains, CountBench shows the most remarkable boost, with Orsta-7B approaching the performance of 32B baselines and Orsta-32B. Overall, V-Triune delivers greater perception improvements for less-aligned base models (0321) than for well-aligned ones (0326).


%Orsta consistently improves visual perception across benchmarks. On COCO, Orsta-7B achieves notable gains (+7.81 mAP and +12.17 mAP@50 for single-object; +3.77 mAP and +5.48 mAP@50 for multi-object), with stronger gains in simpler scenarios. Orsta-32B-0321 shows marked improvements, addressing prior perception issues, while 32B-0326 yields 1.5-2\% mAP gains across both subsets. On OVDEval, Orsta-7B and 32B-0326 improve by +5.3 and +3.5 mAP. The trend of broad improvements continues on other benchmarks: while GUI and OCR tasks see modest but consistent gains, CountBench shows the most remarkable boost, with Orsta-7B approaching the performance of 32B baselines and Orsta-32B. Overall, V-Triune delivers greater perception improvements for less-aligned base models (0321) than for well-aligned ones (0326).
%
\subsubsection{Training Dynamics Analysis}
%
We conducted an in-depth analysis of the model's training dynamics using V-Triune's source-level metric monitoring. As shown in~\cref{fig:train_analysis}, the results reveal distinct behavioral patterns across different task categories. For reasoning-intensive tasks like Math and Puzzle-solving, the model progressively increases its response length, suggesting it learns to employ longer, more elaborate chains of thought.
%
In stark contrast, for the perception task of Detection, the model exhibits an opposite trend: its responses become more concise. This suggests that for tasks requiring precise, direct outputs, the model learns to suppress verbose reasoning in favor of more efficient, direct prediction.
%
Interestingly, the OCR task presents a hybrid pattern. While also a perception task, its response length show a upward trend, similar to the reasoning tasks. This divergence within perception tasks strongly supports a hypothesis that the model activates distinct cognitive pathways tailored to specific task demands, rather than adopting a uniform strategy. A detailed analysis is provided in~\cref{sec:training_dynamics_analysis}.
%
% Furthermore, we conducted an in-depth analysis of the model's training dynamics through V-Triune's source-level metric monitoring. As shown in~\cref{fig:train_analysis}, the results indicate that the model progressively exhibits longer chains of thought and more frequent reflection behaviors in reasoning tasks (such as mathematics and puzzle-solving). In contrast, this pattern does not emerge in perception tasks (like detection). Moreover, we did not find that reasoning tasks drove an increase in response length for perception tasks, suggesting that the model exhibits different reasoning patterns depending on the task. This reveals that different types of tasks may activate distinct cognitive pathways during the reinforcement learning process. A detailed analysis is provided in~\cref{sec:training_dynamics_analysis}.
%
% \begin{figure}[t]
%     % \hfill
%     
%     \centering
%         % \begin{subfigure}{0.24\textwidth}
%         %     \includegraphics[width=\linewidth]{images/figure5/various_iou_map_compare.pdf}
%         % \end{subfigure}
%     % \hfill
%         \begin{subfigure}{0.24\textwidth}
%             \includegraphics[width=\linewidth]{images/figure5/iou_50_99.pdf}
%         \end{subfigure}
%     % \hfill
%         \begin{subfigure}{0.24\textwidth}
%             \includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_coco.pdf}
%         \end{subfigure}
%     % \hfill
%         \begin{subfigure}{0.24\textwidth}
%             \includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_ovd.pdf}
%         \end{subfigure}
%     % \hfill        
%     \caption{Effectiveness of the Dynamic IoU Reward strategy on the 7B model. (Ablation conducted on a data subset of only detection and grounding tasks).}
%     \centering
%     \label{fig:dyn_iou}
%     \vspace{-10px}
% \end{figure}
%
\subsection{Ablation Study}
\label{ablation study}
%
% \begin{wrapfigure}{r}{0.65\textwidth}
%     \centering
%     \begin{subfigure}{0.25\textwidth}
%         \includegraphics[width=\linewidth]{images/figure6/7b_task.pdf}
%     \end{subfigure}
%     % \hfill % You can use \hspace{\fill} for spacing if needed
%     \begin{subfigure}{0.25\textwidth}
%         \includegraphics[width=\linewidth]{images/figure6/32b_lr.pdf}
%     \end{subfigure}
%     \caption{Ablation studies. (a) Various training strategies evaluated on the 7B model; (b) Different task compositions evaluated on the 7B model; (c) Effects of learning rates on the performance of the 32B model. Each figure shows Megabench-core performance over generation steps.}
%     \label{fig:abaltaion_study_wrap} 
% \end{wrapfigure}
%
\begin{figure}[t]
\vspace{-5px}
\centering
\begin{subfigure}{0.20\textwidth}
 \includegraphics[width=\linewidth]{images/figure6/7b_task.pdf}

\end{subfigure}
%
\begin{subfigure}{0.19\textwidth}

\includegraphics[width=\linewidth]{images/figure6/32b_lr.pdf}

\end{subfigure}
%
\begin{subfigure}{0.1925\textwidth}
\includegraphics[width=\linewidth]{images/figure5/iou_50_99.pdf}
\end{subfigure}
%
\begin{subfigure}{0.193\textwidth}
\includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_coco.pdf}
\end{subfigure}
%
\begin{subfigure}{0.20\textwidth}
\includegraphics[width=\linewidth]{images/figure5/iou99_vs_ioudyn_ovd.pdf}
\end{subfigure}

\caption{Ablation studies. (a) Different task compositions evaluated on the 7B model; (b) Effects of learning rates on the performance of the 32B model. (a-b) show Megabench-core performance over generation steps. (c-e) Effectiveness of the dynamic IoU reward strategy on the 7B model.}
\vspace{-10px}
% (Ablation conducted on a data subset of only detection and grounding tasks).

\centering

\label{fig:abaltaion_study}

\end{figure}

\noindent\textbf{Task-composition ablation}
%
As shown in~\cref{fig:abaltaion_study}a, training on both reasoning and perception data yields the strongest performance, reaching approximately 37.5. The reasoning-only data performs nearly as well but the peak performance is slightly lower, which suggests that the benchmark may prioritize logical competence over pure perception. Perception-only data consistently lags by 0.5–1.0 points but still shows steady improvement. The consistent performance hierarchy (Reasoning+Perception $>$ Reasoning $>$ Perception) underscores the value of mixed-task corpora: combining complementary signals leads to additive gains rather than diluted optimization.

\noindent\textbf{Learning-rate ablation}
For the Orsta-32B-0326 model (\cref{fig:abaltaion_study}b),  a learning rate of 1e-6 yields the highest and most stable plateau (45.5), while 1.5e-6 performs similarly until a mild degradation after 80 steps. Increasing the rate to 2e-6 causes a late-stage collapse to around 38, and 3e-6 diverges catastrophically after 50 steps, dropping below 36. This pattern suggests that larger models sit closer to the edge of the loss landscape, benefiting from small, stable updates, with 1e-6 offering the best trade-off between convergence speed and final performance on MEGABench.

\noindent\textbf{Reward strategy ablation}
%
Our ablation study on the reward strategy, conducted on a data subset containing only detection and grounding tasks, validates our dynamic IoU mechanism by revealing the clear limitations of fixed-threshold approaches.
%
\cref{fig:abaltaion_study}c, which evaluates fixed thresholds, highlights their inherent trade-off: a lenient IoU@50 reward proves unstable and leads to performance collapse in later stages, while a strict IoU@99 reward is stable but learns inefficiently. In contrast, subplots \cref{fig:abaltaion_study}d and \cref{fig:abaltaion_study}e demonstrate that our dynamic IoU reward consistently and significantly outperforms the strict IoU@99 baseline on the more challenging COCO multi-object and OVDEval negation subsets, proving its superior performance and learning efficiency.

{
\color{red}
\textbf{Extended Reward strategy ablation} We further justify our Dynamic IoU design ($0.85 \to 0.95 \to 0.99$) via more rigorous analysis (see~\cref{fig:iou99_vs_ioudyn_ovd_rebuttal} \&~\cref{appx:extended_dynamic_iou_schedule}). Comparisons with ""Loose" ($0.7 \to 0.8 \to 0.85$)  and "Strict" ($0.9 \to 0.95 \to 0.99$) variants demonstrate that our schedule optimally balances early-stage learnability (targeting an initial reward in a moderate range, e.g. 0.2-0.4) with late-stage precision enforcement (eliminating reward ambiguity), serving as a robust strategy aligned with the model's intrinsic learning trajectory.
}

% (a) An ablation on fixed IoU thresholds highlights their limitations: a lenient IoU@50 reward leads to unstable performance, while a strict IoU@99 reward results in inefficient learning. (b, c) In contrast, our Dynamic IoU reward consistently and significantly outperforms the strict IoU@99 baseline on the more challenging COCO multi-object and OVDEval negation subsets, demonstrating its superior performance and learning efficiency.
%
% To promote exploration while maintaining stability, we apply the clip-high strategy from DAPO~\citep{yu2025dapo} with clipping thresholds $\varepsilon_{\text{high}} = 0.28$ and $\varepsilon_{\text{low}} = 0.2$. This encourages low-probability token sampling without destabilizing training. No reference model is used; the final loss is computed solely via token-level mean PPO-clip loss.
%
% To further stabilize learning, the ViT and connector modules remain frozen throughout. Learning rates are set to $1 \times 10^{-6}$ (on-policy) and $5 \times 10^{-7}$ (off-policy), with a 5\% warmup before being held constant. During rollout, we use the vLLM engine with a temperature of 1.0, top-$p$ of 1.0, and a maximum sequence length of 2048. Greedy decoding is applied during testing.

%
% \begin{wrapfigure}{t}{0.400\textwidth} 
%   \centering
%   \includegraphics[width=\linewidth]{images/figure3/32b_0321_details.pdf}
%   \caption{\textbf{Training Trends of Orsta-32B-0321 on MEGA-Bench core.} The dark line denotes the overall MEGA-Bench Core, linking to the performance shown in~\cref{fig:mega_performance_track}.} 
%   \label{fig:32b_details}
%   % \vspace{-120pt}
% \end{wrapfigure}

% \begin{subfigure}{0.25\textwidth}
%     \includegraphics[width=\linewidth]{images/figure6/7b_strategy.pdf}
% % \caption{Model 7B}
% \end{subfigure}
% \begin{figure}[t]
%     \vspace{-5px}
%     \centering
%     % \hfill
%         \begin{subfigure}{0.25\textwidth}
%             \includegraphics[width=\linewidth]{images/figure6/7b_task.pdf}
%         \end{subfigure}
%     % \hfill
%         \begin{subfigure}{0.25\textwidth}
%                 \includegraphics[width=\linewidth]{images/figure6/32b_lr.pdf}
%         \end{subfigure}
%     \caption{Ablation studies. (a) Various training strategies evaluated on the 7B model; (b) Different task compositions evaluated on the 7B model; (c) Effects of learning rates on the performance of the 32B model. Each figure shows Megabench-core performance over generation steps.}
%     \centering
%     \label{fig:abaltaion_study}
%     \vspace{-5px}
% \end{figure}
% \noindent\textbf{Training-strategy ablation}
% As shown in~\cref{fig:abaltaion_study}~a, updating only the LLM stack raises the score from approximately 35 to 38 by step 120, indicating that reasoning weights are the primary driver of performance improvement. In contrast, tuning only the vision backbone results in negligible gains, with scores plateauing around 35.5. When both branches are optimized jointly, performance initially mirrors the LLM-only trajectory but slightly surpasses it in later stages (peaking at approximately 38.5).
%

% We compare two RL configurations, both trained for 3 epochs with a rollout batch size of 1024: (1) on-policy, and (2) off-policy with 8 optimization steps per rollout. All experiments use the GRPO algorithm, generating 8 candidate sequences per prompt.
%
%We adopt Group Relative Policy Optimization (GRPO)~\citep{shao2024deepseekmath}, following standard practice, but introduce two key modifications based on recent work~\citep{yu2025dapo, hu2025open}.
%
% First, we remove the reference model and its associated KL loss. This avoids restricting exploration~\citep{hu2025open} and prevents unstable KL divergence estimates~\citep{schulman2020klapprox}, while also reducing GPU memory usage and speeding up training.
% Second, we apply the clip-high trick and use token-level loss~\citep{yu2025dapo}, which help increase output entropy, encouraging better exploration and improving training stability.


==> sections/6_related_work.tex <==
\begin{table}[tb!]
\small

% --- 这里是您的“调节面板” ---

% 1. [行高] 大幅减小行高。1.0 为默认值，1.1 或 1.2 是比较紧凑的选择。
\renewcommand{\arraystretch}{1.1} 

% 2. [列间距] 设置一个更紧凑的列间距。可以尝试 2pt 到 4pt 之间的值。
\setlength{\tabcolsep}{3pt}      

\centering

\resizebox{\textwidth}{!}{%
% 不再使用 tabularx 和 scalebox，回归到原始的 tabular 环境
\begin{tabular}{
    @{} % 去掉表格左侧空白
    l  % 第一列(Model): 左对齐，现在它有更多空间了
    l  % 第二列(Size): 左对齐
    l  % 第三列(Backbone): 左对齐
    *{8}{c} % 中间8个任务列: 居中对齐
    l  % 最后一列(Others): 左对齐
    @{} % 去掉表格右侧空白
}
\toprule

% 3. [缩写标题] 将长标题极限缩写，这是节省空间的关键！
Model & Size & Backbone & Ma & Sc & Ch & Pu & OCR & DET & GND & CNT & Others \\

% 如果缩写还不够，可以考虑旋转标题（见下文注释）

\midrule
Visual-RFT~\citep{liu2025visual} & 2B & Qwen2-VL & - & - & - & - & - & \checkmark & \checkmark & - & CLS \\
DeepPerception~\citep{ma2025deepperception} & 2B & Qwen2-VL Base & - & - & - & - & - & - & - & - & S.QA \\
Vision-R1~\citep{huang2025vision} & 7B,72B & Qwen2.5-VL & \checkmark & \checkmark & - & - & - & - & - & - & - \\
R1-Onevision~\citep{yang2025r1} & 7B & Qwen2.5-VL & \checkmark & \checkmark & \checkmark & - & - & - & - & - & V.QA \\
Reason-RFT~\citep{tan2025reason} & 2B,7B & Qwen2-VL & \checkmark & - & - & - & - & - & - & \checkmark & S.QA \\
OThink-MR1~\citep{liu2025othink} & 2B,7B & Qwen2.5-VL & \checkmark & - & - & - & - & - & - & \checkmark & - \\
Perception-R1~\citep{yu2025perception} & 2B,3B & Qwen2 \& 2.5-VL & - & - & - & - & \checkmark & \checkmark & \checkmark & - & - \\
VLM-R1~\citep{shen2025vlm} & 3B & Qwen2.5-VL & - & - & - & - & - & \checkmark & \checkmark & - & - \\
MM-EUREKA~\citep{meng2025mm} & 7B,32B & Qwen2.5-VL & \checkmark & - & - & - & - & - & - & - & S.QA \\
VL-Rethinker~\citep{vl_rethinker} & 7B,32B,72B & Qwen2.5-VL & \checkmark & \checkmark & \checkmark & - & - & - & - & - & S.QA \\
\midrule
\textbf{Orsta (ours)} & 7B,32B & Qwen2.5-VL & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - \\
\bottomrule
\end{tabular}
}
\caption{Task-wise comparison with related works. The evaluated tasks include Math (Ma), Science (Sc), Chart (Ch), Puzzle (Pu), OCR, Detection (DET), Grounding (GND), Counting (CNT), Classification(CLS), Spatial question answering (S.QA), and Visual question answering (V.QA).} % Backbones marked with a star$^{*}$ indicate models trained from pre-trained backbone (i.e. zero-RL setting), while others are trained from instructed models.}
\label{tab:vlm-rl-comparble}
\vspace{-10px}
\end{table}
%
\section{Related Work}
%
Recent advancements in visual RL (summarized in~\cref{tab:vlm-rl-comparble}) have explored diverse strategies to enhance multimodal reasoning and perception. However, these efforts have largely bifurcated into two specialized tracks.
%
One major line of work has focused on enhancing visual reasoning. Models such as Vision-R1~\citep{huang2025vision}, LMM-R1~\citep{peng2025lmm}, R1-OneVision~\citep{yang2025r1}, VisualThinker-R1-Zero~\citep{zhou2025r1}, MM-Eureka~\citep{meng2025mm}, and PeBR~\citep{chen2025perception} primarily leverage reasoning-heavy datasets and rule-based signals to elicit complex problem-solving capabilities, closely mirroring RL paradigms from the LLM domain.

In parallel, another stream of research has applied RL to improve perception-intensive tasks. Models like Visual-RFT~\citep{liu2025visual}, R1-V~\citep{chen2025r1v}, Reason-RFT~\citep{tan2025reason}, and DeepPerception~\citep{ma2025deepperception} apply task-specific, verifiable reward signals for tasks like detection, grounding, and counting. Others, such as Seg-Zero~\citep{liu2025seg}, Perception-R1~\citep{yu2025perception}, and VLM-R1~\citep{shen2025vlm}, further propose tailored reward functions for segmentation and OCR, though they often remain within task-specific generalization boundaries.

Several approaches have also explored broader cross-task generalization. OThink-MR1~\citep{liu2025othink} incorporates GRPO with Dynamic KL, while VL-Rethinker~\citep{wang2025vl} introduces selective sample replay and forced rethinking to enhance reasoning. VisionReasoner~\citep{liu2025visionreasoner} reformulates diverse perception sub-tasks into a multi-goal problem, and Vision-G1~\citep{zha2025vision} introduces data curation strategies for diverse visual reasoning tasks.
%
In contrast to these prior efforts that largely treat reasoning and perception in isolation, our proposed V-Triune unifies both domains under a single, comprehensive RL system.


==> sections/7_conclusion.tex <==
\section{Discussion \& Future Work}

We presented V-Triune, a unified RL framework for jointly post-training VLMs on reasoning-heavy and perception-heavy tasks.
%
Its three coordinated components, together with Dynamic IoU for localization-centric tasks, make mixed-task RL training more modular, diagnosable, and stable.
%
Across both fair-budget comparisons and final-model evaluations, Orsta improves over its backbones on MEGA-Bench and a broad set of downstream benchmarks, while the same unified pipeline also extends to a new GUI domain.

Two future directions seem especially important.
%
One is to extend unified RL from static benchmark settings to multimodal agentic tool-use tasks.
%
The other is to generalize this training recipe beyond vision, toward joint RL training across speech, video, and text.


\section*{Reproducibility Statement}

Full details necessary for reproducibility are provided in the paper and supplementary materials.
%
The V-Triune framework is described in~\cref{sec:method}, with Dynamic IoU in~\cref{subsec:dynamic_iou}.
%
Model backbones, training data, and hyperparameters are given in~\cref{subsec:implementation details,subsec:data}, and engineering details are documented in~\cref{sec:training_recipe}.
%
Evaluation protocols for MEGA-Bench, COCO, and the other benchmarks are provided in~\cref{subsec:implementation details,sec:eval_details,sec:coco_evaluation}.
%
The full data schema is shown in~\cref{fig:data_curation,appx:data_schema}.
%
Anonymized code, model checkpoints, training scripts, and the curated dataset are included in the supplementary materials.

% To support full reproducibility of our results, we will publicly release all necessary components, including: (1) the trained models Orsta-7B, Orsta-32B-0321, and Orsta-32B-0326; (2) the complete 47.7K visual reasoning and perception training dataset; (3) the source code for V-Triune, our proposed framework; and (4) detailed documentation and running instructions covering environment setup, training procedures, and evaluation protocols. All materials will be made available under an open-source license upon publication.
% Notably, V-Triune yields Orsta-7B and Orsta-32B, with improvements of 3.2\% and 2.1\% over strong backbones, respectively. Our experiments indicate that reinforcement learning in VLMs primarily serves as an alignment strategy, refining the model’s decision-making and response behavior rather than enabling new knowledge acquisition. This supports the notion that RL fine-tuning enhances the utility and robustness of pre-trained VLMs without altering their foundational capabilities.


% We also acknowledge several limitations that merit further investigation:
% \begin{itemize}
%     \item \textbf{Limited performance scaling in perception tasks:} For visual reasoning tasks, we observe clear trends of increasing response length and reflection ratio as training progresses, akin to test-time scaling laws observed in LLMs. However, such trends are not evident in visual perception tasks. The underlying factors driving performance improvements in perception remain unclear. Exploring multi-step RL for perception tasks, similar to approaches in OpenAI’s o3, may offer new insights and avenues for progress.
%     
%     \item \textbf{Underexplored potential of RL-zero in VLMs:} There is currently limited research on RL-zero for vision-language models. Nonetheless, we see early indications that RL-zero has the potential to surpass the current limitations imposed by supervised fine-tuning (SFT). Given that multi-modal alignment remains a fundamental challenge in VLMs, and that supervised fine-tuning (SFT) may be inherently limited in addressing this issue, we believe that RL-zero has the potential to redefine the optimization paradigm and unlock new capabilities for vision-language models.
% 
% \end{itemize}

% The V-Triune system and Orsta models will be publicly available at \href{https://github.com/MiniMax-AI}{https://github.com/MiniMax-AI}. We hope this work inspires further research into reinforcement learning as a general-purpose training paradigm for vision-language understanding, and encourages exploration of richer reward schemes, advanced reasoning strategies, and task-specific adaptations.


==> sections_refined/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models, and has continued to improve model capabilities on complex reasoning and decision-making tasks.
%
Compared with text-only settings, however, RL training recipes for vision-language models (VLMs) remain much less mature.
%
Although an increasing number of works have begun to explore RL post-training in visual settings, clear, reproducible, and unified recipes for multimodal RL are still limited.
%
As multimodal models continue to move toward more general capabilities, enabling RL to scale stably over heterogeneous visual tasks is becoming an increasingly important problem.

For VLMs, the difficulty of this problem does not come simply from having more tasks, but from the need to handle both capability heterogeneity and verification heterogeneity within one training pipeline.
%
On the one hand, VLM post-training must cover both reasoning-heavy tasks and perception-heavy tasks, where the latter further include text recognition, counting, and spatial localization.
%
On the other hand, these tasks are verified in different ways: some can be checked with rule-based or symbolic matching, whereas localization tasks rely on continuous spatial feedback such as IoU.
%
Therefore, unified multimodal RL must not only deal with task diversity itself, but also support heterogeneous reward structures within the same optimization loop.

Existing work usually covers only part of this problem: some studies focus on visual reasoning tasks such as math and science QA~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker}, while others focus on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
By contrast, a clear and stable RL framework for jointly improving a single VLM on both high-level reasoning and fine-grained perception remains missing.

More concretely, this heterogeneity introduces three closely related obstacles for unified training.
%
First, different tasks, and sometimes even different samples within the same task, require different reward compositions and verifiers; once such logic is hard-coded into the training loop, the system quickly becomes brittle and difficult to scale.
%
Second, for localization tasks such as detection and grounding, a fixed IoU threshold creates two opposing problems: if the threshold is too loose, coarse predictions can receive similar rewards and the model lacks pressure to improve localization precision; if the threshold is too strict, rewards become too sparse and training becomes unstable.
%
Finally, in joint training, aggregated metrics often hide source-specific instability, reward degradation, or other training failures, making problems difficult to detect and diagnose in time.

To address these challenges, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a methodological framework for unified multimodal RL rather than a collection of task-specific tricks.
%
Specifically, V-Triune consists of three coordinated abstractions: sample-level reward routing (\S\ref{subsec:sample_level_formatting}), which explicitly binds reward configuration and verifier choice to each sample and thus enables unified routing across heterogeneous tasks; verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), which uses modular verifiers to support different forms of outcome checking, including our proposed Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}), a reward-shaping mechanism for localization tasks that progressively raises the IoU requirement to alleviate reward ambiguity under loose supervision and reward sparsity under strict supervision; and source-level diagnostics (\S\ref{subsec:metric_monitoring}), which provide fine-grained source-level observability for stability analysis and failure diagnosis.
%
Together, these three abstractions support unified training through data routing, outcome verification, and source-level diagnosis.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family, covering both 7B and 32B scales, and jointly optimize it on eight representative tasks under a single RL pipeline, including visual reasoning tasks such as mathematics, science, chart, and puzzle, as well as visual perception tasks such as detection, grounding, OCR, and counting.
%
Our experiments show that such unified training is not a zero-sum compromise: both reasoning and perception tasks benefit from joint training.
%
Concretely, Orsta achieves consistent improvements over its base models on MEGA-Bench Core~\citep{chen2024mega}, a comprehensive benchmark spanning over 440 diverse tasks for evaluating general VLM capability.
%
These gains further transfer to downstream benchmarks including MMMU, MathVista, COCO, and CountBench.
%
Taken together, these results suggest that V-Triune provides an effective and scalable RL path toward more general VLMs that integrate both reasoning and perception.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training from a multimodal RL perspective, and identify that its central difficulty comes not only from heterogeneous task families, but also from heterogeneous verification and reward structures.
%
Second, we propose V-Triune as a training framework for this setting, centered on sample-level reward routing, verifier-based outcome verification, Dynamic IoU reward shaping for localization tasks, and source-level diagnostics.
%
Third, we build the Orsta model family on top of this framework and validate its effectiveness through eight-task unified training, MEGA-Bench, broader reasoning and perception benchmarks, and task-mixture comparisons, showing that unified training is not a zero-sum compromise and that both task families benefit from joint optimization.


==> sections_refined/1_introduction_v2.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models.
%
Yet for vision-language models (VLMs), unified and reproducible recipes for multimodal RL remain limited.
%
As multimodal models move toward more general capabilities, enabling RL to scale stably across heterogeneous visual tasks is becoming an important problem.

For VLMs, this challenge is not simply about adding more tasks, but about handling both capability heterogeneity and verification heterogeneity within one pipeline.
%
Post-training must cover both reasoning-heavy and perception-heavy tasks, while their outcomes may require either rule-based checking or continuous spatial feedback such as IoU.
%
A unified multimodal RL pipeline must therefore support heterogeneous reward structures within the same optimization loop.

Existing work usually addresses only part of this problem, focusing either on visual reasoning~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker} or on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
A clear and stable RL framework for jointly improving a single VLM on both high-level reasoning and fine-grained perception remains missing.

This heterogeneity introduces three obstacles for unified training.
%
First, different tasks and even different samples can require different reward compositions and verifiers, and hard-coding such logic into the training loop quickly becomes brittle.
%
Second, for localization tasks such as detection and grounding, fixed IoU thresholds create two problems: loose thresholds blur reward differences between coarse predictions, whereas strict thresholds make rewards too sparse.
%
Third, aggregated metrics often hide source-specific instability, reward degradation, or other failures, making them difficult to detect and diagnose.

To address these challenges, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a framework for unified multimodal RL rather than a collection of task-specific tricks.
%
Specifically, V-Triune combines sample-level reward routing (\S\ref{subsec:sample_level_formatting}), verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), and source-level diagnostics (\S\ref{subsec:metric_monitoring}).
%
Within this framework, our Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}) serves as a reward-shaping mechanism for localization tasks by progressively increasing the IoU requirement to reduce reward ambiguity under loose supervision and reward sparsity under strict supervision.
%
Together, these abstractions support unified training through data routing, outcome verification, and source-level diagnosis.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family, covering both 7B and 32B scales, and jointly optimize it on eight representative tasks under a single RL pipeline, including mathematics, science, chart, puzzle, detection, grounding, OCR, and counting.
%
Our results show that unified training is not a zero-sum compromise: both reasoning and perception tasks benefit from joint training.
%
Orsta improves over its base models on MEGA-Bench Core~\citep{chen2024mega}, a benchmark spanning over 440 diverse tasks for general VLM capability, and these gains further transfer to MMMU, MathVista, COCO, and CountBench.
%
These results suggest that V-Triune provides an effective and scalable RL path toward more general VLMs.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training from a multimodal RL perspective and identify heterogeneous capabilities and heterogeneous verification as its central challenges.
%
Second, we propose V-Triune, centered on sample-level reward routing, verifier-based outcome verification, Dynamic IoU reward shaping for localization tasks, and source-level diagnostics.
%
Third, we build the Orsta family and validate the framework through eight-task unified training, MEGA-Bench, broader reasoning and perception benchmarks, and task-mixture comparisons, showing that both task families benefit from joint optimization.


==> sections_refined/1_introduction_v3.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models.
%
Compared with text-only settings, however, unified and reproducible recipes for multimodal RL remain much less mature.
%
Although more works have begun to explore RL post-training in visual settings, enabling RL to scale stably across heterogeneous visual tasks remains an important open problem for vision-language models (VLMs).

For VLMs, this challenge is not simply about adding more tasks, but about handling both capability heterogeneity and verification heterogeneity within one pipeline.
%
Post-training must cover both reasoning-heavy and perception-heavy tasks, where the latter further include text recognition, counting, and spatial localization.
%
Meanwhile, their outcomes are verified in different ways: some admit rule-based or symbolic checking, whereas localization tasks rely on continuous spatial feedback such as IoU.
%
Therefore, unified multimodal RL must not only deal with task diversity itself, but also support heterogeneous reward structures within the same optimization loop.

Existing work usually addresses only part of this problem, focusing either on visual reasoning~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker} or on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
A clear and stable RL framework for jointly improving a single VLM on both visual reasoning and fine-grained perception remains missing.

This heterogeneity introduces three obstacles for unified training.
%
First, different tasks, and even different samples, can require different reward compositions and verifiers, and hard-coding such logic into the training loop quickly becomes brittle and difficult to scale.
%
Second, for localization tasks such as detection and grounding, fixed IoU thresholds create two problems: loose thresholds blur reward differences between coarse predictions, whereas strict thresholds make rewards too sparse for stable learning.
%
Finally, in joint training, aggregated metrics often hide source-specific instability, reward degradation, or other failures, making them difficult to detect and diagnose in time.

To address these challenges, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a framework for unified multimodal RL rather than a collection of task-specific tricks.
%
V-Triune combines three coordinated abstractions: sample-level reward routing (\S\ref{subsec:sample_level_formatting}), verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), and source-level diagnostics (\S\ref{subsec:metric_monitoring}).
%
Within this framework, our Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}) serves as a reward-shaping mechanism for localization tasks by progressively increasing the IoU requirement to reduce reward ambiguity under loose supervision and reward sparsity under strict supervision.
%
Together, these abstractions support unified training through data routing, outcome verification, and source-level diagnosis.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family, covering both 7B and 32B scales, and jointly optimize it on eight representative tasks under a single RL pipeline, including reasoning tasks such as mathematics, science, chart, and puzzle, as well as perception tasks such as detection, grounding, OCR, and counting.
%
Our results show that unified training is not a zero-sum compromise: both reasoning and perception tasks benefit from joint training.
%
Orsta improves over its base models on MEGA-Bench Core~\citep{chen2024mega}, a comprehensive benchmark spanning over 440 diverse tasks for evaluating general VLM capability, and these gains further transfer to downstream benchmarks including MMMU, MathVista, COCO, and CountBench.
%
Taken together, these results suggest that V-Triune provides an effective and scalable RL path toward more general VLMs.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training from a multimodal RL perspective and identify heterogeneous capabilities and heterogeneous verification as its central challenges.
%
Second, we propose V-Triune, centered on sample-level reward routing, verifier-based outcome verification, Dynamic IoU reward shaping for localization tasks, and source-level diagnostics.
%
Third, we build the Orsta family and validate the framework through eight-task unified training, MEGA-Bench, broader reasoning and perception benchmarks, and task-mixture comparisons, showing that both task families benefit from joint optimization.


==> sections_refined/1_introduction_v4.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models~\citep{liu2025deepseek,team2025longcat,xiao2026mimo}.
%
Compared with text-only settings, however, unified and reproducible recipes for multimodal RL remain much less mature~\citep{qwen3.5,team2026kimi}.
%
Although more works have begun to explore RL post-training in visual settings~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}, enabling RL to scale stably across heterogeneous visual tasks remains an important open problem for vision-language models (VLMs).

For VLMs, this challenge is not simply about adding more tasks, but about handling both capability heterogeneity and verification heterogeneity within one pipeline.
%
Post-training must cover both reasoning-heavy and perception-heavy tasks, where the latter further include text recognition, counting, and spatial localization.
%
Meanwhile, their outcomes are verified in different ways: some admit rule-based or symbolic checking, whereas localization tasks rely on continuous spatial feedback such as IoU.
%
Therefore, unified multimodal RL must not only deal with task diversity itself, but also support heterogeneous reward structures within the same optimization loop.

Existing work usually addresses only part of this problem, focusing either on visual reasoning~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker} or on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
A clear and stable RL framework for jointly improving a single VLM on both high-level reasoning and fine-grained perception remains missing~\citep{}.

This heterogeneity introduces three obstacles for unified training.
%
First, different tasks, and even different samples, can require different reward compositions and verifiers, and hard-coding such logic into the training loop quickly becomes brittle and difficult to scale.
%
Second, for localization tasks such as detection and grounding, fixed IoU thresholds create two problems: loose thresholds blur reward differences between coarse predictions, whereas strict thresholds make rewards too sparse for stable learning.
%
Finally, in joint training, aggregated metrics often hide source-specific instability, reward degradation, or other failures, making them difficult to detect and diagnose in time.

To address these challenges, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a framework for unified multimodal RL rather than a collection of task-specific tricks.
%
V-Triune combines three coordinated abstractions: sample-level reward routing (\S\ref{subsec:sample_level_formatting}), which binds reward configuration and verifier choice to each sample; verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), which supports heterogeneous outcome checking through modular verifiers; and source-level diagnostics (\S\ref{subsec:metric_monitoring}), which expose source-specific failures hidden by aggregated metrics.
%
Within this framework, our Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}) serves as a reward-shaping mechanism for localization tasks by progressively increasing the IoU requirement to reduce reward ambiguity with loose thresholds and reward sparsity with strict ones.
%
Together, these abstractions support unified training through data routing, outcome verification, and source-level diagnosis.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family, covering both 7B and 32B scales, and jointly optimize it on eight representative tasks under a single RL pipeline, including reasoning tasks such as mathematics, science, chart, and puzzle, as well as perception tasks such as detection, grounding, OCR, and counting.
%
Our results show that unified training is not simply a trade-off: both reasoning and perception tasks benefit from joint training.
%
Orsta improves over its base models on MEGA-Bench Core~\citep{chen2024mega}, a comprehensive benchmark spanning over 440 diverse tasks for evaluating general VLM capability, and these gains further transfer to downstream benchmarks.
%
Taken together, these results suggest that V-Triune provides an effective and scalable RL path toward more general VLMs.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training from a multimodal RL perspective and identify heterogeneous capabilities and verification as its central challenges.
%
Second, we propose V-Triune, a unified training framework that routes heterogeneous rewards at the sample level, supports modular outcome verification, stabilizes localization learning through Dynamic IoU reward shaping, and enables source-level diagnosis.
%
Third, we build the Orsta family and validate the framework through eight-task unified training, MEGA-Bench, broader reasoning and perception benchmarks, and task-mixture comparisons.


==> sections_refined/1_introduction_v5.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models~\citep{liu2025deepseek,team2025longcat,xiao2026mimo}.
%
Compared with text-only settings, however, unified and reproducible recipes for multimodal RL remain much less mature~\citep{qwen3.5,team2026kimi}.
%
Although more works have begun to explore RL post-training in visual settings~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}, enabling RL to scale stably across heterogeneous visual tasks remains an important open problem for vision-language models (VLMs).

For VLMs, this challenge is not simply about adding more tasks, but about handling both capability and verification heterogeneity within one pipeline.
%
Post-training must cover both reasoning-heavy and perception-heavy tasks, while their outcomes may require symbolic checking or continuous spatial feedback such as IoU.
%
Unified multimodal RL therefore needs to support heterogeneous reward structures within the same optimization loop.

Existing work usually addresses only part of this problem, focusing either on visual reasoning~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker} or on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
A clear and stable RL framework for jointly improving a single VLM on both high-level reasoning and fine-grained perception remains missing.

This heterogeneity introduces three obstacles for unified training.
%
First, different tasks, and even different samples, can require different reward compositions and verifiers, and hard-coding such logic into the training loop quickly becomes brittle and difficult to scale.
%
Second, for localization tasks such as detection and grounding, fixed IoU thresholds create two problems: loose thresholds blur reward differences between coarse predictions, whereas strict thresholds make rewards too sparse for stable learning.
%
Finally, in joint training, aggregated metrics often hide source-specific instability, reward degradation, or other failures, making them difficult to detect and diagnose in time.

To address these challenges, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a unified multimodal RL framework for heterogeneous visual tasks.
%
V-Triune combines three coordinated abstractions: sample-level reward routing (\S\ref{subsec:sample_level_formatting}), which binds reward configuration and verifier choice to each sample; verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), which supports heterogeneous outcome checking through modular verifiers; and source-level diagnostics (\S\ref{subsec:metric_monitoring}), which expose source-specific failures hidden by aggregated metrics.
%
Within this framework, our Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}) serves as a reward-shaping mechanism for localization tasks by progressively increasing the IoU requirement to reduce reward ambiguity with loose thresholds and reward sparsity with strict ones.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family, covering both 7B and 32B scales, and jointly optimize it on eight representative tasks under a single RL pipeline, including reasoning tasks such as mathematics, science, chart, and puzzle, as well as perception tasks such as detection, grounding, OCR, and counting.
%
Our results show that unified training can benefit both reasoning and perception within a single RL pipeline.
%
Orsta improves over its base models on MEGA-Bench~\citep{chen2024mega}, a comprehensive benchmark spanning over 440 diverse tasks for evaluating general VLM capability, and these gains further transfer to downstream benchmarks.
%
Taken together, these results suggest that V-Triune provides an effective and scalable RL path toward more general VLMs.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training as a heterogeneous multimodal RL problem and identify capability and verification heterogeneity as its central challenges.
%
Second, we propose V-Triune, a unified training framework built on three coordinated abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics, with Dynamic IoU reward shaping for localization tasks.
%
Third, we build the Orsta family and validate the framework through eight-task unified training, fair-budget mixture comparisons, MEGA-Bench evaluation, broader reasoning and perception benchmarks, and extension to a new GUI task domain.


==> sections_refined/1_introduction_v6.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models~\citep{liu2025deepseek,team2025longcat,xiao2026mimo}.
%
Compared with text-only settings, however, public and reproducible recipes for multimodal RL remain much less mature~\citep{qwen3.5,team2026kimi}.
%
Although more works have begun to explore RL post-training in visual settings~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}, a stable recipe for scaling RL across heterogeneous visual tasks remains an important open problem for vision-language models (VLMs).
%
For VLMs, this challenge is not simply about adding more tasks, but about handling both capability and verification heterogeneity within one pipeline.
%
Post-training must cover both reasoning-heavy and perception-heavy tasks, while their outcomes may require symbolic checking or continuous spatial feedback such as IoU.
%
A unified multimodal RL recipe must therefore support heterogeneous reward structures and verification regimes within the same optimization loop.

Existing work usually addresses only part of this problem, focusing either on visual reasoning~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker} or on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
A clear and stable RL framework for jointly improving a single VLM on both high-level reasoning and fine-grained perception remains missing.

This heterogeneity creates three recurring failure modes for unified training.
%
First, different tasks, and even different samples, can require different reward compositions and verifiers, and hard-coding such logic into the training loop quickly becomes brittle and difficult to scale.
%
Second, for localization tasks such as detection and grounding, fixed IoU thresholds create two problems: loose thresholds blur reward differences between coarse predictions, whereas strict thresholds make rewards too sparse for stable learning.
%
Finally, in joint training, aggregated metrics often hide source-specific instability, reward degradation, or other failures, making them difficult to detect and diagnose in time.

To address these failure modes, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a training methodology for unified multimodal RL over heterogeneous visual tasks.
%
V-Triune is built around three coordinated abstractions, each addressing one blocker in unified RL: sample-level reward routing (\S\ref{subsec:sample_level_formatting}), which decouples reward composition and verifier choice from the trainer core; verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), which provides a common interface for heterogeneous outcome rewarding; and source-level diagnostics (\S\ref{subsec:metric_monitoring}), which expose source-specific failures hidden by aggregated metrics.
%
Within this methodology, our Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}) serves as a localization-specific reward-shaping mechanism by progressively increasing the IoU requirement, avoiding both reward ambiguity under loose thresholds and reward sparsity under strict ones.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family, covering both 7B and 32B scales, and jointly optimize it on eight representative tasks under a single RL pipeline, including reasoning tasks such as mathematics, science, chart, and puzzle, as well as perception tasks such as detection, grounding, OCR, and counting.
%
Under matched budgets, unified training matches or outperforms specialist mixtures and improves both reasoning and perception within a single RL pipeline.
%
Orsta improves over its base models on MEGA-Bench~\citep{chen2024mega}, a comprehensive benchmark spanning over 440 diverse tasks for evaluating general VLM capability, and these gains further transfer to downstream benchmarks.
%
Taken together, these results suggest that V-Triune provides an effective and scalable RL path toward more general VLMs.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training as a heterogeneous multimodal RL problem and identify three recurring failure modes: rigid reward interfaces, localization reward ambiguity versus sparsity, and lack of source-level observability.
%
Second, we propose V-Triune, a training methodology built on three coordinated abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics, with Dynamic IoU reward shaping for localization tasks.
%
Third, we build the Orsta family and validate the framework through eight-task unified training, matched-budget mixture comparisons, MEGA-Bench evaluation, broader reasoning and perception benchmarks, and extension to a new GUI task domain.


==> sections_refined/1_introduction_v7.tex <==
\section{Introduction}
\label{sec:intro}

Reinforcement learning (RL) is becoming an important direction for post-training foundation models~\citep{liu2025deepseek,team2025longcat,xiao2026mimo}.
%
Compared with text-only settings, however, public and reproducible recipes for multimodal RL remain much less mature~\citep{qwen3.5,team2026kimi}.
%
Although more works have begun to explore RL post-training in visual settings~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}, a stable recipe for scaling RL across heterogeneous visual tasks remains an important open problem for vision-language models (VLMs).

For VLMs, this challenge is not simply about adding more tasks, but about handling both capability heterogeneity and verification heterogeneity within one pipeline.
%
Post-training must cover both reasoning-heavy and perception-heavy tasks, while their outcomes may require symbolic checking or continuous spatial feedback such as IoU.
%
A unified multimodal RL recipe must therefore support heterogeneous reward structures and verification regimes within the same optimization loop.

Existing work usually addresses only part of this problem, focusing either on visual reasoning~\citep{huang2025vision,yang2025r1,meng2025mm,vl_rethinker} or on perception tasks such as detection and grounding~\citep{liu2025visual,ma2025deepperception,tan2025reason,liu2025othink,shen2025vlm,wang2025vl,yu2025perception,liu2025visionreasoner}.
%
A clear and stable RL framework for jointly improving a single VLM on both high-level reasoning and fine-grained perception remains missing.

In practice, unified multimodal RL breaks down for three concrete reasons.
%
First, different tasks, and even different samples, can require different reward compositions and verifiers, so hard-coding this logic into the trainer quickly becomes brittle and difficult to scale.
%
Second, for localization tasks such as detection and grounding, fixed IoU thresholds create two failure modes: loose thresholds blur reward differences between coarse predictions, whereas strict thresholds make rewards too sparse for stable learning.
%
Third, in joint training, aggregate metrics often hide source-specific instability, reward degradation, or other failures, making them difficult to detect and diagnose in time.

To address these blockers, we introduce \textbf{V}isual \textbf{Tri}ple \textbf{U}nified Rei\textbf{n}forcement L\textbf{e}arning (V-Triune), a training methodology for unified multimodal RL over heterogeneous visual tasks.
%
V-Triune organizes unified training around three coordinated abstractions: sample-level reward routing (\S\ref{subsec:sample_level_formatting}), which decouples reward composition and verifier choice from the trainer core; verifier-level outcome verification (\S\ref{subsec:verifier_level_reward_computation}), which provides a common interface for heterogeneous rewarding; and source-level diagnostics (\S\ref{subsec:metric_monitoring}), which expose source-specific failures hidden by aggregated metrics.
%
Within this methodology, Dynamic IoU Reward (\S\ref{subsec:dynamic_iou}) serves as a localization-specific reward-shaping mechanism by progressively increasing the IoU requirement, avoiding both reward ambiguity under loose thresholds and reward sparsity under strict ones.

Built on V-Triune, we develop the Orsta (\textbf{O}ne \textbf{R}L to \textbf{S}ee \textbf{T}hem \textbf{A}ll) model family at both 7B and 32B scales and jointly train these models on eight representative tasks under a single RL pipeline, including reasoning tasks such as mathematics, science, chart, and puzzle, as well as perception tasks such as detection, grounding, OCR, and counting.
%
Under matched budgets, unified training matches or outperforms specialist mixtures and improves both reasoning and perception within a single RL pipeline.
%
Orsta improves over its base models on MEGA-Bench~\citep{chen2024mega}, a comprehensive benchmark spanning over 440 diverse tasks for evaluating general VLM capability, and these gains further transfer to downstream benchmarks.
%
Taken together, these results suggest that V-Triune provides an effective and practical recipe for joint RL post-training of reasoning and perception in open VLMs.

Our main contributions are threefold.
%
First, we formulate unified VLM post-training as a heterogeneous multimodal RL problem and identify three practical blockers: rigid reward interfaces, the ambiguity-versus-sparsity trade-off in localization rewards, and lack of source-level observability during joint training.
%
Second, we propose V-Triune, a training methodology built on sample-level reward routing, verifier-level outcome verification, and source-level diagnostics, together with Dynamic IoU reward shaping for localization tasks.
%
Third, we instantiate this recipe in the Orsta family and validate it through eight-task unified training, matched-budget specialist comparisons, MEGA-Bench evaluation, broader reasoning and perception benchmarks, and extension to a new GUI task domain.


==> sections_refined/3_method_v1.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/figure2_v13.pdf}
    \caption{\textbf{Overview of V-Triune.} The framework organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. Together they support mixed-task training across reasoning-heavy and perception-heavy tasks, while Dynamic IoU provides precision-oriented reward shaping for localization-centric tasks.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}
%
This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models. The central question is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline. The main difficulty is not merely that the task set is broad, but that different tasks simultaneously introduce different reward interfaces, different outcome verification regimes, and different observability requirements during training.
%
More concretely, this setting raises three coupled challenges. First, heterogeneous tasks do not naturally fit a rigid shared reward interface; once reward computation and routing logic are written directly into the trainer, the training loop quickly becomes brittle, hard to extend, and hard to analyze. Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds: loose thresholds blur the distinction between coarse predictions, while strict thresholds make rewards too sparse early in training. Third, in joint training, aggregated metrics can hide source-specific collapse, reward degradation, task overshadowing, or abnormal generation behavior, making failures difficult to localize.
%
V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}. Sample-level reward routing binds reward composition and subsequent verification to each sample. Verifier-level outcome verification provides a shared interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks. Source-level diagnostics expose training dynamics that are invisible under aggregate-only monitoring. Together, these abstractions define the routing, verification, and diagnosis layers of our unified RL framework.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}
%
The first requirement for unified multimodal RL is a reward interface that can accommodate heterogeneous tasks without entangling task-specific branches inside the training loop. In our setting, samples differ not only in objective, but also in reward type: some require discrete rule-based supervision, while others rely on continuous spatial feedback such as IoU. Some need only an accuracy reward, whereas others require a joint reward over accuracy and output format. If these cases are hard-coded into the trainer, the resulting system becomes tightly coupled and increasingly difficult to maintain as tasks are added.
%
V-Triune therefore makes reward routing explicit at the sample level. Each sample specifies its reward components, their relative weights, and its subsequent verification path through a unified interface. The trainer consumes this common structure and no longer needs task-specific reward branches in the main update loop. In effect, reward routing is encoded in the sample metadata rather than hard-coded throughout the trainer.
%
Concretely, in addition to common inputs such as \texttt{images} and \texttt{prompt}, we attach a small set of task-agnostic metadata for reward routing. The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} specify the relative weights of reward components, supporting accuracy-only and accuracy-plus-format settings within one pipeline. The \texttt{verifier} field determines which verifier should process the sample, providing the entry point for the verifier-level interface described in~\cref{subsec:verifier_level_reward_computation}. Finally, \texttt{data\_source} records the sample origin and later serves as the indexing key for source-level diagnostics in~\cref{subsec:metric_monitoring}. The full data format is shown in~\cref{fig:data_format}.
%
This design matters in three ways. First, it decouples heterogeneous reward interfaces from the trainer, allowing mixed task families to coexist in one RL run. Second, it defines a clean extensibility boundary: adding a new task only requires preparing data, attaching the appropriate metadata, and selecting a compatible verifier, without rewriting the trainer itself. We later validate this extensibility by adding a new GUI task domain in an extension experiment. Third, the same sample-level metadata provides the structural basis for source-aware diagnosis, since rewards and behaviors can be regrouped by source after verification. For V-Triune, sample-level formatting is therefore best viewed as a reward routing abstraction rather than a data format alone.
%
\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}
%
Sample-level routing determines where each sample should go, but unified training still requires a common way to handle heterogeneous outcome verification. Some tasks have outcomes that can be checked with deterministic rules after parsing the model output, while others require continuous spatial evaluation. V-Triune addresses this by defining reward computation at the verifier level: the trainer does not implement task-specific reward logic directly, but instead sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation within a shared interface.
%
This abstraction isolates heterogeneous outcome verification from the training loop. What must be unified is not a single reward function for all tasks, but a single verifier interface through which different reward logics can be routed, executed, and returned. In implementation, we support this design with an asynchronous client-server architecture that scales reward computation independently of the trainer. Methodologically, however, the key contribution is the verifier abstraction itself rather than the deployment pattern.
%
In this work we primarily instantiate two verifiers, corresponding to two verification regimes.
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.
%
\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.
%
For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.
%
From the perspective of unified multimodal RL, verifier-level computation establishes a clear boundary: different task families preserve their own deterministic reward logic, while the trainer only interacts with a shared verifier interface. The same boundary also reduces the marginal cost of extension. For new task domains that can reuse an existing output structure and verification regime, the RL pipeline remains unchanged and only the data routing needs to be updated. We later verify this point with an added GUI task domain in an extension experiment.
%
\subsubsection{Dynamic IoU Reward in DetectionVerifier}
\label{subsec:dynamic_iou}
%
Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemmag
%
With a loose threshold such as IoU@50, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.
%
To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively tightens the IoU requirement, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.
%
Dynamic IoU should therefore be understood as a targeted reward shaping mechanism for localization-centric RL. Its role is to make high-precision localization learnable under joint training, rather than to serve as an arbitrary heuristic schedule. We provide the exact thresholds and stage boundaries in the implementation details, and further compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}
%
Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that are difficult to see. Different sources may have different data quality, reward regimes, and generation behaviors, yet aggregated metrics expose only an averaged global trend. As a result, source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden. Unified multimodal RL therefore requires source-level observability.
%
Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity. The point is not simply to record more metrics, but to make hidden failure modes visible. We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics. Together they track whether the correct reward is being learned, whether generation behavior is drifting, whether different task families develop different response strategies, and whether perception-specific indicators reveal additional issues.
%
The \textit{Training Reward} metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward, making it possible to distinguish genuine progress from source-specific degradation. \textit{Response Behavior} metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse. \textit{Reflection} metrics offer a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is provided in~\cref{appx:reflection_metrics}. Finally, \textit{Auxiliary Metrics} include fixed-threshold IoU, mAP, and representative responses for qualitative inspection.
%
Crucially, these diagnostics are methodologically useful rather than merely descriptive. They directly helped identify several failure modes that matter for unified training, including ViT gradient explosion, leaked image special tokens, and the divergence of response patterns across task families. They also support later analysis of task interaction by showing whether reasoning-heavy and localization-heavy tasks converge to a shared response strategy or to distinct ones. Just as importantly, source-level signals reveal when one source or task family is being overshadowed by stronger training signals elsewhere. Our later stability analysis and training-dynamics results provide direct evidence for the necessity of this diagnostic layer.
%
Source-level diagnostics therefore form the third core abstraction of V-Triune: they make unified training not only executable, but diagnosable. This is essential in heterogeneous multimodal RL, where failures rarely manifest uniformly across all tasks and sources.


==> sections_refined/3_method_v2.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/figure2_v13.pdf}
    \caption{\textbf{Overview of V-Triune.} The framework organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. Together they support mixed-task training across reasoning-heavy and perception-heavy tasks, while Dynamic IoU provides precision-oriented reward shaping for localization-centric tasks.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}
%
This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models. The central question is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline. The main difficulty is not merely that the task set is broad, but that different tasks simultaneously introduce different reward interfaces, different outcome verification regimes, and different observability requirements during training.
%
More concretely, this setting raises three coupled challenges. First, heterogeneous tasks do not naturally fit a rigid shared reward interface; once reward computation and routing logic are written directly into the trainer, the training loop quickly becomes brittle, hard to extend, and hard to analyze. Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds: loose thresholds blur the distinction between coarse predictions, while strict thresholds make rewards too sparse early in training. Third, in joint training, aggregated metrics can hide source-specific collapse, reward degradation, task overshadowing, or abnormal generation behavior, making failures difficult to localize.
%
V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}. Sample-level reward routing binds reward composition and subsequent verification to each sample. Verifier-level outcome verification provides a shared interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks. Source-level diagnostics expose training dynamics that are invisible under aggregate-only monitoring. Together, these abstractions define the routing, verification, and diagnosis layers of our unified RL framework.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}
%
The first requirement for unified multimodal RL is a reward interface that can accommodate heterogeneous tasks without entangling task-specific branches inside the training loop. In our setting, samples differ not only in objective, but also in reward type: some require discrete rule-based supervision, while others rely on continuous spatial feedback such as IoU. Some need only an accuracy reward, whereas others require a joint reward over accuracy and output format. If these cases are hard-coded into the trainer, the resulting system becomes tightly coupled and increasingly difficult to maintain as tasks are added.
%
V-Triune therefore makes reward routing explicit at the sample level. Each sample specifies its reward components, their relative weights, and its subsequent verification path through a unified interface. The trainer consumes this common structure and no longer needs task-specific reward branches in the main update loop. In effect, reward routing is encoded in the sample metadata rather than hard-coded throughout the trainer.
%
Concretely, in addition to common inputs such as \texttt{images} and \texttt{prompt}, we attach a small set of task-agnostic metadata for reward routing. The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} specify the relative weights of reward components, supporting accuracy-only and accuracy-plus-format settings within one pipeline. The \texttt{verifier} field determines which verifier should process the sample, providing the entry point for the verifier-level interface described in~\cref{subsec:verifier_level_reward_computation}. Finally, \texttt{data\_source} records the sample origin and later serves as the indexing key for source-level diagnostics in~\cref{subsec:metric_monitoring}. The full data format is shown in~\cref{fig:data_format}.
%
This design matters in three ways. First, it decouples heterogeneous reward interfaces from the trainer, allowing mixed task families to coexist in one RL run. Second, it defines a clean extensibility boundary: adding a new task only requires preparing data, attaching the appropriate metadata, and selecting a compatible verifier, without rewriting the trainer itself. We later validate this extensibility by adding a new GUI task domain in an extension experiment. Third, the same sample-level metadata provides the structural basis for source-aware diagnosis, since rewards and behaviors can be regrouped by source after verification. For V-Triune, sample-level formatting is therefore best viewed as a reward routing abstraction rather than a data format alone.
%
\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}
%
Sample-level routing determines where each sample should go, but unified training still requires a common way to handle heterogeneous outcome verification. Some tasks have outcomes that can be checked with deterministic rules after parsing the model output, while others require continuous spatial evaluation. V-Triune addresses this by defining reward computation at the verifier level: the trainer does not implement task-specific reward logic directly, but instead sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation within a shared interface.
%
This abstraction isolates heterogeneous outcome verification from the training loop. What must be unified is not a single reward function for all tasks, but a single verifier interface through which different reward logics can be routed, executed, and returned. In implementation, we support this design with an asynchronous client-server architecture that scales reward computation independently of the trainer. Methodologically, however, the key contribution is the verifier abstraction itself rather than the deployment pattern.
%
In this work we primarily instantiate two verifiers, corresponding to two verification regimes.
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.
%
\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.
%
For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.
%
From the perspective of unified multimodal RL, verifier-level computation establishes a clear boundary: different task families preserve their own deterministic reward logic, while the trainer only interacts with a shared verifier interface. The same boundary also reduces the marginal cost of extension. For new task domains that can reuse an existing output structure and verification regime, the RL pipeline remains unchanged and only the data routing needs to be updated. We later verify this point with an added GUI task domain in an extension experiment.
%
\subsubsection{Dynamic IoU Reward in DetectionVerifier}
\label{subsec:dynamic_iou}
%
Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemma.
%
With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.
%
To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively tightens the IoU requirement, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.
%
Dynamic IoU should therefore be understood as a targeted reward shaping mechanism for localization-centric RL. Its role is to make high-precision localization learnable under joint training, rather than to serve as an arbitrary heuristic schedule. We provide the exact thresholds and stage boundaries in the implementation details, and further compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}
%
Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that are difficult to see. Different sources may have different data quality, reward regimes, and generation behaviors, yet aggregated metrics expose only an averaged global trend. As a result, source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden. Unified multimodal RL therefore requires source-level observability.
%
Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity. The point is not simply to record more metrics, but to make hidden failure modes visible. We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics. Together they track whether the correct reward is being learned, whether generation behavior is drifting, whether different task families exhibit different response-length and reflection patterns, and whether perception-specific indicators reveal additional issues.
%
The \textit{Training Reward} metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward, making it possible to distinguish genuine progress from source-specific degradation. \textit{Response Behavior} metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse. These signals are especially informative because different task families may benefit from different generation patterns: longer reasoning traces are often useful for reasoning-heavy tasks, whereas concise responses are often more effective for localization-centric perception tasks~\citep{li2025think}. We therefore track response length at the source level to examine whether unified training preserves task-appropriate behaviors across tasks. \textit{Reflection} metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is provided in~\cref{appx:reflection_metrics}. Finally, \textit{Auxiliary Metrics} include fixed-threshold IoU, mAP, and representative responses for qualitative inspection.
%
Crucially, these diagnostics are methodologically useful rather than merely descriptive. They directly helped identify several failure modes that matter for unified training, including ViT gradient explosion and leaked image special tokens~(\cref{sec:training_recipe}), as well as divergent response-length and reflection patterns across task families~(\cref{sec:training_dynamics_analysis}). These source-level diagnostics also support later analysis of task interaction by revealing whether unified training preserves task-appropriate behaviors or instead pushes different task families toward the same generation pattern. They further reveal when one source or task family is being overshadowed by stronger training signals elsewhere. Our later stability analysis and training-dynamics results provide direct evidence for the necessity of this diagnostic mechanism.
%
Source-level diagnostics therefore form the third core abstraction of V-Triune: they make unified training not only executable, but diagnosable. This is essential in heterogeneous multimodal RL, where failures rarely manifest uniformly across all tasks and sources.


==> sections_refined/3_method_v3.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/figure2_v13.pdf}
    \caption{\textbf{Overview of V-Triune.} The framework organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. Together they support mixed-task training across reasoning-heavy and perception-heavy tasks, while Dynamic IoU provides precision-oriented reward shaping for localization-centric tasks.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}
%
This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models. The central question is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline. The main difficulty is not merely that the task set is broad, but that different tasks simultaneously introduce different reward interfaces, different outcome verification regimes, and different observability requirements during training.
%
More concretely, this setting raises three coupled challenges. First, heterogeneous tasks do not naturally fit a rigid shared reward interface; once reward computation and routing logic are written directly into the trainer, the training loop quickly becomes brittle, hard to extend, and hard to analyze. Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds: loose thresholds blur the distinction between coarse predictions, while strict thresholds make rewards too sparse early in training. Third, in joint training, aggregated metrics can hide source-specific collapse, reward degradation, task overshadowing, or abnormal generation behavior, making failures difficult to localize.
%
V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}. Sample-level reward routing binds reward composition and subsequent verification to each sample. Verifier-level outcome verification provides a shared interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks. Source-level diagnostics expose training dynamics that are invisible under aggregate-only monitoring. Together, these abstractions define the routing, verification, and diagnosis layers of our unified RL framework.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}
%
The first requirement for unified multimodal RL is a reward interface that can accommodate heterogeneous tasks without entangling task-specific branches inside the training loop. In our setting, samples differ not only in objective, but also in reward type: some require discrete rule-based supervision, while others rely on continuous spatial feedback such as IoU. Some need only an accuracy reward, whereas others require a joint reward over accuracy and output format. If these cases are hard-coded into the trainer, the resulting system becomes tightly coupled and increasingly difficult to maintain as tasks are added.
%
V-Triune therefore makes reward routing explicit at the sample level. Each sample specifies its reward components, their relative weights, and its subsequent verification path through a unified interface. The trainer consumes this common structure and no longer needs task-specific reward branches in the main update loop. In effect, reward routing is encoded in the sample metadata rather than hard-coded throughout the trainer.
%
Concretely, in addition to common inputs such as \texttt{images} and \texttt{prompt}, we attach a small set of task-agnostic metadata for reward routing. The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} specify the relative weights of reward components, supporting accuracy-only and accuracy-plus-format settings within one pipeline. The \texttt{verifier} field determines which verifier should process the sample, providing the entry point for the verifier-level interface described in~\cref{subsec:verifier_level_reward_computation}. Finally, \texttt{data\_source} records the sample origin and later serves as the indexing key for source-level diagnostics in~\cref{subsec:metric_monitoring}. The full data format is shown in~\cref{fig:data_format}.
%
This design decouples heterogeneous reward interfaces from the trainer, allowing mixed task families to coexist in one RL run. It also defines a clean extensibility boundary: adding a new task only requires preparing data, attaching the appropriate metadata, and selecting a compatible verifier, without rewriting the trainer itself. We later validate this extensibility by adding a new GUI task domain in an extension experiment. The same sample-level metadata also provides the structural basis for source-aware diagnosis, since rewards and behaviors can be regrouped by source after verification. In V-Triune, sample-level formatting functions as a reward routing abstraction rather than a data format alone.
%
\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}
%
Sample-level routing determines where each sample should go, but unified training still requires a common way to handle heterogeneous outcome verification. Some tasks have outcomes that can be checked with deterministic rules after parsing the model output, while others require continuous spatial evaluation. V-Triune addresses this by defining reward computation at the verifier level: the trainer does not implement task-specific reward logic directly, but instead sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation within a shared interface.
%
This abstraction isolates heterogeneous outcome verification from the training loop. What must be unified is not a single reward function for all tasks, but a single verifier interface through which different reward logics can be routed, executed, and returned. In implementation, we support this design with an asynchronous client-server architecture that scales reward computation independently of the trainer. The key point, however, is the verifier abstraction itself rather than the deployment pattern.
%
In this work we primarily instantiate two verifiers, corresponding to two verification regimes.
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.
%
\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.
%
For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.
%
From the perspective of unified multimodal RL, verifier-level computation establishes a clear boundary: different task families preserve their own deterministic reward logic, while the trainer only interacts with a shared verifier interface. The same boundary also reduces the marginal cost of extension. For new task domains that can reuse an existing output structure and verification regime, the RL pipeline remains unchanged and only the data routing needs to be updated. We later verify this point with an added GUI task domain in an extension experiment.
%
\subsubsection{Dynamic IoU Reward in DetectionVerifier}
\label{subsec:dynamic_iou}
%
Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemma.
%
With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.
%
To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively tightens the IoU requirement, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.
%
Dynamic IoU makes high-precision localization learnable under joint training. It is designed for localization-centric RL, where a fixed threshold is either too loose to refine localization or too strict to bootstrap learning. We provide the exact thresholds and stage boundaries in the implementation details, and further compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}
%
Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that are difficult to see. Different sources may have different data quality, reward regimes, and generation behaviors, yet aggregated metrics expose only an averaged global trend. As a result, source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden. Unified multimodal RL therefore requires source-level observability.
%
Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity. The point is not simply to record more metrics, but to make hidden failure modes visible. We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics. Together they track whether the correct reward is being learned, whether generation behavior is drifting, whether different task families exhibit different response-length and reflection patterns, and whether perception-specific indicators reveal additional issues.
%
The \textit{Training Reward} metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward, making it possible to distinguish genuine progress from source-specific degradation. \textit{Response Behavior} metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse. These signals are especially informative because different task families may benefit from different generation patterns: longer reasoning traces are often useful for reasoning-heavy tasks, whereas concise responses are often more effective for localization-centric perception tasks~\citep{li2025think}. We therefore track response length at the source level to examine whether unified training preserves task-appropriate behaviors across tasks. \textit{Reflection} metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is provided in~\cref{appx:reflection_metrics}. Finally, \textit{Auxiliary Metrics} include fixed-threshold IoU, mAP, and representative responses for qualitative inspection.
%
These diagnostics do more than summarize training. They helped identify several failure modes that matter for unified training, including ViT gradient explosion and leaked image special tokens~(\cref{sec:training_recipe}), as well as divergent response-length and reflection patterns across task families~(\cref{sec:training_dynamics_analysis}). These source-level diagnostics also support later analysis of task interaction by revealing whether unified training preserves task-appropriate behaviors or instead pushes different task families toward the same generation pattern. They further reveal when one source or task family is being overshadowed by stronger training signals elsewhere. Our later stability analysis and training-dynamics results provide direct evidence for the necessity of this diagnostic mechanism.
%
Source-level diagnostics form the third core abstraction of V-Triune: they make unified training not only executable, but diagnosable. This is essential in heterogeneous multimodal RL, where failures rarely manifest uniformly across all tasks and sources.


==> sections_refined/3_method_v4.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/figure2_v15.pdf}
    \caption{\textbf{Overview of V-Triune.} The framework organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. Together they support mixed-task training across reasoning-heavy and perception-heavy tasks, while Dynamic IoU provides precision-oriented reward shaping for localization-centric tasks.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}

This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models. The central problem is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline. The difficulty is not only task diversity itself, but also the fact that different tasks bring different reward interfaces, outcome verification regimes, and observability requirements.

This setting raises three coupled challenges. First, heterogeneous tasks do not fit a rigid shared reward interface; if reward computation and routing are written directly into the trainer, the training loop quickly becomes brittle and hard to extend. Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds: loose thresholds blur the distinction between coarse predictions, while strict thresholds make rewards too sparse early in training. Third, aggregated metrics can hide source-specific collapse, reward degradation, task overshadowing, or abnormal generation behavior, making failures difficult to localize.

V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}. Sample-level reward routing binds reward composition and subsequent verification to each sample. Verifier-level outcome verification provides a common interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks. Source-level diagnostics expose training dynamics that are invisible under aggregate-only monitoring.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}

Unified multimodal RL requires a reward interface that can accommodate heterogeneous tasks without entangling task-specific branches inside the training loop. In our setting, samples differ not only in task type, but also in reward type: some require discrete rule-based supervision, while others rely on continuous spatial feedback such as IoU. Some need only an accuracy reward, whereas others require a joint reward over accuracy and output format. Hard-coding these cases into the trainer quickly leads to a tightly coupled system that is difficult to maintain as tasks are added.

V-Triune therefore makes reward routing explicit at the sample level. Each sample specifies its reward components, their relative weights, and its subsequent verification path through a unified interface. The trainer consumes this common structure and no longer needs task-specific reward branches in the main update loop. In effect, reward routing is encoded in the sample metadata rather than hard-coded throughout the trainer.

In addition to common inputs such as \texttt{images} and \texttt{prompt}, we attach a small set of task-agnostic metadata for reward routing. The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} specify the relative weights of reward components, supporting accuracy-only and accuracy-plus-format settings within one pipeline. The \texttt{verifier} field determines which verifier should process the sample, providing the entry point for the verifier-level interface in~\cref{subsec:verifier_level_reward_computation}. Finally, \texttt{data\_source} records the sample origin and later serves as the indexing key for source-level diagnostics in~\cref{subsec:metric_monitoring}. The full data format is shown in~\cref{fig:data_format}.

This design decouples heterogeneous reward interfaces from the trainer and defines a clean extensibility boundary: adding a new task only requires preparing data, attaching the appropriate metadata, and selecting a compatible verifier, without rewriting the trainer itself. We later validate this extensibility with a GUI-domain extension experiment in~\cref{subsec:gui_extension}. The same metadata also provides the structural basis for source-aware diagnosis, since rewards and behaviors can be regrouped by source after verification. In V-Triune, sample-level formatting functions as a reward routing abstraction rather than a data format alone.
%
\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}

Sample-level routing determines where each sample should go, but unified training still needs a common way to handle heterogeneous outcome verification. Some tasks have outcomes that can be checked with deterministic rules after parsing the model output, while others require continuous spatial evaluation. V-Triune addresses this by defining reward computation at the verifier level: the trainer sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation through a common interface.

This abstraction separates heterogeneous outcome verification from the training loop. The trainer interacts with different verifiers through one common interface, while each verifier preserves its own reward logic. In implementation, we support this design with an asynchronous client-server architecture that scales reward computation independently of the trainer. The key contribution here is the verifier abstraction itself, not the particular implementation used to support it.

In this work we primarily instantiate two verifiers, corresponding to two verification regimes.
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.

\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.

For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.

Verifier-level computation gives different task families a clear boundary for reward logic while letting the trainer interact with them through one common interface. It also lowers the marginal cost of extension. For new task domains that can reuse an existing output structure and verification regime, the RL pipeline remains unchanged and only the data routing needs to be updated. We verify this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.
%
\subsubsection{Dynamic IoU for Precision Enhancement}
\label{subsec:dynamic_iou}

Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemma.

With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.

To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively raises the IoU threshold, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.

Dynamic IoU makes high-precision localization learnable under joint training. It is designed for localization-centric RL, where a fixed threshold is either too loose to refine localization or too strict to bootstrap learning. We provide the exact thresholds and stage boundaries in the implementation details, and further compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}

Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that are difficult to see. Different sources may have different data quality, reward regimes, and generation behaviors, yet aggregated metrics expose only an averaged global trend. As a result, source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden. Unified multimodal RL therefore requires source-level observability.

Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity. We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics. Together they track whether the correct reward is being learned, whether generation behavior is drifting, whether different task families exhibit different response-length and reflection patterns, and whether perception-specific indicators reveal additional issues.

The \textit{Training Reward} metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward, making it possible to distinguish genuine progress from source-specific degradation. \textit{Response Behavior} metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse. These signals are especially informative because different task families may benefit from different generation patterns: longer reasoning traces are often useful for reasoning-heavy tasks, whereas concise responses are often more effective for localization-centric perception tasks~\citep{li2025think}. We therefore track response length at the source level to examine whether unified training preserves task-appropriate behaviors across tasks. \textit{Reflection} metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is provided in~\cref{appx:reflection_metrics}. Finally, \textit{Auxiliary Metrics} include fixed-threshold IoU, ViT/LLM gradient and response examples for qualitative analysis.

These diagnostics do more than summarize training. They helped identify several failure modes that matter for unified training, including ViT gradient explosion and leaked image special tokens~(\cref{sec:training_recipe}), as well as divergent response-length and reflection patterns across task families. They also support later analysis of task interaction by revealing whether unified training preserves task-appropriate behaviors or instead pushes different task families toward the same generation pattern. They further reveal when one source or task family is being overshadowed by stronger training signals elsewhere. Our later stability analysis results provide direct evidence for the necessity of this diagnostic mechanism.

Source-level diagnostics form the third core abstraction of V-Triune: they make unified training not only executable, but diagnosable. This is essential in heterogeneous multimodal RL, where failures rarely manifest uniformly across all tasks and sources.


==> sections_refined/3_method_v5.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.99\linewidth]{images/figure2_v15.pdf}
    \caption{\textbf{Overview of V-Triune.} The framework organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. Together they support mixed-task training across reasoning-heavy and perception-heavy tasks, while Dynamic IoU provides precision-oriented reward shaping for localization-centric tasks.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}

This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models.
%
The central problem is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline despite their different reward interfaces, outcome verification regimes, and observability requirements.

This setting creates three coupled challenges.
%
First, heterogeneous tasks do not fit a rigid shared reward interface, and hard-coding task-specific reward branches into the trainer makes the training loop brittle and difficult to extend.
%
Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds.
%
Third, aggregate-only monitoring can hide source-specific failure modes, making training problems difficult to localize.

V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}.
%
Sample-level reward routing binds reward composition and subsequent verification to each sample.
%
Verifier-level outcome verification provides a common interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks.
%
Source-level diagnostics expose training dynamics that are invisible under aggregate-only monitoring.
%
Together, these abstractions make heterogeneous rewards, verification, and failure signals manageable within one pipeline, supporting stable unified training.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}

Unified multimodal RL requires a reward interface that can accommodate heterogeneous reward compositions and verification paths without entangling task-specific branches inside the training loop.
%
In our setting, samples differ not only in task type but also in reward composition and verification path, so hard-coding these cases into the trainer quickly makes the system brittle and difficult to extend.

V-Triune therefore makes reward routing explicit at the sample level.
%
Each sample specifies its reward components, their relative weights, and its subsequent verification path through a unified interface.
%
The trainer consumes this common structure rather than maintaining task-specific reward branches in the main update loop.

In addition to common inputs such as \texttt{images} and \texttt{prompt}, we attach a small set of task-agnostic metadata for reward routing.
%
The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} specify the relative weights of reward components, supporting accuracy-only and accuracy-plus-format settings within one pipeline.
%
The \texttt{verifier} field determines which verifier should process the sample, providing the entry point for the verifier-level interface in~\cref{subsec:verifier_level_reward_computation}.
%
Finally, \texttt{data\_source} records the sample origin and later serves as the indexing key for source-level diagnostics in~\cref{subsec:metric_monitoring}.
%
The full data format is shown in~\cref{fig:data_format}.

This design defines a clean extensibility boundary: adding a new task only requires preparing data, attaching the appropriate metadata, and selecting a compatible verifier.
%
We later validate this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.
%
The same metadata also supports source-aware diagnosis by allowing rewards and behaviors to be regrouped by source after verification.

\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}

Sample-level routing determines where each sample should go, but unified training still needs a common way to handle heterogeneous outcome verification.
%
Some tasks can be checked with deterministic rules after parsing the model output, whereas others require continuous spatial evaluation.
%
V-Triune addresses this at the verifier level: the trainer sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation through a common interface.

This abstraction lets the trainer interact with heterogeneous reward logic through one interface while preserving task-specific verification inside each verifier.
%
In implementation, we support it with an asynchronous client-server architecture for scalable reward computation.

In this work we primarily instantiate two verifiers, corresponding to two verification regimes:
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.

\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.

For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.

Verifier-level computation gives different task families a clear boundary for reward logic while keeping the trainer unchanged.
%
For new task domains that can reuse an existing output structure and verification regime, only the data routing needs to be updated.
%
We verify this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.

\subsubsection{Dynamic IoU for Precision Enhancement}
\label{subsec:dynamic_iou}

Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemma.

With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.

To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively raises the IoU threshold, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.

Dynamic IoU makes high-precision localization learnable under joint training by combining dense early supervision with stricter late-stage refinement.
%
We provide the exact thresholds and stage boundaries in the implementation details, and compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}

Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that aggregate metrics cannot easily reveal.
%
Different sources may have different data quality, reward regimes, and generation behaviors, so source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden under global averages.

Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity.
%
We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics.
%
Training reward metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward.
%
Response behavior metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse.
%
Reflection metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is given in~\cref{appx:reflection_metrics}.
%
Auxiliary metrics include fixed-threshold IoU, ViT/LLM gradients, and response examples for qualitative analysis.

These diagnostics helped identify several failure modes that matter for unified training, including ViT gradient explosion and leaked image special tokens~(\cref{sec:training_recipe}), as well as divergent response-length and reflection patterns across task families.
%
They also reveal when one source or task family is being overshadowed by stronger training signals elsewhere.
%
Source-level diagnostics therefore make unified training not only executable, but diagnosable.


==> sections_refined/3_method_v6.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/figure2_v15.pdf}
    \caption{\textbf{Overview of V-Triune.} The methodology organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. They address rigid reward interfaces, localization reward ambiguity versus sparsity, and lack of source-level observability in mixed-task training.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}

This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models.
%
The central problem is how to stably train reasoning-heavy and perception-heavy tasks within one RL pipeline despite their different reward interfaces, outcome verification regimes, and observability requirements.

This heterogeneous setting creates three recurring failure modes.
%
First, heterogeneous tasks do not fit a rigid shared reward interface, and hard-coding task-specific reward branches into the trainer makes the training loop brittle and difficult to extend.
%
Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds.
%
Third, aggregate-only monitoring can hide source-specific failure modes, making training problems difficult to localize.

V-Triune addresses these failure modes through three coordinated abstractions, shown in~\cref{fig:framework}.
%
Sample-level reward routing decouples reward composition and verifier choice from the trainer core.
%
Verifier-level outcome verification provides a common interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks.
%
Source-level diagnostics restore observability that aggregate-only monitoring cannot provide.
%
Together, these abstractions turn heterogeneous rewards, verification, and failure signals into a manageable training recipe for stable unified RL.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}

Unified multimodal RL needs a routing abstraction that can accommodate heterogeneous reward compositions and verification paths without entangling task-specific branches inside the training loop.
%
In our setting, samples differ not only in task family but also in reward composition and verification path, so hard-coding these cases into the trainer quickly makes the system brittle and difficult to extend.

V-Triune therefore makes reward routing explicit at the sample level.
%
Each sample specifies the metadata needed for reward composition and subsequent verification through a unified interface.
%
The trainer consumes this common structure rather than maintaining task-specific reward branches in the main update loop.

In addition to common inputs such as \texttt{images} and \texttt{prompt}, each sample carries a small set of task-agnostic routing metadata.
%
The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} define the reward composition, \texttt{verifier} selects the downstream verification path, and \texttt{data\_source} preserves source identity for the diagnostics discussed in~\cref{subsec:metric_monitoring}.
%
The full data format is shown in~\cref{fig:data_format}.

This design defines a clean extensibility boundary: for a new task that can reuse an existing verification regime, extending the mixture only requires preparing data and attaching compatible routing metadata.
%
We later validate this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.
%
The same metadata also supports source-aware diagnosis by allowing rewards and behaviors to be regrouped by source after verification.

\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}

Sample-level routing determines where each sample should go, but unified training still needs a common way to handle heterogeneous outcome verification.
%
Some tasks can be checked with deterministic rules after parsing the model output, whereas others require continuous spatial evaluation.
%
V-Triune addresses this at the verifier level: the trainer sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation through a common interface.

This abstraction lets the trainer interact with heterogeneous reward logic through one interface while preserving task-specific verification inside each verifier.
%
In implementation, we support it with an asynchronous client-server architecture for scalable reward computation.

In this work we primarily instantiate two verifiers, corresponding to two verification regimes:
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.

\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.

For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.

Verifier-level computation gives different task families a clear boundary for reward logic while keeping the trainer unchanged.
%
For new task domains that can reuse an existing output structure and verification regime, only the data routing needs to be updated.
%
We verify this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.

\subsubsection{Dynamic IoU for Precision Enhancement}
\label{subsec:dynamic_iou}

Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemma.

With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.

To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively raises the IoU threshold, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.

Dynamic IoU makes high-precision localization learnable under joint training by combining dense early supervision with stricter late-stage refinement.
%
We provide the exact thresholds and stage boundaries in the implementation details, and compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}

Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that aggregate metrics cannot easily reveal.
%
Different sources may have different data quality, reward regimes, and generation behaviors, so source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden under global averages.

Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity.
%
We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics.
%
Training reward metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward.
%
Response behavior metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse.
%
Reflection metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is given in~\cref{appx:reflection_metrics}.
%
Auxiliary metrics include fixed-threshold IoU, ViT/LLM gradients, and response examples for qualitative analysis.

These diagnostics helped identify several failure modes that matter for unified training, including ViT gradient explosion and leaked image special tokens~(\cref{sec:training_recipe}), as well as divergent response-length and reflection patterns across task families.
%
They also reveal when one source or task family is being overshadowed by stronger training signals elsewhere.
%
Source-level diagnostics therefore make unified training not only executable, but diagnosable.


==> sections_refined/3_method_v7.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/figure2_v15.pdf}
    \caption{\textbf{Overview of V-Triune.} The methodology organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. They address rigid reward interfaces, localization reward ambiguity versus sparsity, and lack of source-level observability in mixed-task training.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}

This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models.
%
The central problem is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline despite their different reward interfaces, outcome verification regimes, and observability requirements.

This setting creates three recurring challenges in practice.
%
First, heterogeneous tasks do not fit a rigid shared reward interface, and hard-coding task-specific reward branches into the trainer makes the training loop brittle and difficult to extend.
%
Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds.
%
Third, aggregate-only monitoring can hide source-specific failure modes, making training problems difficult to localize.

V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}.
%
Sample-level reward routing decouples reward composition and verifier choice from the trainer core.
%
Verifier-level outcome verification provides a common interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks.
%
Source-level diagnostics restore observability that aggregate-only monitoring cannot provide.
%
Together, these abstractions make heterogeneous rewards, verification, and failure signals manageable within one pipeline, supporting stable unified training.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}

Unified multimodal RL requires a reward interface that can accommodate heterogeneous reward compositions and verification paths without entangling task-specific branches inside the training loop.
%
In our setting, samples differ not only in task type but also in reward composition and verification path, so hard-coding these cases into the trainer quickly makes the system brittle and difficult to extend.

V-Triune therefore makes reward routing explicit at the sample level.
%
Each sample specifies its reward components, their relative weights, and its subsequent verification path through a unified interface.
%
The trainer consumes this common structure rather than maintaining task-specific reward branches in the main update loop.

In addition to common inputs such as \texttt{images} and \texttt{prompt}, we attach a small set of task-agnostic metadata for reward routing.
%
The fields \texttt{accuracy\_ratio} and \texttt{format\_ratio} specify the relative weights of reward components, supporting accuracy-only and accuracy-plus-format settings within one pipeline.
%
The \texttt{verifier} field determines which verifier should process the sample, providing the entry point for the verifier-level interface in~\cref{subsec:verifier_level_reward_computation}.
%
Finally, \texttt{data\_source} records the sample origin and later serves as the indexing key for source-level diagnostics in~\cref{subsec:metric_monitoring}.
%
The full data format is shown in~\cref{fig:data_format}.

This design defines a clean extensibility boundary: adding a new task only requires preparing data, attaching the appropriate metadata, and selecting a compatible verifier.
%
We later validate this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.
%
The same metadata also supports source-aware diagnosis by allowing rewards and behaviors to be regrouped by source after verification.

\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}

Sample-level routing determines where each sample should go, but unified training still needs a common way to handle heterogeneous outcome verification.
%
Some tasks can be checked with deterministic rules after parsing the model output, whereas others require continuous spatial evaluation.
%
V-Triune addresses this at the verifier level: the trainer sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation through a common interface.

This abstraction lets the trainer interact with heterogeneous reward logic through one interface while preserving task-specific verification inside each verifier.
%
In implementation, we support it with an asynchronous client-server architecture for scalable reward computation.

In this work we primarily instantiate two verifiers, corresponding to two verification regimes:
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting. For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}. The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer. In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.

\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion. In early experiments, the model struggled to emit valid JSON within \texttt{\textbackslash boxed\{\}}, but learned the \texttt{<answer>} pattern reliably. We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.

For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box. The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level metadata.

Verifier-level computation gives different task families a clear boundary for reward logic while keeping the trainer unchanged.
%
For new task domains that can reuse an existing output structure and verification regime, only the data routing needs to be updated.
%
We verify this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.

\subsubsection{Dynamic IoU for Precision Enhancement}
\label{subsec:dynamic_iou}

Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse. IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a familiar dilemma.

With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization. With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem. This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.

To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism. Rather than fixing a single threshold throughout training, we use a simple three-stage schedule that begins with higher reward density, then progressively raises the IoU threshold, and finally enforces near-exact localization later in training. This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.

Dynamic IoU makes high-precision localization learnable under joint training by combining dense early supervision with stricter late-stage refinement.
%
We provide the exact thresholds and stage boundaries in the implementation details, and compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}

Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that aggregate metrics cannot easily reveal.
%
Different sources may have different data quality, reward regimes, and generation behaviors, so source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden under global averages.

Using the \texttt{data\_source} field, we regroup verified samples by source after reward computation and log training signals at that granularity.
%
We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics.
%
Training reward metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward.
%
Response behavior metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse.
%
Reflection metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is given in~\cref{appx:reflection_metrics}.
%
Auxiliary metrics include fixed-threshold IoU, ViT/LLM gradients, and response examples for qualitative analysis.

These diagnostics helped identify several failure modes that matter for unified training, including ViT gradient explosion and leaked image special tokens~(\cref{sec:training_recipe}), as well as divergent response-length and reflection patterns across task families.
%
They also reveal when one source or task family is being overshadowed by stronger training signals elsewhere.
%
Source-level diagnostics therefore make unified training not only executable, but diagnosable.


==> sections_refined/3_method_v8.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/figure2_v15.pdf}
    \caption{\textbf{Overview of V-Triune.} The methodology organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. They address rigid reward interfaces, localization reward ambiguity versus sparsity, and lack of source-level observability in mixed-task training.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}

This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models.
%
The central problem is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline despite their different reward interfaces, outcome verification regimes, and observability requirements.

In practice, this setting breaks down in three recurring ways.
%
First, heterogeneous tasks do not fit a rigid shared reward interface, and hard-coded task-specific reward branches make the trainer brittle and difficult to extend.
%
Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds.
%
Third, aggregate-only monitoring can hide source-specific failure modes, making training problems difficult to localize.

V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}.
%
Sample-level reward routing defines a clean boundary between the trainer and task-specific reward logic.
%
Verifier-level outcome verification provides a common interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks.
%
Source-level diagnostics restore the observability that aggregate-only monitoring cannot provide.
%
Together, these abstractions make heterogeneous rewards, verification, and failure signals manageable within one pipeline, supporting stable unified training.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}

Unified multimodal RL needs an extensibility boundary between the trainer and task-specific reward logic.
%
Without such a boundary, adding new task families means inserting special-case reward branches into the training loop, which quickly becomes brittle and hard to maintain.
%
V-Triune makes this boundary explicit through sample-level reward routing.

Each sample carries a compact routing specification that determines which reward components should be used, how they are weighted, and which verifier should evaluate the rollout.
%
The trainer consumes only this shared routing interface, while task-specific verification logic stays outside the update loop.
%
This turns heterogeneous reward handling from trainer-side branching into a unified sample-side interface.

In practice, the routing metadata includes component weights, a verifier key, and the source identifier later used for diagnostics.
%
The full schema is shown in~\cref{fig:data_format}.
%
What matters methodologically is that the trainer no longer needs task-specific reward code paths in order to mix reasoning-heavy and perception-heavy tasks in one run.

This design defines a clean extensibility boundary: adding a new task requires preparing data that matches an existing verification regime, or registering a new verifier when a new regime is needed, without rewriting the trainer itself.
%
We later validate this point with the GUI-domain extension in~\cref{subsec:gui_extension}.
%
The same routing metadata also supports source-aware diagnosis by allowing rewards and behaviors to be regrouped by source after verification.

\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}

Sample-level routing determines which verification path a rollout should follow, but unified training still needs a common interface for heterogeneous outcome evaluation.
%
Some tasks can be checked with deterministic rules after parsing the model output, whereas others require continuous spatial scoring.
%
V-Triune handles this at the verifier level: the trainer sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation through a shared interface.

This abstraction lets the trainer interact with heterogeneous reward logic in one way while preserving task-specific verification inside each verifier.
%
In this work we primarily instantiate two verifiers, corresponding to two verification regimes:
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting.
%
For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}.
%
The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer.
%
In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.

\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion.
%
We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.

For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box.
%
The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level routing metadata.

Verifier-level computation gives different task families a clear boundary for reward logic while keeping the trainer unchanged.
%
For new task domains that can reuse an existing output structure and verification regime, only the data routing needs to be updated.
%
We verify this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.

\subsubsection{Dynamic IoU for Precision Enhancement}
\label{subsec:dynamic_iou}

Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse.
%
IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a practical dilemma.

With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization.
%
With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem.
%
This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.

To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism.
%
Rather than fixing one threshold throughout training, we use a simple three-stage schedule that begins with denser supervision, then progressively raises the IoU requirement, and finally enforces near-exact localization later in training.
%
This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.

Dynamic IoU makes high-precision localization learnable under joint training by combining dense early supervision with stricter late-stage refinement.
%
We provide the exact thresholds and stage boundaries in the implementation details, and compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}

Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that aggregate metrics do not expose.
%
Different sources may have different data quality, reward regimes, and response behaviors, so source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden under global averages.

V-Triune therefore tracks verified samples at the source level using the same \texttt{data\_source} key introduced in the routing interface.
%
We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics.
%
Training reward metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward.
%
Response behavior metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse.
%
Reflection metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is given in~\cref{appx:reflection_metrics}.
%
Auxiliary diagnostics include fixed-threshold IoU, ViT/LLM gradients, and response examples for qualitative analysis.

In our experiments, these diagnostics directly informed two training decisions in the final recipe: freezing the vision encoder after observing ViT gradient explosion, and filtering leaked image special tokens before reward recomputation~(\cref{sec:training_recipe}).
%
They also reveal divergent response-length and reflection patterns across task families and help detect when one source is being overshadowed by stronger training signals elsewhere.
%
Source-level diagnostics are therefore part of the training methodology rather than a dashboard add-on: they make unified training actionable and diagnosable.


==> sections_refined/3_method_v9.tex <==
%
\begin{figure}[tb!]
    \centering
    \includegraphics[width=0.95\linewidth]{images/figure2_v15.pdf}
    \caption{\textbf{Overview of V-Triune.} The methodology organizes unified multimodal RL around three training abstractions: sample-level reward routing, verifier-level outcome verification, and source-level diagnostics. They address rigid reward interfaces, localization reward ambiguity versus sparsity, and lack of source-level observability in mixed-task training.}
    \label{fig:framework}
    \vspace{-10px}
\end{figure}
%
\section{V-Triune: Visual Triple Unified Reinforcement Learning}
\label{sec:method}

This section presents V-Triune, our training methodology for unified multimodal RL in vision-language models.
%
The central problem is how to stably train reasoning-heavy and perception-heavy tasks within a single RL pipeline despite their different reward interfaces, outcome verification regimes, and observability requirements.

In practice, this setting breaks down in three recurring ways.
%
First, heterogeneous tasks do not fit a rigid shared reward interface, and hard-coded task-specific reward branches make the trainer brittle and difficult to extend.
%
Second, localization-centric tasks such as detection and grounding face an ambiguity-versus-sparsity trade-off under fixed IoU thresholds.
%
Third, aggregate-only monitoring can hide source-specific failure modes, making training problems difficult to localize.

V-Triune addresses these issues through three coordinated abstractions, shown in~\cref{fig:framework}.
%
Sample-level reward routing defines a clean boundary between the trainer and task-specific reward logic.
%
Verifier-level outcome verification provides a common interface for heterogeneous reward computation and incorporates Dynamic IoU for localization tasks.
%
Source-level diagnostics restore the observability that aggregate-only monitoring cannot provide.
%
Together, these abstractions make heterogeneous rewards, verification, and failure signals manageable within one pipeline, supporting stable unified training.
%
\subsection{Sample-Level Reward Routing}
\label{subsec:sample_level_formatting}

Unified multimodal RL needs an extensibility boundary between the trainer and task-specific reward logic.
%
Without such a boundary, adding new task families means inserting special-case reward branches into the training loop, which quickly becomes brittle and hard to maintain.
%
V-Triune makes this boundary explicit through sample-level reward routing.

Each sample carries a compact routing specification that determines which reward components should be used, how they are weighted, and which verifier should evaluate the rollout.
%
The trainer consumes only this shared routing interface, while task-specific verification logic stays outside the update loop.
%
This turns heterogeneous reward handling from trainer-side branching into a unified sample-side interface.

In practice, the routing metadata includes component weights, a verifier key, and the source identifier later used for diagnostics.
%
Although this interface is sample-level, it is not per-sample reward tuning.
%
In our main setup, the metadata only selects among a small set of verifier-defined reward templates, making explicit the routing that heterogeneous verifiable-reward training already requires.
%
The full schema is shown in~\cref{fig:data_format}.
%
What matters methodologically is that the trainer no longer needs task-specific reward code paths in order to mix reasoning-heavy and perception-heavy tasks in one run.

This design defines a clean extensibility boundary: adding a new task requires preparing data that matches an existing verification regime, or registering a new verifier when a new regime is needed, without rewriting the trainer itself.
%
We later validate this point with the GUI-domain extension in~\cref{subsec:gui_extension}.
%
The same routing metadata also supports source-aware diagnosis by allowing rewards and behaviors to be regrouped by source after verification.

\subsection{Verifier-Level Outcome Verification}
\label{subsec:verifier_level_reward_computation}

Sample-level routing determines which verification path a rollout should follow, but unified training still needs a common interface for heterogeneous outcome evaluation.
%
Some tasks can be checked with deterministic rules after parsing the model output, whereas others require continuous spatial scoring.
%
V-Triune handles this at the verifier level: the trainer sends predictions and references to the designated verifier, which performs parsing, verification, and reward computation through a shared interface.

This abstraction lets the trainer interact with heterogeneous reward logic in one way while preserving task-specific verification inside each verifier.
%
In this work we primarily instantiate two verifiers, corresponding to two verification regimes:
%
\noindent\paragraph{MathVerifyVerifier: Rule-verifiable outcomes}
This verifier handles tasks whose outputs can be parsed and deterministically checked, including mathematics, puzzles, science, chart reasoning, OCR, and counting.
%
For these tasks, we parse the model output into a normalized answer and verify it against the reference using \texttt{math\_verify}~\citep{mathverify2025}.
%
The resulting accuracy reward follows the standard 0--1 rule-based form:
%
\begin{equation}
    R_\text{acc}(\hat{a}, a) = \mathbb{I}(\texttt{verify}(\texttt{parse}(\hat{a}), \texttt{parse}(a)))
    \label{eq:math_rule}
\end{equation}
%
where $\hat{a}$ denotes the predicted answer and $a$ the ground-truth answer.
%
In our setup, model responses are instructed to place the final answer inside \texttt{\textbackslash boxed\{\}}, after which deterministic verification is applied.

\noindent\paragraph{DetectionVerifier: Localization-centric outcomes}
This verifier handles tasks such as detection and grounding, where outputs must satisfy both a structural format and a spatial accuracy criterion.
%
We therefore compute a composite reward with separate format and accuracy terms.
%
To enforce the required output structure, we define a format reward as
%
\begin{equation}
    R_{\text{format}}(o_q) = 0.25 \sum_{i=1}^{4} \mathbb{I}(\text{count}(o_q, s_i) = 1)
    \label{eq:format_rule}
\end{equation}
%
where $o_q$ is the model response to query $q$, and the four format tags are $\{s_i\}_{i=1}^4 = \{\texttt{<think>}, \texttt{</think>}, \texttt{<answer>}, \texttt{</answer>}\}$.

For the spatial component, we use IoU-based accuracy:
%
\begin{equation}
R_\text{acc}(\hat{a}, a) =
\begin{cases}
\text{IoU}(\hat{a}, a), & \text{if}\quad\text{IoU}(\hat{a}, a) \ge \epsilon \\
0, & \text{else}
\end{cases},
\qquad \text{where} \quad
\text{IoU}(\hat{a}, a) = \frac{\text{Area}(\hat{a} \cap a)}{\text{Area}(\hat{a} \cup a)}
\label{eq:iou_rule}
\end{equation}
%
where $\hat{a}$ is the predicted box and $a$ is the ground-truth box.
%
The final reward combines the two parts as $\alpha_{\text{acc}} \cdot R_{\text{acc}} + \alpha_{\text{format}} \cdot R_{\text{format}}$, where $\alpha_{\text{acc}}$ and $\alpha_{\text{format}}$ are specified by the sample-level routing metadata.

Verifier-level computation gives different task families a clear boundary for reward logic while keeping the trainer unchanged.
%
For new task domains that can reuse an existing output structure and verification regime, only the data routing needs to be updated.
%
We verify this point with the GUI-domain extension experiment in~\cref{subsec:gui_extension}.

\subsubsection{Dynamic IoU for Precision Enhancement}
\label{subsec:dynamic_iou}

Within \textit{DetectionVerifier}, the main optimization challenge is to construct a localization reward that is informative without becoming too sparse.
%
IoU is the most direct spatial signal for detection and grounding, but a fixed threshold creates a practical dilemma.

With a loose threshold such as IoU@50~\citep{yu2025perception,liu2025visionreasoner}, reward density is high but reward ambiguity remains severe: multiple coarse boxes can receive nearly identical rewards, leaving limited pressure for finer localization.
%
With a highly strict threshold such as near-exact matching, the objective becomes clearer but early rollouts receive almost no positive feedback, creating a cold-start problem.
%
This issue is amplified in unified training because localization rewards must coexist with sharper rule-based rewards from reasoning tasks.

To address this trade-off, we introduce Dynamic IoU, a dense-to-strict reward shaping mechanism.
%
Rather than fixing one threshold throughout training, we use a simple three-stage schedule that begins with denser supervision, then progressively raises the IoU requirement, and finally enforces near-exact localization later in training.
%
This staging preserves learnability in early optimization while still imposing high-precision supervision in the late phase.

Dynamic IoU makes high-precision localization learnable under joint training by combining dense early supervision with stricter late-stage refinement.
%
We provide the exact thresholds and stage boundaries in the implementation details, and compare this design against fixed thresholds and alternative schedules in the experiments and appendix.
%
\subsection{Source-Level Diagnostics}
\label{subsec:metric_monitoring}

Even with sample-level routing and verifier-level computation, unified RL can still fail in ways that aggregate metrics do not expose.
%
Different sources may have different data quality, reward regimes, and response behaviors, so source-specific reward collapse, format drift, abnormal token generation, local task suppression, or optimization instability may remain hidden under global averages.

V-Triune therefore tracks verified samples at the source level using the same \texttt{data\_source} key introduced in the routing interface.
%
We organize these signals into four groups: training reward, response behavior, reflection-related metrics, and auxiliary diagnostics.
%
Training reward metrics provide a source-level breakdown of rule-based accuracy, format reward, and IoU-based reward.
%
Response behavior metrics include average length, lengths of correct and incorrect responses, and truncation rates, which help reveal verbosity drift or collapse.
%
Reflection metrics provide a lightweight online proxy for response strategy by tracking whether reflective cues appear in responses; the precise definition is given in~\cref{appx:reflection_metrics}.
%
Auxiliary diagnostics include fixed-threshold IoU, ViT/LLM gradients, and response examples for qualitative analysis.

In our experiments, these diagnostics directly informed two training decisions in the final recipe: freezing the vision encoder after observing ViT gradient explosion, and filtering leaked image special tokens before reward recomputation~(\cref{sec:training_recipe}).
%
They also reveal divergent response-length and reflection patterns across task families and help detect when one source is being overshadowed by stronger training signals elsewhere.
%
Source-level diagnostics are therefore part of the training methodology rather than a dashboard add-on: they make unified training actionable and diagnosable.


==> sections_refined/5_experiment_v1.tex <==
\section{Experiment}
\label{sec:experiment}

\begin{table*}[t]
\centering
\caption{Fair-budget evidence under a fixed training budget. Left: MEGA-Bench task-composition curves for the 7B off-policy setting. Right: benchmark breakdown at the same 60-step budget. MME-R = MME-Reasoning~\citep{yuan2025mme}. CharXiv(RQ) = CharXiv Reasoning Question. COCO (S$\mid$M) reports single-object and multi-object mAP in COCO val-2017. COCO mAP uses the standard cocoapi; see details in~\cref{sec:coco_evaluation}. Best results are bolded and second-best results are underlined.}
\label{fig:fair_budget_evidence}
\begin{minipage}[t]{0.31\textwidth}
\vspace{-1pt}
\centering
\includegraphics[width=\linewidth]{images/figure6/7b_task_new.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.68\textwidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Reasoning Benchmarks} \\
\midrule
Mixture & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) \\
\midrule
Unified & \underline{56.56} & \underline{71.40} & \underline{30.51} & \textbf{28.20} & \textbf{44.50} \\
Reason-only & 54.89 & \textbf{71.70} & \textbf{31.24} & \underline{28.03} & \underline{44.00} \\
Perception-only & \textbf{56.67} & 68.20 & 29.59 & 26.26 & 41.00 \\
\bottomrule
\end{tabular}
}

\vspace{4pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Perception Benchmarks} \\
\midrule
Mixture & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
\midrule
Unified & \underline{73.75} & \textbf{82.20} & \underline{80.69} $\mid$ \textbf{38.62} & \textbf{55.87} & \underline{23.91} \\
Reason-only & 73.25 & 78.53 & 78.36 $\mid$ 33.87 & \underline{55.77} & \textbf{23.97} \\
Perception-only & \textbf{76.00} & \underline{80.10} & \textbf{80.78} $\mid$ \underline{37.37} & 55.33 & 23.78 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table*}

\subsection{Experimental Setup}
\label{subsec:implementation details}

We evaluate V-Triune at two levels.
%
First, we compare three training mixtures under a fixed budget: a unified mixture with both reasoning and perception data, and two specialist mixtures that keep only one side (\textit{Reason-only} and \textit{Perception-only}).
%
This lets us test whether joint RL training produces cross-task gains.
%
Second, we report the final Orsta models under a longer training horizon to evaluate overall competitiveness on broad and task-specific benchmarks.

We use Qwen2.5-VL-7B-Instruct and Qwen2.5-VL-32B-Instruct~\citep{Qwen2.5-VL} as backbones.
%
RL post-training is conducted on a 47.7K-sample VQA training set with verifiable answers from 18 sources, covering four reasoning tasks (math, puzzle, science, and chart) and four perception tasks (detection, grounding, counting, and OCR).
%
Detailed data construction is given in~\cref{subsec:data,tab:data_source}.
%
We use GRPO~\citep{shao2024deepseekmath} for all main experiments, with a rollout batch size of 1024 and 8 sampled responses per prompt.
%
Our unified RL pipeline is implemented on top of Verl.
%
The controlled comparisons use a fixed training budget, while the final-model results use 3 training epochs.
%
For stability, we freeze the vision encoder and connector and update only the language model layers.
%
Rollouts are generated with the vLLM engine using sampling with \texttt{temperature=1.0}, \texttt{top-p=1.0}, and \texttt{max\_length=2048}.
%
For localization tasks, the main experiments use a three-stage Dynamic IoU schedule.

\subsection{Does Unified Training Help Under Fair Budgets?}
\label{subsec:fair_budget}

We first study unified training under a fixed training budget.
%
Unless otherwise stated, all fair-budget comparisons use the same 7B off-policy setup with 8 optimization steps per rollout.
%
We compare the unified mixture against the two specialist mixtures under the same budget, and test whether joint training improves both overall capability and task-specific performance.

The first piece of evidence comes from the MEGA-Bench task-composition curves in~\cref{fig:fair_budget_evidence}.
%
Under the same 60-step budget, \textit{Reason+Perception} follows the strongest or tied-strongest trajectory throughout training.
%
This suggests that joint training does not introduce a clear reasoning-versus-perception trade-off on MEGA-Bench, and instead leads to a better overall optimization trend.

MEGA-Bench alone, however, is not enough to show whether this gain covers both task families.
%
We therefore compare the same three mixtures on a 10-benchmark suite that spans both reasoning and perception, and report the results at the end of the same fixed budget in~\cref{fig:fair_budget_evidence}.
%
The benchmark list and evaluation protocols are given in the appendix.
%
The unified mixture remains stronger or comparable on both sides, and reaches the best result on multiple benchmarks.

Across this suite, the unified model matches or exceeds the specialist baselines on 5/10 benchmarks and stays close on the rest.
%
This is notable because, under the same training budget, each task family receives fewer effective updates in the unified mixture than in its specialist counterpart.
%
This points to better data efficiency under unified RL training and is consistent with a mild form of cross-task regularization.
%
One plausible explanation is that perception tasks provide direct visual grounding signals, while reasoning tasks improve the shared vision-language representation and instruction-following behavior.

% =============================================================================================

\begin{table*}[t]
\centering

% ================= LEFT COLUMN =================
\begin{minipage}[t]{0.29\linewidth}
\vspace{0pt}
\centering

\captionof{table}{Performance on MEGA-Bench Core.}
\label{tab:mega_bench_core}

\small
\setlength{\tabcolsep}{2pt}

% -------- 7B --------
\begin{tabular}{@{}lr@{}}
\toprule
Model & Score \\
\midrule
\multicolumn{2}{c}{7B Models} \\
\midrule
Qwen2.5-VL-7B      & 35.07 \\
MM-Eureka-7B       & 35.96 \\
VL-Rethinker-7B    & 37.25 \\
\textbf{Orsta-7B}  & \textbf{38.31} \\
$\Delta$ (Ours - Backbone) & +3.24 \\
\bottomrule
\end{tabular}

\vspace{5pt}

% -------- 32B 0321 --------
\begin{tabular}{@{}lr@{}}
\toprule
\multicolumn{2}{c}{32B Models (0321)} \\
\midrule
Qwen2.5-VL-32B-0321     & 11.87 \\
MM-Eureka-32B           & 18.57 \\
VL-Rethinker-32B        & 19.41 \\
\textbf{Orsta-32B-0321} & \textbf{25.94} \\
$\Delta$ (Ours - Backbone) & +14.07 \\
\bottomrule
\end{tabular}

\vspace{5pt}

% -------- 32B 0326 --------
\begin{tabular}{@{}lr@{}}
\toprule
\multicolumn{2}{c}{32B Models (0326)} \\
\midrule
Qwen2.5-VL-32B-0326     & 43.67 \\
Gemma3-27B              & 41.82 \\
InternVL-3-38B          & \textbf{46.69} \\
\textbf{Orsta-32B-0326} & 45.77 \\
$\Delta$ (Ours - Backbone) & +2.10 \\
\bottomrule
\end{tabular}

\end{minipage}
\hfill
% ================= RIGHT COLUMN =================
\begin{minipage}[t]{0.68\linewidth}
\vspace{0pt}
\centering

% -------- Baseline comparison --------
\captionof{table}{Comparison against strong multi-task RL-VLM baselines on reasoning and perception benchmarks.}
\label{tab:baseline_comparison}

\scriptsize
\setlength{\tabcolsep}{3pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{6}{c}{\textbf{Reasoning Benchmarks}} \\
\midrule
Model & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) \\
\midrule
\textbf{Orsta-7B}       & \textbf{57.10} & 72.50 & 31.73 & \textbf{31.14} & \textbf{48.40} \\
MM-Eureka-7B            & 55.33          & 74.10 & 30.84 & 28.45          & 42.10 \\
VL-Rethinker-7B         & 56.70          & \textbf{75.40} & \textbf{32.46} & 29.38 & 44.00 \\
VisionReasoner-7B       & 56.56          & 69.70 & 29.20 & 25.84          & 41.20 \\
\bottomrule
\end{tabular}
}

\vspace{5pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{6}{c}{\textbf{Perception Benchmarks}} \\
\midrule
Model & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
\midrule
\textbf{Orsta-7B}       & \textbf{77.25} & \textbf{81.68} & \textbf{80.73} $\mid$ \textbf{41.41} & \textbf{56.05} & 23.91 \\
MM-Eureka-7B            & 59.62          & 57.07          & 79.73 $\mid$ 35.84                   & 53.38          & 24.23 \\
VL-Rethinker-7B         & 65.12          & 68.60          & 72.50 $\mid$ 31.54                   & 55.70          & \textbf{24.48} \\
VisionReasoner-7B       & 74.38          & 80.63          & 80.22 $\mid$ 36.58                   & 55.44          & 24.23 \\
\bottomrule
\end{tabular}
}

\vspace{10pt}

% -------- GUI extension --------
\captionof{table}{Extension to a new GUI task domain with 3K ShowUI samples under the same 60-step fixed-compute budget.}
\label{tab:gui_extension}
\vspace{4pt}


\small
\setlength{\tabcolsep}{20pt}

\resizebox{0.99\linewidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Mixture & ScreenSpot-Pro & OCRBenchV2 \\
\midrule
Unified (original)           & 23.91         & 55.87 \\
Perception-only (original)   & 23.78         & 55.33 \\
Perception + GUI-3K          & 29.85         & 55.96 \\
Unified + GUI-3K             & \textbf{31.68} & \textbf{56.09} \\
\bottomrule
\end{tabular}
}

\end{minipage}

\end{table*}

\subsection{General Performance on MEGA-Bench}
\label{subsec:mega_bench}

The fixed-budget results in~\cref{subsec:fair_budget} show that unified RL training matches or outperforms specialist mixtures under matched budgets.
%
We now turn to the final Orsta models and report their overall performance on MEGA-Bench Core~\citep{chen2024mega}, which spans over 440 diverse tasks for general VLM capability.
%
For the final-model results, we train both on-policy and off-policy variants for 3 epochs, and for each backbone designate one model as the final Orsta variant based on its performance on MEGA-Bench Core.
%
We evaluate that same selected model on all subsequent benchmarks.
%
We provide the full MEGA-Bench evaluation curves in~\cref{appx:mega_bench_curves}.

Overall, Orsta consistently improves the MEGA-Bench performance of its base model at both 7B and 32B scales.
%
For the 7B model, unified RL post-training yields a clear overall gain.
%
The same pattern holds at 32B, but with two different gain profiles in~\cref{tab:mega_bench_core}: for the \texttt{0321} checkpoint,\footnote{\texttt{0321} and \texttt{0326} follow the release dates of the public HuggingFace checkpoints. The former shows noticeably weaker perception and formatting abilities, while the latter is a stronger later release.} RL post-training brings a much larger improvement; for the stronger \texttt{0326} checkpoint, V-Triune still delivers stable and notable gains.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/combined_iou_train_disable_vit.pdf}
\caption{Dynamic IoU ablations and source-level diagnostics. (a) On COCO multi-object, fixed IoU@50 learns quickly but degrades later, while fixed IoU@99 is more stable but learns more slowly; among staged schedules, our $0.85 \rightarrow 0.95 \rightarrow 0.99$ design gives the best balance between early learnability and late precision enforcement. (b) In unified RL training, the reasoning-heavy Puzzle source shows increasing response length and reflection ratio, whereas the localization-centric Detection source remains short and nearly reflection-free, indicating task-dependent response behavior. (c) Continuing to update the vision encoder causes COCO performance to drop and total gradient norms to grow sharply, motivating the decision to freeze the vision encoder and connector in the main experiments. More detailed failure analyses are provided in~\cref{sec:training_recipe}.}
\label{fig:combined_iou_source_level}
\end{figure*}


\subsection{Comparison with Strong Multi-task RL-VLM Baselines}
\label{subsec:baseline_comparison}

Beyond the overall capability and scaling trends in~\cref{subsec:mega_bench}, we further compare Orsta-7B against three strong multi-task RL-VLM baselines.
%
MM-Eureka-7B~\citep{meng2025mm} and VL-Rethinker-7B~\citep{vl_rethinker} are more reasoning-oriented multi-task RL models, whereas VisionReasoner-7B~\citep{liu2025visionreasoner} adopts a more perception-centric design.
%
We use the same 10-benchmark suite as in~\cref{subsec:fair_budget}.

As shown in~\cref{tab:baseline_comparison}, Orsta-7B achieves the best score on 7/10 benchmarks.
%
On the reasoning side, it wins MMMU, MME-Reasoning, and CharXiv(RQ), while staying competitive on MathVista and MathVision.
%
On the perception side, it reaches the top score on 4/5 benchmarks, with the clearest margin on the challenging COCO multi-object setting.

This comparison complements the fair-budget evidence in~\cref{subsec:fair_budget}: the benefit of unified training is not limited to controlled mixture analysis, but remains visible in the final model.
%
More concretely, the gain is not confined to either reasoning or perception alone, but helps the final model stay competitive on both capability families.

\subsection{Why is Dynamic IoU Necessary for Localization Tasks?}
\label{subsec:dynamic_iou_ablation}

We next examine why Dynamic IoU is necessary for localization-centric tasks and why a staged schedule is effective.
%
Unless otherwise stated, the ablations in this subsection use only the detection and grounding subsets of the training data, while keeping the 7B off-policy setup unchanged.
%
The main Dynamic IoU schedule uses three stages: IoU threshold $0.85$ in the first 10\% of training, $0.95$ from 10\% to 25\%, and $0.99$ thereafter.

On COCO multi-object, the fixed-threshold comparison in~\cref{fig:combined_iou_source_level}(a) shows the two failure modes directly.
%
IoU@50 learns quickly but degrades later, which we attribute to reward ambiguity under a loose threshold.
%
Qualitative cases in~\cref{appx:dynamic_iou_cases} support this interpretation: late-stage predictions often drift among multiple coarse boxes that remain similarly rewarded under IoU@50, rather than continuing to sharpen around the ground-truth box.
%
IoU@99 is more precise but learns much more slowly because the reward is too sparse early on.
%
Dynamic IoU avoids both issues: it remains learnable at the start while still pushing the model toward higher-precision localization later.

We further compare alternative staged schedules in~\cref{fig:combined_iou_source_level}(a).
%
The loose variant ($0.7 \rightarrow 0.8 \rightarrow 0.85$) plateaus because its final threshold remains too permissive, whereas the strict variant ($0.9 \rightarrow 0.95 \rightarrow 0.99$) slows early learning by making the task too difficult from the start.
%
Our main schedule ($0.85 \rightarrow 0.95 \rightarrow 0.99$) gives the best balance between early learnability and late precision enforcement.

The same advantage pattern also appears on the OVDEval negation subset; full curves are given in~\cref{appx:ovd_dynamic_iou}.
%
In addition, we implemented an adaptive scheduler that automatically adjusts the threshold according to the bbox success rate within each batch; full results are given in~\cref{appx:adaptive}.


\subsection{What Do Source-Level Diagnostics Reveal?}
\label{subsec:source_level_diagnostics}

Source-level diagnostics expose signals that aggregate metrics can easily hide, as shown in~\cref{fig:combined_iou_source_level}.
%
Across our unified RL experiments, they reveal two kinds of patterns: task-dependent response behavior and failure modes that directly affect training stability.

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{images/combined_train_disable_vit.pdf}
% \caption{Source-level diagnostics in unified RL. (a) In Orsta-32B-0321 unified RL training, the reasoning-heavy Puzzle source shows increasing response length and reflection ratio, whereas the localization-centric Detection source remains short and nearly reflection-free, indicating task-dependent response behavior. (b) Continuing to update the vision encoder causes COCO performance to drop and total gradient norms to grow sharply, motivating the decision to freeze the vision encoder and connector in the main experiments. More detailed failure analyses are provided in~\cref{sec:training_recipe}.}
% \label{fig:source_level_diagnostics}
% \end{figure*}

On the behavior side, \cref{fig:combined_iou_source_level}(b) uses Puzzle and Detection as two representative sources.
%
Under unified training, the two task families do not converge to the same response pattern.
%
For the reasoning-heavy Puzzle source, both response length and reflection ratio increase over training.
%
For the localization-centric Detection source, responses remain short and direct, and reflection stays at a low level.
%
This suggests that unified training preserves task-appropriate response patterns across task families.
%
More detailed multi-source dynamics are provided in~\cref{sec:training_dynamics_analysis}.

On the stability side, \cref{fig:combined_iou_source_level}(c) shows two immediate effects of continuing to update the vision encoder.
%
COCO performance drops quickly, and total gradient norms become much larger.
%
\cref{sec:training_recipe} further shows that this instability eventually appears as gradient explosion in the ViT and soon hurts detection and grounding performance.
%
The same source-level logs also exposed leaked image special tokens in model responses.
%
These leaked tokens can cause the number of visual features to no longer match the input sequence and directly lead to training failure.
%
Based on these findings, we freeze the vision encoder and connector in the main experiments and filter leaked image special tokens before reward recomputation.
%
More detailed layer-wise gradients, image-token failure cases, and stability analysis are provided in~\cref{sec:training_recipe}.

\subsection{Can V-Triune Extend to New Task Domains?}
\label{subsec:gui_extension}

Finally, we test whether V-Triune can absorb a new task domain beyond the original training mix.
%
As a concrete case, we add about 3K GUI grounding samples from ShowUI~\citep{lin2025showui}, a domain that is not covered in the original dataset.
%
This experiment asks two questions: whether the unified pipeline can directly benefit from the new domain, and whether the advantage of unified training remains after the new domain is added.

As shown in~\cref{tab:gui_extension}, adding ShowUI data substantially improves ScreenSpot-Pro, with the unified model rising from 23.91 to 31.68.

More importantly, after adding the same GUI data, \textit{Unified + GUI} still outperforms \textit{Perception + GUI} by +1.83 points on ScreenSpot-Pro.
%
Reasoning-heavy data therefore does not block learning in the new GUI domain.
%
Instead, once the model has basic in-domain visual support, unified training continues to provide positive transfer.

These results suggest that V-Triune can extend beyond the original training domains while preserving the benefit of unified training.
%
In the ShowUI case, this extension is straightforward because the GUI task can reuse the existing localization-style verifier regime, without rewriting the core RL loop.



% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3.5pt}
% \caption{Performance on MEGA-Bench Core. Orsta consistently improves its backbone at both 7B and 32B scales, with especially large gains on the weaker 32B-0321 checkpoint.}
% \label{tab:mega_bench_core}
% \begin{tabular}{@{}l r|l r|l r@{}}
% \toprule
% \multicolumn{2}{c|}{7B Models} & \multicolumn{2}{c|}{32B Models (0321)} & \multicolumn{2}{c}{32B Models (0326)} \\
% \midrule
% Model & Score & Model & Score & Model & Score \\
% \midrule
% Qwen2.5-VL-7B & 35.07
% & Qwen2.5-VL-32B-0321 & 11.87
% & Qwen2.5-VL-32B-0326 & 43.67 \\
% MM-Eureka-7B & 35.96
% & MM-Eureka-32B & 18.57
% & Gemma3-27B & 41.82 \\
% VL-Rethinker-7B & 37.25
% & VL-Rethinker-32B & 19.41
% & InternVL-3-38B & \textbf{46.69} \\
% \textbf{Orsta-7B} & \textbf{38.31}
% & \textbf{Orsta-32B-0321} & \textbf{25.94}
% & \textbf{Orsta-32B-0326} & 45.77 \\
% $\Delta$ (Ours - Backbone) & +3.24
% & $\Delta$ (Ours - Backbone) & +14.07
% & $\Delta$ (Ours - Backbone) & +2.10 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \caption{Extension to a new GUI task domain with 3K ShowUI samples under the same 60-step fixed-compute budget.}
% \label{tab:gui_extension}
% \begin{tabular}{lcc}
% \toprule
% Mixture & ScreenSpot-Pro & OCRBenchV2 \\
% \midrule
% Unified (original) & 23.91 & 55.87 \\
% Perception-only (original) & 23.78 & 55.33 \\
% Perception + GUI-3K & 29.85 & 55.96 \\
% Unified + GUI-3K & \textbf{31.68} & \textbf{56.09} \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}[t]
% \centering
% \caption{Comparison against strong multi-task RL-VLM baselines on 10 reasoning and perception benchmarks. COCO (S$\mid$M) reports single-object and multi-object mAP. Best results are bolded.}
% \label{tab:baseline_comparison}
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc}
% \toprule
% Model & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
% \midrule
% \textbf{Orsta-7B} & \textbf{57.10} & 72.50 & 31.73 & \textbf{31.14} & \textbf{48.40} & \textbf{77.25} & \textbf{81.68} & \textbf{80.73} $\mid$ \textbf{41.41} & \textbf{56.05} & 23.91 \\
% MM-Eureka-7B & 55.33 & 74.10 & 30.84 & 28.45 & 42.10 & 59.62 & 57.07 & 79.73 $\mid$ 35.84 & 53.38 & 24.23 \\
% VL-Rethinker-7B & 56.70 & \textbf{75.40} & \textbf{32.46} & 29.38 & 44.00 & 65.12 & 68.60 & 72.50 $\mid$ 31.54 & 55.70 & \textbf{24.48} \\
% VisionReasoner-7B & 56.56 & 69.70 & 29.20 & 25.84 & 41.20 & 74.38 & 80.63 & 80.22 $\mid$ 36.58 & 55.44 & 24.23 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{images/figure5/iou_coco_combined.pdf}
%   \caption{Dynamic IoU ablations for localization-centric RL. (a) On COCO multi-object, fixed IoU@50 learns quickly but degrades later, while fixed IoU@99 is more stable but learns more slowly; Dynamic IoU achieves the best overall trajectory. (b) On the same benchmark, compared with loose and strict staged schedules, our $0.85 \rightarrow 0.95 \rightarrow 0.99$ schedule provides the best balance between early learnability and late precision enforcement. (c) On the OVDEval negation subset~\citep{yao2024evaluate}, Dynamic IoU also improves over fixed IoU@99, showing that the advantage extends beyond COCO.}
% \label{fig:dynamic_iou_ablation}
% \end{figure*}


==> sections_refined/5_experiment_v2.tex <==
\section{Experiment}
\label{sec:experiment}

\begin{table*}[t]
\centering
\caption{Fair-budget evidence under a fixed training budget. Left: MEGA-Bench task-composition curves for the 7B off-policy setting. Right: benchmark breakdown at the same 60-step budget. Unified = Reason+Perception. MME-R = MME-Reasoning~\citep{yuan2025mme}. CharXiv(RQ) = CharXiv Reasoning Question. COCO (S$\mid$M) reports single-object and multi-object mAP in COCO val-2017. COCO mAP uses the standard cocoapi; see details in~\cref{sec:coco_evaluation}. Best results are bolded and second-best results are underlined.}
\label{fig:fair_budget_evidence}
\begin{minipage}[t]{0.31\textwidth}
\vspace{-1pt}
\centering
\includegraphics[width=\linewidth]{images/figure6/7b_task_new.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.68\textwidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Reasoning Benchmarks} \\
\midrule
Mixture & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) \\
\midrule
Unified & \underline{56.56} & \underline{71.40} & \underline{30.51} & \textbf{28.20} & \textbf{44.50} \\
Reason-only & 54.89 & \textbf{71.70} & \textbf{31.24} & \underline{28.03} & \underline{44.00} \\
Perception-only & \textbf{56.67} & 68.20 & 29.59 & 26.26 & 41.00 \\
\bottomrule
\end{tabular}
}

\vspace{4pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Perception Benchmarks} \\
\midrule
Mixture & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
\midrule
Unified & \underline{73.75} & \textbf{82.20} & \underline{80.69} $\mid$ \textbf{38.62} & \textbf{55.87} & \underline{23.91} \\
Reason-only & 73.25 & 78.53 & 78.36 $\mid$ 33.87 & \underline{55.77} & \textbf{23.97} \\
Perception-only & \textbf{76.00} & \underline{80.10} & \textbf{80.78} $\mid$ \underline{37.37} & 55.33 & 23.78 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table*}
%
\vspace{-10pt}

\subsection{Experimental Setup}
\label{subsec:implementation details}

We evaluate V-Triune at two levels.
%
First, under a fixed budget, we compare a unified mixture against two specialist mixtures: \textit{Reason-only} and \textit{Perception-only}.
%
Second, we report the final Orsta models under a longer training horizon to evaluate overall competitiveness on broad and task-specific benchmarks.

We use Qwen2.5-VL-7B and 32B~\citep{Qwen2.5-VL} as backbones.
%
RL post-training uses a 47.7K-sample VQA training set with verifiable answers from 18 sources, covering four reasoning tasks (math, puzzle, science, and chart) and four perception tasks (detection, grounding, counting, and OCR).
%
Detailed data construction is given in~\cref{subsec:data,tab:data_source}.
%
We use GRPO~\citep{shao2024deepseekmath} in all main experiments, with a rollout batch size of 1024 and 8 sampled responses per prompt, and implement the unified RL pipeline on top of Verl~\citep{sheng2024hybridflow}.
%
Controlled comparisons use a fixed training budget, whereas final-model results use 3 training epochs.
%
For stability, we freeze the vision encoder and update only the LLM layers.
%
Rollouts are generated with vLLM using \texttt{temperature=1.0}, \texttt{top-p=1.0}, and \texttt{max\_length=2048}, and localization tasks use a three-stage Dynamic IoU schedule.

\subsection{Does Unified Training Help Under Fair Budgets?}
\label{subsec:fair_budget}

We first study unified training under a fixed training budget.
%
Unless otherwise stated, all fair-budget comparisons use the same 7B off-policy with 8 optimization steps per rollout.
%
We compare the unified mixture against two specialist mixtures under the same budget.

The left panel of~\cref{fig:fair_budget_evidence} provides the first evidence through the MEGA-Bench task-composition curves.
%
Under the same 60-step budget, \textit{Reason+Perception} follows the strongest or tied-strongest trajectory throughout training.
%
This suggests that joint training does not introduce a clear reasoning-versus-perception trade-off on MEGA-Bench.

We further compare the same three mixtures on a 10-benchmark suite spanning both reasoning and perception, and report the fixed-budget benchmark breakdown in~\cref{fig:fair_budget_evidence}.
%
The benchmark list and evaluation protocols are given in~\cref{sec:eval_details}.
%
The unified mixture remains stronger or comparable on both sides and reaches the best result on multiple benchmarks.
%
Across this suite, the unified model matches or exceeds the specialist baselines on 5/10 benchmarks and stays close on the rest.
%
This is consistent with better data efficiency under unified RL training and suggests mild cross-task regularization.

% =============================================================================================

\begin{table*}[t]
\centering

% ================= LEFT COLUMN =================
\begin{minipage}[t]{0.29\linewidth}
\vspace{0pt}
\centering

\captionof{table}{Performance on MEGA-Bench Core.}
\label{tab:mega_bench_core}

\small
\setlength{\tabcolsep}{2pt}

% -------- 7B --------
\begin{tabular}{@{}lr@{}}
\toprule
Model & Score \\
\midrule
\multicolumn{2}{c}{7B Models} \\
\midrule
Qwen2.5-VL-7B      & 35.07 \\
MM-Eureka-7B       & 35.96 \\
VL-Rethinker-7B    & 37.25 \\
\textbf{Orsta-7B}  & \textbf{38.31} \\
$\Delta$ (Ours - Backbone) & +3.24 \\
\bottomrule
\end{tabular}

\vspace{5pt}

% -------- 32B 0321 --------
\begin{tabular}{@{}lr@{}}
\toprule
\multicolumn{2}{c}{32B Models (0321)} \\
\midrule
Qwen2.5-VL-32B-0321     & 11.87 \\
MM-Eureka-32B           & 18.57 \\
VL-Rethinker-32B        & 19.41 \\
\textbf{Orsta-32B-0321} & \textbf{25.94} \\
$\Delta$ (Ours - Backbone) & +14.07 \\
\bottomrule
\end{tabular}

\vspace{5pt}

% -------- 32B 0326 --------
\begin{tabular}{@{}lr@{}}
\toprule
\multicolumn{2}{c}{32B Models (0326)} \\
\midrule
Qwen2.5-VL-32B-0326     & 43.67 \\
Gemma3-27B              & 41.82 \\
InternVL-3-38B          & \textbf{46.69} \\
\textbf{Orsta-32B-0326} & 45.77 \\
$\Delta$ (Ours - Backbone) & +2.10 \\
\bottomrule
\end{tabular}

\end{minipage}
\hfill
% ================= RIGHT COLUMN =================
\begin{minipage}[t]{0.68\linewidth}
\vspace{0pt}
\centering

% -------- Baseline comparison --------
\captionof{table}{Comparison against strong multi-task RL-VLM baselines on reasoning and perception benchmarks.}
\label{tab:baseline_comparison}

\scriptsize
\setlength{\tabcolsep}{3pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{6}{c}{\textbf{Reasoning Benchmarks}} \\
\midrule
Model & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) \\
\midrule
\textbf{Orsta-7B}       & \textbf{57.10} & 72.50 & 31.73 & \textbf{31.14} & \textbf{48.40} \\
MM-Eureka-7B            & 55.33          & 74.10 & 30.84 & 28.45          & 42.10 \\
VL-Rethinker-7B         & 56.70          & \textbf{75.40} & \textbf{32.46} & 29.38 & 44.00 \\
VisionReasoner-7B       & 56.56          & 69.70 & 29.20 & 25.84          & 41.20 \\
\bottomrule
\end{tabular}
}

\vspace{5pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{6}{c}{\textbf{Perception Benchmarks}} \\
\midrule
Model & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
\midrule
\textbf{Orsta-7B}       & \textbf{77.25} & \textbf{81.68} & \textbf{80.73} $\mid$ \textbf{41.41} & \textbf{56.05} & 23.91 \\
MM-Eureka-7B            & 59.62          & 57.07          & 79.73 $\mid$ 35.84                   & 53.38          & 24.23 \\
VL-Rethinker-7B         & 65.12          & 68.60          & 72.50 $\mid$ 31.54                   & 55.70          & \textbf{24.48} \\
VisionReasoner-7B       & 74.38          & 80.63          & 80.22 $\mid$ 36.58                   & 55.44          & 24.23 \\
\bottomrule
\end{tabular}
}

\vspace{10pt}

% -------- GUI extension --------
\captionof{table}{Extension to a new GUI task domain with 3K ShowUI samples under the same 60-step fixed-compute budget.}
\label{tab:gui_extension}
\vspace{4pt}


\small
\setlength{\tabcolsep}{20pt}

\resizebox{0.99\linewidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Mixture & ScreenSpot-Pro & OCRBenchV2 \\
\midrule
Unified           & 23.91         & 55.87 \\
Perception-only   & 23.78         & 55.33 \\
Perception-only + GUI-3K          & 29.85         & 55.96 \\
Unified + GUI-3K             & \textbf{31.68} & \textbf{56.09} \\
\bottomrule
\end{tabular}
}

\end{minipage}

\end{table*}

\subsection{General Performance on MEGA-Bench}
\label{subsec:mega_bench}

The fixed-budget results in~\cref{subsec:fair_budget} show that unified RL training matches or outperforms specialist mixtures under matched budgets.
%
We now turn to the final Orsta models and report their overall performance on MEGA-Bench, which spans over 440 diverse tasks for general VLM capability.
%
For each backbone, we train both on-policy and off-policy variants for 3 epochs, designate one model as Orsta based on its MEGA-Bench performance, and evaluate that same selected model on all subsequent benchmarks.
%
We provide the full MEGA-Bench evaluation curves in~\cref{appx:mega_bench_curves}.

Overall, Orsta consistently improves the MEGA-Bench performance of its base model at both 7B and 32B scales.
%
For the 7B model, unified RL post-training yields a clear overall gain.
%
The same pattern holds at 32B, but with two different gain profiles in~\cref{tab:mega_bench_core}: for the \texttt{0321} checkpoint,\footnote{\texttt{0321} and \texttt{0326} follow the release dates of the public HuggingFace checkpoints. The former shows noticeably weaker perception and formatting abilities, while the latter is a stronger later release.} RL post-training brings a much larger improvement; for the stronger \texttt{0326} checkpoint, V-Triune still delivers stable and notable gains.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/combined_iou_train_disable_vit.pdf}
\caption{Dynamic IoU ablations and source-level diagnostics. (a) Dynamic IoU ablations on COCO multi-object using only the detection and grounding subsets for training. The left plot compares fixed IoU@50, fixed IoU@99, and the main Dynamic IoU schedule; the right plot compares alternative staged schedules. Fixed IoU@50 learns quickly but degrades later, whereas fixed IoU@99 is more stable but learns more slowly; the main Dynamic IoU schedule gives the best balance. (b) Source-level logs from full 8-task Orsta-32B unified RL training show that the reasoning-heavy Puzzle source has increasing response length and reflection ratio, whereas the localization-centric Detection source remains short and nearly reflection-free. (c) In a full 8-task 7B training ablation that updates the ViT only, the LLM only, or both, continuing to update the vision encoder hurts COCO performance and increases gradient norms, motivating the decision to freeze the vision encoder and connector in the main experiments. More detailed failure analyses are provided in~\cref{sec:training_recipe}.}
\label{fig:combined_iou_source_level}
\end{figure*}


\subsection{Comparison with Strong Multi-task RL-VLM Baselines}
\label{subsec:baseline_comparison}

Beyond the overall MEGA-Bench gains in~\cref{subsec:mega_bench}, we compare Orsta-7B against three strong multi-task RL-VLM baselines on the same 10-benchmark suite as in~\cref{subsec:fair_budget}.
%
MM-Eureka-7B~\citep{meng2025mm} and VL-Rethinker-7B~\citep{vl_rethinker} are more reasoning-oriented, whereas VisionReasoner-7B~\citep{liu2025visionreasoner} is more perception-centric.

As shown in~\cref{tab:baseline_comparison}, Orsta-7B achieves the best score on 7/10 benchmarks.
%
On the reasoning side, it wins MMMU, MME-Reasoning, and CharXiv(RQ), while staying competitive on MathVista and MathVision.
%
On the perception side, it reaches the top score on 4/5 benchmarks, with the clearest margin on the challenging COCO multi-object setting.

This complements the fair-budget evidence in~\cref{subsec:fair_budget}: the benefit of unified training remains visible in the final model and is not confined to either reasoning or perception alone.

\subsection{Why is Dynamic IoU Necessary for Localization Tasks?}
\label{subsec:dynamic_iou_ablation}

We next examine why Dynamic IoU is necessary for localization-centric tasks and why a staged schedule is effective.
%
Unless otherwise stated, the ablations in this subsection use only the detection and grounding subsets of the training data in the same 7B off-policy setup.
%
The main schedule uses IoU thresholds $0.85$, $0.95$, and $0.99$ over the first 10\%, the next 15\%, and the remaining training steps.

On COCO multi-object, the fixed-threshold comparison in~\cref{fig:combined_iou_source_level}(a) shows the two failure modes directly.
%
IoU@50 learns quickly but degrades later, which we attribute to reward ambiguity under a loose threshold.
%
Qualitative cases in~\cref{appx:dynamic_iou_cases} support this interpretation: late-stage predictions often drift among multiple coarse boxes that remain similarly rewarded under IoU@50, rather than continuing to sharpen around the ground-truth box.
%
IoU@99 is more precise but learns much more slowly because the reward is too sparse early on.
%
Dynamic IoU avoids both issues by remaining learnable early while enforcing higher precision later.
%
We further compare alternative staged schedules in~\cref{fig:combined_iou_source_level}(a).
%
The loose variant ($0.7 \rightarrow 0.8 \rightarrow 0.85$) plateaus because its final threshold remains too permissive, whereas the strict variant ($0.9 \rightarrow 0.95 \rightarrow 0.99$) slows early learning by making the initial reward too sparse.
%
Our main schedule ($0.85 \rightarrow 0.95 \rightarrow 0.99$) gives the best balance.

The same advantage pattern also appears on the OVDEval negation subset; full curves are given in~\cref{appx:ovd_dynamic_iou}.
%
We also implemented an adaptive scheduler based on the batch-level bbox success rate, but it does not yield a clear advantage over the fixed three-stage schedule in our setting; full results are given in~\cref{appx:adaptive}.


\subsection{What Do Source-Level Diagnostics Reveal?}
\label{subsec:source_level_diagnostics}

These diagnostics reveal signals that aggregate metrics can easily hide, revealing both task-dependent response behavior and failure modes that directly affect training stability~(\cref{fig:combined_iou_source_level}).

On the behavior side, \cref{fig:combined_iou_source_level}(b) uses Puzzle and Detection as two representative sources and shows unified training does not collapse them into the same response pattern.
%
For the reasoning-heavy Puzzle source, both response length and reflection ratio increase over training.
%
For the localization-centric Detection source, responses remain short and direct, and reflection stays low.
%
This suggests unified training preserves task-appropriate response patterns across task families.
%
More detailed multi-source dynamics are provided in~\cref{sec:training_dynamics_analysis}.

On stability side, \cref{fig:combined_iou_source_level}(c) shows that continuing to update the vision encoder quickly hurts COCO performance and increases total gradient norms.
%
\cref{sec:training_recipe} further shows that this instability appears as gradient explosion in the ViT and soon hurts detection and grounding performance.
%
The same source-level logs also exposed leaked image special tokens in model responses, which can cause the number of visual features to no longer match the input sequence and directly lead to training failure.
%
Based on these findings, we freeze the vision encoder and connector in the main experiments and filter leaked image special tokens before reward recomputation; more detailed layer-wise gradients, image-token failure cases, and stability analysis are provided in~\cref{sec:training_recipe}.

\subsection{Can V-Triune Extend to New Task Domains?}
\label{subsec:gui_extension}

Finally, we test whether V-Triune can absorb a new task domain beyond the original training mix, and whether the benefit of unified training remains after the new domain is added.
%
As a concrete case, we add about 3K GUI grounding samples from ShowUI~\citep{lin2025showui}, a domain not covered in the original dataset.
%
We treat GUI grounding as a new domain to test the scalability of our framework, which can be added by reusing the existing localization-style verifier regime.

As shown in~\cref{tab:gui_extension}, adding ShowUI data substantially improves ScreenSpot-Pro, with the unified model rising from 23.91 to 31.68.
%
Notably, after adding the same GUI data, \textit{Unified + GUI} still outperforms \textit{Perception + GUI} by +1.83 points on ScreenSpot-Pro.
%
Reasoning-heavy data therefore does not block learning in the new GUI domain, and unified training continues to provide positive transfer once the model has basic in-domain visual support.

These results suggest that V-Triune can extend beyond the original training domains while preserving the benefit of unified training.
%
In the ShowUI case, this extension is straightforward because the GUI task can reuse the existing localization-style verifier regime.



% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3.5pt}
% \caption{Performance on MEGA-Bench Core. Orsta consistently improves its backbone at both 7B and 32B scales, with especially large gains on the weaker 32B-0321 checkpoint.}
% \label{tab:mega_bench_core}
% \begin{tabular}{@{}l r|l r|l r@{}}
% \toprule
% \multicolumn{2}{c|}{7B Models} & \multicolumn{2}{c|}{32B Models (0321)} & \multicolumn{2}{c}{32B Models (0326)} \\
% \midrule
% Model & Score & Model & Score & Model & Score \\
% \midrule
% Qwen2.5-VL-7B & 35.07
% & Qwen2.5-VL-32B-0321 & 11.87
% & Qwen2.5-VL-32B-0326 & 43.67 \\
% MM-Eureka-7B & 35.96
% & MM-Eureka-32B & 18.57
% & Gemma3-27B & 41.82 \\
% VL-Rethinker-7B & 37.25
% & VL-Rethinker-32B & 19.41
% & InternVL-3-38B & \textbf{46.69} \\
% \textbf{Orsta-7B} & \textbf{38.31}
% & \textbf{Orsta-32B-0321} & \textbf{25.94}
% & \textbf{Orsta-32B-0326} & 45.77 \\
% $\Delta$ (Ours - Backbone) & +3.24
% & $\Delta$ (Ours - Backbone) & +14.07
% & $\Delta$ (Ours - Backbone) & +2.10 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \caption{Extension to a new GUI task domain with 3K ShowUI samples under the same 60-step fixed-compute budget.}
% \label{tab:gui_extension}
% \begin{tabular}{lcc}
% \toprule
% Mixture & ScreenSpot-Pro & OCRBenchV2 \\
% \midrule
% Unified (original) & 23.91 & 55.87 \\
% Perception-only (original) & 23.78 & 55.33 \\
% Perception + GUI-3K & 29.85 & 55.96 \\
% Unified + GUI-3K & \textbf{31.68} & \textbf{56.09} \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}[t]
% \centering
% \caption{Comparison against strong multi-task RL-VLM baselines on 10 reasoning and perception benchmarks. COCO (S$\mid$M) reports single-object and multi-object mAP. Best results are bolded.}
% \label{tab:baseline_comparison}
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc}
% \toprule
% Model & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
% \midrule
% \textbf{Orsta-7B} & \textbf{57.10} & 72.50 & 31.73 & \textbf{31.14} & \textbf{48.40} & \textbf{77.25} & \textbf{81.68} & \textbf{80.73} $\mid$ \textbf{41.41} & \textbf{56.05} & 23.91 \\
% MM-Eureka-7B & 55.33 & 74.10 & 30.84 & 28.45 & 42.10 & 59.62 & 57.07 & 79.73 $\mid$ 35.84 & 53.38 & 24.23 \\
% VL-Rethinker-7B & 56.70 & \textbf{75.40} & \textbf{32.46} & 29.38 & 44.00 & 65.12 & 68.60 & 72.50 $\mid$ 31.54 & 55.70 & \textbf{24.48} \\
% VisionReasoner-7B & 56.56 & 69.70 & 29.20 & 25.84 & 41.20 & 74.38 & 80.63 & 80.22 $\mid$ 36.58 & 55.44 & 24.23 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{images/figure5/iou_coco_combined.pdf}
%   \caption{Dynamic IoU ablations for localization-centric RL. (a) On COCO multi-object, fixed IoU@50 learns quickly but degrades later, while fixed IoU@99 is more stable but learns more slowly; Dynamic IoU achieves the best overall trajectory. (b) On the same benchmark, compared with loose and strict staged schedules, our $0.85 \rightarrow 0.95 \rightarrow 0.99$ schedule provides the best balance between early learnability and late precision enforcement. (c) On the OVDEval negation subset~\citep{yao2024evaluate}, Dynamic IoU also improves over fixed IoU@99, showing that the advantage extends beyond COCO.}
% \label{fig:dynamic_iou_ablation}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{images/combined_train_disable_vit.pdf}
% \caption{Source-level diagnostics in unified RL. (a) In Orsta-32B-0321 unified RL training, the reasoning-heavy Puzzle source shows increasing response length and reflection ratio, whereas the localization-centric Detection source remains short and nearly reflection-free, indicating task-dependent response behavior. (b) Continuing to update the vision encoder causes COCO performance to drop and total gradient norms to grow sharply, motivating the decision to freeze the vision encoder and connector in the main experiments. More detailed failure analyses are provided in~\cref{sec:training_recipe}.}
% \label{fig:source_level_diagnostics}
% \end{figure*}


==> sections_refined/5_experiment_v3.tex <==
\section{Experiment}
\label{sec:experiment}

\begin{table*}[t]
\centering
\caption{Fair-budget evidence under a fixed training budget. Left: MEGA-Bench task-composition curves for the 7B off-policy setting. Right: benchmark breakdown at the same 60-step budget. Unified = Reason+Perception. MME-R = MME-Reasoning~\citep{yuan2025mme}. CharXiv(RQ) = CharXiv Reasoning Question. COCO (S$\mid$M) reports single-object and multi-object mAP in COCO val-2017. COCO mAP uses the standard cocoapi; see details in~\cref{sec:coco_evaluation}. Best results are bolded and second-best results are underlined.}
\label{fig:fair_budget_evidence}
\begin{minipage}[t]{0.31\textwidth}
\vspace{-1pt}
\centering
\includegraphics[width=\linewidth]{images/figure6/7b_task_new.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.68\textwidth}
\vspace{0pt}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Reasoning Benchmarks} \\
\midrule
Mixture & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) \\
\midrule
Unified & \underline{56.56} & \underline{71.40} & \underline{30.51} & \textbf{28.20} & \textbf{44.50} \\
Reason-only & 54.89 & \textbf{71.70} & \textbf{31.24} & \underline{28.03} & \underline{44.00} \\
Perception-only & \textbf{56.67} & 68.20 & 29.59 & 26.26 & 41.00 \\
\bottomrule
\end{tabular}
}

\vspace{4pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\multicolumn{6}{c}{Perception Benchmarks} \\
\midrule
Mixture & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
\midrule
Unified & \underline{73.75} & \textbf{82.20} & \underline{80.69} $\mid$ \textbf{38.62} & \textbf{55.87} & \underline{23.91} \\
Reason-only & 73.25 & 78.53 & 78.36 $\mid$ 33.87 & \underline{55.77} & \textbf{23.97} \\
Perception-only & \textbf{76.00} & \underline{80.10} & \textbf{80.78} $\mid$ \underline{37.37} & 55.33 & 23.78 \\
\bottomrule
\end{tabular}
}
\end{minipage}
\end{table*}
%
\vspace{-5pt}

\subsection{Experimental Setup}
\label{subsec:implementation details}

We evaluate V-Triune at two levels.
%
First, under a fixed budget, we compare a unified mixture against two specialist mixtures: \textit{Reason-only} and \textit{Perception-only}.
%
Second, we report the final Orsta models under a longer training horizon to evaluate overall competitiveness on broad and task-specific benchmarks.

We use Qwen2.5-VL-7B and 32B~\citep{Qwen2.5-VL} as backbones.
%
We study unified RL post-training on strong public VLM backbones when the target outcomes are verifiable.
%
RL post-training uses a 47.7K-sample VQA training set with verifiable answers from 18 sources, covering four reasoning tasks (math, puzzle, science, and chart) and four perception tasks (detection, grounding, counting, and OCR).
%
Detailed data construction is given in~\cref{subsec:data,tab:data_source}.
%
Appendix~\cref{sec:curated_vs_random} further reports a matched-count curated-versus-random control to separate data quality from the training methodology.
%
We use GRPO~\citep{shao2024deepseekmath} in all main experiments, with a rollout batch size of 1024 and 8 sampled responses per prompt, and implement the unified RL pipeline on top of Verl~\citep{sheng2024hybridflow}.
%
Controlled comparisons use a fixed training budget, whereas final-model results use 3 training epochs.
%
For stability, we freeze the vision encoder and update only the LLM layers.
%
Rollouts are generated with vLLM using \texttt{temperature=1.0}, \texttt{top-p=1.0}, and \texttt{max\_length=2048}, and localization tasks use a three-stage Dynamic IoU schedule.

\subsection{Does Unified Training Help Under Fair Budgets?}
\label{subsec:fair_budget}

We first study unified training under a fixed training budget.
%
Unless otherwise stated, all fair-budget comparisons use the same 7B off-policy with 8 optimization steps per rollout.
%
We compare the unified mixture against two specialist mixtures under the same budget.

The left panel of~\cref{fig:fair_budget_evidence} provides the first evidence through the MEGA-Bench task-composition curves.
%
Under the same 60-step budget, \textit{Reason+Perception} follows the strongest or tied-strongest trajectory throughout training.
%
This suggests that joint training does not introduce a clear reasoning-versus-perception trade-off on MEGA-Bench.

We further compare the same three mixtures on a 10-benchmark suite spanning both reasoning and perception, and report the fixed-budget benchmark breakdown in~\cref{fig:fair_budget_evidence}.
%
The benchmark list and evaluation protocols are given in~\cref{sec:eval_details}.
%
The unified mixture remains stronger or comparable on both sides and reaches the best result on multiple benchmarks.
%
Across this suite, the unified model matches or exceeds the specialist baselines on 5/10 benchmarks and stays close on the rest.

This indicates that unified training remains competitive despite less task-specific exposure.
%
This is consistent with better data efficiency under unified RL training and suggests mild cross-task regularization.
%
Why joint training helps remains open, however, and the source-level diagnostics in~\cref{subsec:source_level_diagnostics} help characterize how different task families behave under unified training.

% =============================================================================================

\begin{table*}[t]
\centering

% ================= LEFT COLUMN =================
\begin{minipage}[t]{0.29\linewidth}
\vspace{0pt}
\centering

\captionof{table}{Performance on MEGA-Bench Core.}
\label{tab:mega_bench_core}

\small
\setlength{\tabcolsep}{2pt}

% -------- 7B --------
\begin{tabular}{@{}lr@{}}
\toprule
Model & Score \\
\midrule
\multicolumn{2}{c}{7B Models} \\
\midrule
Qwen2.5-VL-7B      & 35.07 \\
MM-Eureka-7B       & 35.96 \\
VL-Rethinker-7B    & 37.25 \\
\textbf{Orsta-7B}  & \textbf{38.31} \\
$\Delta$ (Ours - Backbone) & +3.24 \\
\bottomrule
\end{tabular}

\vspace{5pt}

% -------- 32B 0321 --------
\begin{tabular}{@{}lr@{}}
\toprule
\multicolumn{2}{c}{32B Models (0321)} \\
\midrule
Qwen2.5-VL-32B-0321     & 11.87 \\
MM-Eureka-32B           & 18.57 \\
VL-Rethinker-32B        & 19.41 \\
\textbf{Orsta-32B-0321} & \textbf{25.94} \\
$\Delta$ (Ours - Backbone) & +14.07 \\
\bottomrule
\end{tabular}

\vspace{5pt}

% -------- 32B 0326 --------
\begin{tabular}{@{}lr@{}}
\toprule
\multicolumn{2}{c}{32B Models (0326)} \\
\midrule
Qwen2.5-VL-32B-0326     & 43.67 \\
Gemma3-27B              & 41.82 \\
InternVL-3-38B          & \textbf{46.69} \\
\textbf{Orsta-32B-0326} & 45.77 \\
$\Delta$ (Ours - Backbone) & +2.10 \\
\bottomrule
\end{tabular}

\end{minipage}
\hfill
% ================= RIGHT COLUMN =================
\begin{minipage}[t]{0.68\linewidth}
\vspace{0pt}
\centering

% -------- Baseline comparison --------
\captionof{table}{Comparison against strong multi-task RL-VLM baselines on reasoning and perception benchmarks.}
\label{tab:baseline_comparison}

\scriptsize
\setlength{\tabcolsep}{3pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{6}{c}{\textbf{Reasoning Benchmarks}} \\
\midrule
Model & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) \\
\midrule
\textbf{Orsta-7B}       & \textbf{57.10} & 72.50 & 31.73 & \textbf{31.14} & \textbf{48.40} \\
MM-Eureka-7B            & 55.33          & 74.10 & 30.84 & 28.45          & 42.10 \\
VL-Rethinker-7B         & 56.70          & \textbf{75.40} & \textbf{32.46} & 29.38 & 44.00 \\
VisionReasoner-7B       & 56.56          & 69.70 & 29.20 & 25.84          & 41.20 \\
\bottomrule
\end{tabular}
}

\vspace{5pt}

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multicolumn{6}{c}{\textbf{Perception Benchmarks}} \\
\midrule
Model & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
\midrule
\textbf{Orsta-7B}       & \textbf{77.25} & \textbf{81.68} & \textbf{80.73} $\mid$ \textbf{41.41} & \textbf{56.05} & 23.91 \\
MM-Eureka-7B            & 59.62          & 57.07          & 79.73 $\mid$ 35.84                   & 53.38          & 24.23 \\
VL-Rethinker-7B         & 65.12          & 68.60          & 72.50 $\mid$ 31.54                   & 55.70          & \textbf{24.48} \\
VisionReasoner-7B       & 74.38          & 80.63          & 80.22 $\mid$ 36.58                   & 55.44          & 24.23 \\
\bottomrule
\end{tabular}
}

\vspace{10pt}

% -------- GUI extension --------
\captionof{table}{Extension to a new GUI task domain with 3K ShowUI samples under the same 60-step fixed-compute budget.}
\label{tab:gui_extension}
\vspace{4pt}


\small
\setlength{\tabcolsep}{20pt}

\resizebox{0.99\linewidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Mixture & ScreenSpot-Pro & OCRBenchV2 \\
\midrule
Unified           & 23.91         & 55.87 \\
Perception-only   & 23.78         & 55.33 \\
Perception-only + GUI-3K          & 29.85         & 55.96 \\
Unified + GUI-3K             & \textbf{31.68} & \textbf{56.09} \\
\bottomrule
\end{tabular}
}

\end{minipage}

\end{table*}

\subsection{General Performance on MEGA-Bench}
\label{subsec:mega_bench}

The fixed-budget results in~\cref{subsec:fair_budget} show that unified RL training matches or outperforms specialist mixtures under matched budgets.
%
We now turn to the final Orsta models and report their overall performance on MEGA-Bench, which spans over 440 diverse tasks for general VLM capability.
%
For each backbone, we train both on-policy and off-policy variants for 3 epochs, designate one model as Orsta based on its MEGA-Bench performance, and evaluate that same selected model on all subsequent benchmarks.
%
We provide the full MEGA-Bench evaluation curves in~\cref{appx:mega_bench_curves}.

Overall, Orsta consistently improves the MEGA-Bench performance of its base model at both 7B and 32B scales.
%
For the 7B model, unified RL post-training yields a clear overall gain.
%
The same pattern holds at 32B, but with two different gain profiles in~\cref{tab:mega_bench_core}: for the \texttt{0321} checkpoint,\footnote{\texttt{0321} and \texttt{0326} follow the release dates of the public HuggingFace checkpoints. The former shows noticeably weaker perception and formatting abilities, while the latter is a stronger later release.} RL post-training brings a much larger improvement; for the stronger \texttt{0326} checkpoint, V-Triune still delivers stable and notable gains.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{images/combined_iou_train_disable_vit.pdf}
\caption{Dynamic IoU ablations and source-level diagnostics. (a) Dynamic IoU ablations on COCO multi-object using only the detection and grounding subsets for training. The left plot compares fixed IoU@50, fixed IoU@99, and the main Dynamic IoU schedule; the right plot compares alternative staged schedules. Fixed IoU@50 learns quickly but degrades later, whereas fixed IoU@99 is more stable but learns more slowly; the main Dynamic IoU schedule gives the best balance. (b) Source-level logs from full 8-task Orsta-32B unified RL training show that the reasoning-heavy Puzzle source has increasing response length and reflection ratio, whereas the localization-centric Detection source remains short and nearly reflection-free. (c) In a full 8-task 7B training ablation that updates the ViT only, the LLM only, or both, continuing to update the vision encoder hurts COCO performance and increases gradient norms, motivating the decision to freeze the vision encoder and connector in the main experiments. More detailed failure analyses are provided in~\cref{sec:training_recipe}.}
\label{fig:combined_iou_source_level}
\end{figure*}

\subsection{Comparison with Strong Multi-task RL-VLM Baselines}
\label{subsec:baseline_comparison}

Beyond the overall MEGA-Bench gains in~\cref{subsec:mega_bench}, we compare Orsta-7B against three strong multi-task RL-VLM baselines on the same 10-benchmark suite as in~\cref{subsec:fair_budget}.
%
MM-Eureka-7B~\citep{meng2025mm} and VL-Rethinker-7B~\citep{vl_rethinker} are more reasoning-oriented, whereas VisionReasoner-7B~\citep{liu2025visionreasoner} is more perception-centric.

As shown in~\cref{tab:baseline_comparison}, Orsta-7B achieves the best score on 7/10 benchmarks.
%
On the reasoning side, it wins MMMU, MME-Reasoning, and CharXiv(RQ), while staying competitive on MathVista and MathVision.
%
On the perception side, it reaches the top score on 4/5 benchmarks, with the clearest margin on the challenging COCO multi-object setting.
%
This complements the fair-budget evidence in~\cref{subsec:fair_budget}: the benefit of unified training remains visible in the final model and is not confined to either reasoning or perception alone.

\subsection{Why is Dynamic IoU Necessary for Localization Tasks?}
\label{subsec:dynamic_iou_ablation}

We next examine why Dynamic IoU is necessary for localization-centric tasks and why a staged schedule is effective.
%
Unless otherwise stated, the ablations in this subsection use only the detection and grounding subsets of the training data in the same 7B off-policy setup.
%
The main schedule uses IoU thresholds $0.85$, $0.95$, and $0.99$ over the first 10\%, the next 15\%, and the remaining training steps.

On COCO multi-object, the fixed-threshold comparison in~\cref{fig:combined_iou_source_level}(a) shows the two failure modes directly.
%
IoU@50 learns quickly but degrades later, which we attribute to reward ambiguity under a loose threshold.
%
Qualitative cases in~\cref{appx:dynamic_iou_cases} support this interpretation: late-stage predictions often drift among multiple coarse boxes that remain similarly rewarded under IoU@50, rather than continuing to sharpen around the ground-truth box.
%
IoU@99 is more precise but learns much more slowly because the reward is too sparse early on.
%
Dynamic IoU avoids both issues by remaining learnable early while enforcing higher precision later.
%
We further compare alternative staged schedules in~\cref{fig:combined_iou_source_level}(a).
%
The loose variant ($0.7 \rightarrow 0.8 \rightarrow 0.85$) plateaus because its final threshold remains too permissive, whereas the strict variant ($0.9 \rightarrow 0.95 \rightarrow 0.99$) slows early learning by making the initial reward too sparse.
%
Our main schedule ($0.85 \rightarrow 0.95 \rightarrow 0.99$) gives the best balance.

The same advantage pattern also appears on the OVDEval negation subset; full curves are given in~\cref{appx:ovd_dynamic_iou}.
%
We also implemented an adaptive scheduler based on the batch-level bbox success rate, but it does not yield a clear advantage over the fixed three-stage schedule in our setting; full results are given in~\cref{appx:adaptive}.


\subsection{What Do Source-Level Diagnostics Reveal?}
\label{subsec:source_level_diagnostics}

These diagnostics reveal signals that aggregate metrics can easily hide: global averages may look stable while source-specific response behavior and failure modes diverge during training~(\cref{fig:combined_iou_source_level}).

On the behavior side, \cref{fig:combined_iou_source_level}(b) uses Puzzle and Detection as two representative sources and shows unified training does not collapse them into the same response pattern.
%
For the reasoning-heavy Puzzle source, both response length and reflection ratio increase over training.
%
For the localization-centric Detection source, responses remain short and direct, and reflection stays low.
%
This suggests unified training preserves task-appropriate response patterns across task families.
%
Combined with the fair-budget results, this supports the view that joint training may have mild cross-task regularization while still allowing different task families to use different response strategies.
%
More detailed multi-source dynamics are provided in~\cref{sec:training_dynamics_analysis}.

On stability side, \cref{fig:combined_iou_source_level}(c) shows that continuing to update the vision encoder quickly hurts COCO performance and increases total gradient norms.
%
\cref{sec:training_recipe} further shows that this instability appears as gradient explosion in the ViT and soon hurts detection and grounding performance.
%
The same source-level logs also exposed leaked image special tokens in model responses, which can cause the number of visual features to no longer match the input sequence and directly lead to training failure.
%
Based on these findings, we freeze the vision encoder and connector in the main experiments and filter leaked image special tokens before reward recomputation; more detailed layer-wise gradients, image-token failure cases, and stability analysis are provided in~\cref{sec:training_recipe}.

\subsection{Can V-Triune Extend to New Task Domains?}
\label{subsec:gui_extension}

Finally, we test whether V-Triune can absorb a new task domain beyond the original training mix, and whether the benefit of unified training remains after the new domain is added.
%
As a concrete case, we add about 3K GUI grounding samples from ShowUI~\citep{lin2025showui}, a domain not covered in the original dataset.
%
We treat GUI grounding as a new domain to test the scalability of our framework, which can be added by reusing the existing localization-style verifier regime.

As shown in~\cref{tab:gui_extension}, adding ShowUI data substantially improves ScreenSpot-Pro, with the unified model rising from 23.91 to 31.68.
%
Notably, after adding the same GUI data, \textit{Unified + GUI} still outperforms \textit{Perception + GUI} by +1.83 points on ScreenSpot-Pro.
%
Reasoning-heavy data therefore does not block learning in the new GUI domain, and unified training continues to show positive transfer once the model has basic in-domain visual support.

These results suggest that V-Triune can extend beyond the original training domains while preserving the benefit of unified training.
%
In the ShowUI case, this extension is straightforward because the GUI task can reuse the existing localization-style verifier regime.



% \begin{table*}[t]
% \centering
% \small
% \setlength{\tabcolsep}{3.5pt}
% \caption{Performance on MEGA-Bench Core. Orsta consistently improves its backbone at both 7B and 32B scales, with especially large gains on the weaker 32B-0321 checkpoint.}
% \label{tab:mega_bench_core}
% \begin{tabular}{@{}l r|l r|l r@{}}
% \toprule
% \multicolumn{2}{c|}{7B Models} & \multicolumn{2}{c|}{32B Models (0321)} & \multicolumn{2}{c}{32B Models (0326)} \\
% \midrule
% Model & Score & Model & Score & Model & Score \\
% \midrule
% Qwen2.5-VL-7B & 35.07
% & Qwen2.5-VL-32B-0321 & 11.87
% & Qwen2.5-VL-32B-0326 & 43.67 \\
% MM-Eureka-7B & 35.96
% & MM-Eureka-32B & 18.57
% & Gemma3-27B & 41.82 \\
% VL-Rethinker-7B & 37.25
% & VL-Rethinker-32B & 19.41
% & InternVL-3-38B & \textbf{46.69} \\
% \textbf{Orsta-7B} & \textbf{38.31}
% & \textbf{Orsta-32B-0321} & \textbf{25.94}
% & \textbf{Orsta-32B-0326} & 45.77 \\
% $\Delta$ (Ours - Backbone) & +3.24
% & $\Delta$ (Ours - Backbone) & +14.07
% & $\Delta$ (Ours - Backbone) & +2.10 \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{5pt}
% \caption{Extension to a new GUI task domain with 3K ShowUI samples under the same 60-step fixed-compute budget.}
% \label{tab:gui_extension}
% \begin{tabular}{lcc}
% \toprule
% Mixture & ScreenSpot-Pro & OCRBenchV2 \\
% \midrule
% Unified (original) & 23.91 & 55.87 \\
% Perception-only (original) & 23.78 & 55.33 \\
% Perception + GUI-3K & 29.85 & 55.96 \\
% Unified + GUI-3K & \textbf{31.68} & \textbf{56.09} \\
% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table*}[t]
% \centering
% \caption{Comparison against strong multi-task RL-VLM baselines on 10 reasoning and perception benchmarks. COCO (S$\mid$M) reports single-object and multi-object mAP. Best results are bolded.}
% \label{tab:baseline_comparison}
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc}
% \toprule
% Model & MMMU & MathVista & MathVision & MME-R & CharXiv (RQ) & HrBench4K & VStar & COCO (S$\mid$M) & OCRBenchV2 & ScreenSpot-Pro \\
% \midrule
% \textbf{Orsta-7B} & \textbf{57.10} & 72.50 & 31.73 & \textbf{31.14} & \textbf{48.40} & \textbf{77.25} & \textbf{81.68} & \textbf{80.73} $\mid$ \textbf{41.41} & \textbf{56.05} & 23.91 \\
% MM-Eureka-7B & 55.33 & 74.10 & 30.84 & 28.45 & 42.10 & 59.62 & 57.07 & 79.73 $\mid$ 35.84 & 53.38 & 24.23 \\
% VL-Rethinker-7B & 56.70 & \textbf{75.40} & \textbf{32.46} & 29.38 & 44.00 & 65.12 & 68.60 & 72.50 $\mid$ 31.54 & 55.70 & \textbf{24.48} \\
% VisionReasoner-7B & 56.56 & 69.70 & 29.20 & 25.84 & 41.20 & 74.38 & 80.63 & 80.22 $\mid$ 36.58 & 55.44 & 24.23 \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{images/figure5/iou_coco_combined.pdf}
%   \caption{Dynamic IoU ablations for localization-centric RL. (a) On COCO multi-object, fixed IoU@50 learns quickly but degrades later, while fixed IoU@99 is more stable but learns more slowly; Dynamic IoU achieves the best overall trajectory. (b) On the same benchmark, compared with loose and strict staged schedules, our $0.85 \rightarrow 0.95 \rightarrow 0.99$ schedule provides the best balance between early learnability and late precision enforcement. (c) On the OVDEval negation subset~\citep{yao2024evaluate}, Dynamic IoU also improves over fixed IoU@99, showing that the advantage extends beyond COCO.}
% \label{fig:dynamic_iou_ablation}
% \end{figure*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{images/combined_train_disable_vit.pdf}
% \caption{Source-level diagnostics in unified RL. (a) In Orsta-32B-0321 unified RL training, the reasoning-heavy Puzzle source shows increasing response length and reflection ratio, whereas the localization-centric Detection source remains short and nearly reflection-free, indicating task-dependent response behavior. (b) Continuing to update the vision encoder causes COCO performance to drop and total gradient norms to grow sharply, motivating the decision to freeze the vision encoder and connector in the main experiments. More detailed failure analyses are provided in~\cref{sec:training_recipe}.}
% \label{fig:source_level_diagnostics}
% \end{figure*}


==> sections_refined/6_related_work_v1.tex <==
\section{Related Work}

RL post-training is expanding from language models to multimodal models, and an increasing number of works have begun to explore reinforcement post-training for vision-language models.
%
Compared with text-only settings, however, public recipes still remain largely organized around specific task families, and a unified training recipe across reasoning-heavy and perception-heavy tasks is still unclear.

One line of work focuses on visual reasoning.
%
Models such as Vision-R1~\citep{huang2025vision}, R1-OneVision~\citep{yang2025r1}, MM-Eureka~\citep{meng2025mm}, VL-Rethinker~\citep{vl_rethinker}, and GThinker mainly target mathematics, science, or more general multimodal reasoning tasks, typically using rule-based rewards and R1-style post-training to improve complex reasoning.
%
These works have substantially advanced multimodal reasoning RL, but their task composition and reward regimes still remain centered on reasoning-heavy problems.

Another line of work focuses on perception-heavy or relatively homogeneous visual tasks.
%
Visual-RFT~\citep{liu2025visual}, DeepPerception~\citep{ma2025deepperception}, Reason-RFT~\citep{tan2025reason}, Perception-R1~\citep{yu2025perception}, VLM-R1~\citep{shen2025vlm}, and VisionReasoner~\citep{liu2025visionreasoner} show that RL can be effective for detection, grounding, OCR, counting, segmentation, and related visual tasks, and some of them further explore task-specific reward designs such as IoU- or mAP-based signals.
%
These studies make clear that perception tasks are not outside the scope of RL, but they mostly remain within perception-only settings or relatively homogeneous task families.
%
Overall, neither reasoning-centric nor perception-centric prior work directly answers how reasoning-heavy and perception-heavy tasks can stably coexist within the same RL training framework.

Mixed-R1 mainly unifies multimodal RL post-training from the perspective of mixed answer types and mixed reward design, while also extending the setting to open-ended text rewards.
%
OneThinker studies an image-video all-in-one setting and addresses reward balancing in heterogeneous multi-task training through optimizer-side reward normalization and a GRPO variant.
%
These works suggest that multimodal RL is moving beyond isolated capability families toward more unified training settings.
%
In contrast, our work focuses on joint RL training over reasoning-heavy and perception-heavy tasks in open VLMs, where task, capability, and verification heterogeneity must be handled together.

Our distinction from prior work is therefore not a new RL optimizer, nor simply broader task coverage, but a unified multimodal RL training framework for a heterogeneous reasoning-plus-perception setting.
%
The gap we target is a public training recipe that must simultaneously support multiple task families within one RL pipeline, heterogeneous verifiers, specialized reward design for localization tasks, and fine-grained diagnosis of unified training dynamics.


==> sections_refined/6_related_work_v2.tex <==
\section{Related Work}

RL post-training is expanding from language models to multimodal models, and more works have begun to explore reinforcement post-training for vision-language models~\citep{}.
%
Compared with text-only settings, however, public recipes still remain largely organized around specific task families, and a unified training recipe across reasoning-heavy and perception-heavy tasks is still unclear~\citep{}.

One line of work focuses on visual reasoning.
%
Vision-R1~\citep{huang2025vision}, R1-OneVision~\citep{yang2025r1}, MM-Eureka~\citep{meng2025mm}, VL-Rethinker~\citep{vl_rethinker}, and GThinker~\citep{zhan2025gthinker} mainly target mathematics, science, or more general multimodal reasoning tasks, typically using rule-based rewards and R1-style post-training to improve complex reasoning.
%
Another line of work focuses on perception-heavy or relatively homogeneous visual tasks.
%
Visual-RFT~\citep{liu2025visual}, DeepPerception~\citep{ma2025deepperception}, Reason-RFT~\citep{tan2025reason}, Perception-R1~\citep{yu2025perception}, VLM-R1~\citep{shen2025vlm}, and VisionReasoner~\citep{liu2025visionreasoner} show that RL can be effective for detection, grounding, OCR, counting, segmentation, and related tasks, often with task-specific rewards such as IoU- or mAP-based signals.
%
Overall, neither reasoning-centric nor perception-centric prior work directly answers how reasoning-heavy and perception-heavy tasks can stably coexist within the same RL training framework.

Mixed-R1~\citep{xu2025mixedr1} mainly unifies multimodal RL post-training from the perspective of mixed answer types and mixed reward design, while also extending the setting to open-ended text rewards.
%
OneThinker~\citep{feng2025onethinker} studies an image-video all-in-one setting and addresses reward balancing in heterogeneous multi-task training through optimizer-side reward normalization and a GRPO~\citep{shao2024deepseekmath} variant.
%
In contrast, our work focuses on joint RL training over reasoning-heavy and perception-heavy tasks in open VLMs, where task, capability, and verification heterogeneity must be handled together.
%
Our distinction from prior work is therefore not a new RL optimizer, nor simply broader task coverage, but a unified multimodal RL training framework for a heterogeneous reasoning-plus-perception setting.


==> sections_refined/6_related_work_v3.tex <==
\section{Related Work}

RL post-training is becoming important for foundation models and is extending from language models to multimodal models~\citep{liu2025deepseek,qwen3.5,team2026kimi,team2025longcat,xiao2026mimo}.
%
However, public multimodal RL recipes remain much less mature than their text-only counterparts, especially for setups that span heterogeneous tasks and reward regimes.
%
As a result, existing VLM-RL work is still mostly organized around particular capability families or relatively homogeneous task settings, rather than a unified recipe for jointly training reasoning-heavy and perception-heavy tasks.

Prior work on VLM-RL has largely followed two lines.
%
Vision-R1~\citep{huang2025vision}, R1-OneVision~\citep{yang2025r1}, MM-Eureka~\citep{meng2025mm}, VL-Rethinker~\citep{vl_rethinker}, and GThinker~\citep{zhan2025gthinker} mainly target mathematics, science, and related multimodal reasoning tasks, typically using rule-based rewards and R1-style post-training to improve reasoning.
%
These works have substantially advanced multimodal reasoning RL, but their task composition and reward design still remain centered on reasoning-heavy problems.

The other focuses on perception-heavy or relatively homogeneous visual tasks.
%
Visual-RFT~\citep{liu2025visual}, DeepPerception~\citep{ma2025deepperception}, Reason-RFT~\citep{tan2025reason}, Perception-R1~\citep{yu2025perception}, VLM-R1~\citep{shen2025vlm}, and VisionReasoner~\citep{liu2025visionreasoner} show that RL can be effective for detection, grounding, OCR, counting, segmentation, and related tasks, often with task-specific rewards such as IoU or mAP.
%
Taken together, these lines do not directly answer how reasoning-heavy and perception-heavy tasks can stably coexist within the same RL training framework.

Mixed-R1~\citep{xu2025mixedr1} unifies multimodal RL post-training around mixed answer types and mixed reward design, while also extending the setting to open-ended text rewards.
%
OneThinker~\citep{feng2025onethinker} studies an image-video all-in-one setting and addresses heterogeneous multi-task training through optimizer-side reward normalization and a GRPO~\citep{shao2024deepseekmath} variant.
%
These works move toward more unified multimodal RL settings, but they address different problems from ours.
%
In contrast, our work focuses on joint RL training over reasoning-heavy and perception-heavy tasks in open VLMs, where task, capability, and verification heterogeneity must be handled within one pipeline.

Our contribution is therefore not a new RL algorithm, nor simply broader task coverage, but a unified multimodal RL training framework for a heterogeneous reasoning-plus-perception setting.
%
The gap we target is a public training recipe that supports multiple task families in one RL pipeline, heterogeneous verifiers, reward design, and fine-grained observability of unified training dynamics.


==> sections_refined/6_related_work_v4.tex <==
\section{Related Work}

RL post-training is becoming important for foundation models and is extending from language models to multimodal models~\citep{liu2025deepseek,qwen3.5,team2026kimi,team2025longcat,xiao2026mimo}.
%
However, public multimodal RL recipes remain much less mature than their text-only counterparts, especially for setups that span heterogeneous tasks and reward regimes.
%
As a result, most existing VLM-RL work is still organized around particular capability families or relatively homogeneous task settings, rather than a unified recipe for jointly training reasoning-heavy and perception-heavy tasks.

One major line of work focuses on multimodal reasoning.
%
Vision-R1~\citep{huang2025vision}, R1-OneVision~\citep{yang2025r1}, MM-Eureka~\citep{meng2025mm}, VL-Rethinker~\citep{vl_rethinker}, and GThinker~\citep{zhan2025gthinker} mainly target mathematics, science, and related reasoning tasks, typically using rule-based rewards and R1-style post-training to improve reasoning.
%
These works have substantially advanced multimodal reasoning RL, but their task composition and reward design remain centered on reasoning-heavy problems.

Another line focuses on perception-heavy or relatively homogeneous visual tasks.
%
Visual-RFT~\citep{liu2025visual}, DeepPerception~\citep{ma2025deepperception}, Reason-RFT~\citep{tan2025reason}, Perception-R1~\citep{yu2025perception}, VLM-R1~\citep{shen2025vlm}, and VisionReasoner~\citep{liu2025visionreasoner} show that RL can be effective for detection, grounding, OCR, counting, segmentation, and related tasks, often with task-specific rewards such as IoU or mAP.
%
Taken together, these two lines do not directly address how reasoning-heavy and perception-heavy tasks can stably coexist within the same RL training framework.

A smaller set of recent work moves toward more unified multimodal RL settings.
%
Mixed-R1~\citep{xu2025mixedr1} unifies multimodal RL post-training around mixed answer types and mixed reward design, while also extending the setting to open-ended text rewards.
%
OneThinker~\citep{feng2025onethinker} studies an image-video all-in-one setting and addresses heterogeneous multi-task training through optimizer-side reward normalization and a GRPO~\citep{shao2024deepseekmath} variant.
%
These works move toward more unified multimodal RL settings, but they address different problems from ours.
%
In contrast, our work focuses on joint RL training over reasoning-heavy and perception-heavy tasks in open VLMs, where task, capability, verification, and observability heterogeneity must all be handled within one pipeline.

Our work focuses on a unified multimodal RL training framework for a heterogeneous reasoning-plus-perception setting.
%
The key gap is a public training recipe that supports multiple task families in one pipeline, heterogeneous verifiers and reward design, and fine-grained observability of unified training dynamics.

% We therefore focus on a different gap: a public unified RL recipe that supports multiple task families in one pipeline, heterogeneous verifiers and reward design, and fine-grained observability of unified training dynamics.


==> sections_refined/6_related_work_v5.tex <==
\section{Related Work}

RL post-training is becoming important for foundation models and is extending from language models to multimodal models~\citep{liu2025deepseek,qwen3.5,team2026kimi,team2025longcat,xiao2026mimo}.
%
However, public multimodal RL recipes remain much less mature than their text-only counterparts, especially for setups that span heterogeneous tasks and reward regimes.
%
As a result, most existing VLM-RL work is still organized around particular capability families or relatively homogeneous task settings, rather than a unified recipe for jointly training reasoning-heavy and perception-heavy tasks.

One major line of work focuses on multimodal reasoning.
%
Vision-R1~\citep{huang2025vision}, R1-OneVision~\citep{yang2025r1}, MM-Eureka~\citep{meng2025mm}, VL-Rethinker~\citep{vl_rethinker}, and GThinker~\citep{zhan2025gthinker} mainly target mathematics, science, and related reasoning tasks, typically using rule-based rewards and R1-style post-training to improve reasoning.
%
These works have substantially advanced multimodal reasoning RL, but their task composition and reward design remain centered on reasoning-heavy problems.

Another line focuses on perception-heavy or relatively homogeneous visual tasks.
%
Visual-RFT~\citep{liu2025visual}, DeepPerception~\citep{ma2025deepperception}, Reason-RFT~\citep{tan2025reason}, Perception-R1~\citep{yu2025perception}, VLM-R1~\citep{shen2025vlm}, and VisionReasoner~\citep{liu2025visionreasoner} show that RL can be effective for detection, grounding, OCR, counting, segmentation, and related tasks, often with task-specific rewards such as IoU or mAP.
%
Taken together, these two lines do not directly address how reasoning-heavy and perception-heavy tasks can stably coexist within the same RL training framework.

A smaller set of recent work moves toward broader multimodal RL settings.
%
Mixed-R1~\citep{xu2025mixedr1} unifies multimodal RL post-training around mixed answer types and mixed reward design, while also extending the setting to open-ended text rewards.
%
OneThinker~\citep{feng2025onethinker} studies an image-video all-in-one setting and addresses heterogeneous multi-task training through optimizer-side reward normalization and a GRPO~\citep{shao2024deepseekmath} variant.
%
These works move toward broader multimodal RL settings, but they address different problems from ours.
%
Our work instead studies joint RL training over reasoning-heavy and perception-heavy tasks in open VLMs, where capability heterogeneity, verifier heterogeneity, localization-specific reward shaping, and source-level observability must all be handled within one pipeline.
%
The key gap we address is a public training recipe for heterogeneous reasoning-plus-perception RL that supports multiple task families, modular verifiers, and fine-grained observability of unified training dynamics.


==> sections_refined/7_conclusion_v2.tex <==
\section{Discussion \& Future Work}

We presented V-Triune, a training methodology for unified multimodal RL over reasoning-heavy and perception-heavy VLM tasks.
%
Our results suggest that unified multimodal RL is mainly limited by the lack of a stable way to handle heterogeneous rewards, localization-specific precision shaping, and source-level observability within one pipeline.
%
By organizing training around reward routing, verifier-level outcome verification, and source-level diagnostics, together with Dynamic IoU for localization-centric tasks, V-Triune addresses these bottlenecks in mixed-task RL.
%
Under matched budgets, unified training matches or outperforms specialist mixtures without showing a clear reasoning-versus-perception trade-off, and the final Orsta models improve over their backbones on MEGA-Bench and a broad set of downstream benchmarks, while the same methodology also extends to a new GUI domain.

Two future directions seem especially important.
%
One is to extend unified RL from static benchmark settings to multimodal agentic tool-use tasks.
%
The other is to generalize this training methodology beyond vision, toward joint RL training across speech, video, and text.




% To support full reproducibility of our results, we will publicly release all necessary components, including: (1) the trained models Orsta-7B, Orsta-32B-0321, and Orsta-32B-0326; (2) the complete 47.7K visual reasoning and perception training dataset; (3) the source code for V-Triune, our proposed framework; and (4) detailed documentation and running instructions covering environment setup, training procedures, and evaluation protocols. All materials will be made available under an open-source license upon publication.
% Notably, V-Triune yields Orsta-7B and Orsta-32B, with improvements of 3.2\% and 2.1\% over strong backbones, respectively. Our experiments indicate that reinforcement learning in VLMs primarily serves as an alignment strategy, refining the model’s decision-making and response behavior rather than enabling new knowledge acquisition. This supports the notion that RL fine-tuning enhances the utility and robustness of pre-trained VLMs without altering their foundational capabilities.


% We also acknowledge several limitations that merit further investigation:
% \begin{itemize}
%     \item \textbf{Limited performance scaling in perception tasks:} For visual reasoning tasks, we observe clear trends of increasing response length and reflection ratio as training progresses, akin to test-time scaling laws observed in LLMs. However, such trends are not evident in visual perception tasks. The underlying factors driving performance improvements in perception remain unclear. Exploring multi-step RL for perception tasks, similar to approaches in OpenAI’s o3, may offer new insights and avenues for progress.
%     
%     \item \textbf{Underexplored potential of RL-zero in VLMs:} There is currently limited research on RL-zero for vision-language models. Nonetheless, we see early indications that RL-zero has the potential to surpass the current limitations imposed by supervised fine-tuning (SFT). Given that multi-modal alignment remains a fundamental challenge in VLMs, and that supervised fine-tuning (SFT) may be inherently limited in addressing this issue, we believe that RL-zero has the potential to redefine the optimization paradigm and unlock new capabilities for vision-language models.
% 
% \end{itemize}

% The V-Triune system and Orsta models will be publicly available at \href{https://github.com/MiniMax-AI}{https://github.com/MiniMax-AI}. We hope this work inspires further research into reinforcement learning as a general-purpose training paradigm for vision-language understanding, and encourages exploration of richer reward schemes, advanced reasoning strategies, and task-specific adaptations.

